Classification of spin-chain braid representations

A braid representation is a monoidal functor from the braid category $\mathsf{B}$, for example given by a solution to the constant Yang-Baxter equation. Given a monoidal category $\mathsf{C}$ with $ob(\mathsf{C})=\mathbb{N}$, a rank-$N$ charge-conserving representation (or spin-chain representation) is a strict monoidal functor $F$ from $\mathsf{C}$ to the category $\mathrm{Match}^N$ of rank-$N$ charge-conserving matrices that is natural in the sense that $F(1)=1$}. In this work we construct all spin-chain braid representations, and classify up to suitable notions of isomorphism.

==> reps-03112.tex <==

\module{reps-03112}


\section{Proof of the main theorem, Theorem~\ref{th:mainx}: conclusion}
%$\;$
\subsection{A key combinatorial lemma} $\;$ 
%{{{ Higgs and LEMMAS notation

\ignore{{  %% prmoted to macros2
\newcommand{\chippy}{parted}
\newcommand{\choppy}{choppy}
\newcommand{\roo}{Rule-of-1}
\newcommand{\configuration}{$\II$-configuration}
\newcommand{\SET}{{\mathsf{ Set}}}  % category
\newcommand{\Hom}{Hom}
\newcommand{\Power}{{\mathcal P}}   % power set
\newcommand{\pig}{\overline{\pi}}
\newcommand{\bb}{{\mathsf b}} 
\newcommand{\rrrr}{{\mathsf r}}
}}

We first give a little more notation. 

\mdef
Recall that 
$K_n$ denotes the complete graph on vertices $\{ 1,2,...,n \}$.
Note the natural orientation of edges $i \rightarrow j$ when $i <j$.
We will have in mind also the corresponding 2-graph, the complex over
$K_n$ that includes the triangular faces.
We write $K_n^0$, $K_n^1$, $K_n^2$ for the sets of vertices, edges and faces respectively.
Thus $K_n^0 = \{ 1,2,...,n \}$.

We write $\Hom(A,B)$ for the set of morphisms in the category $\SET$ between
sets $A$ and $B$, i.e. the set of functions.
Thus for example $\Hom(K_n^1, \{x,y\})$ is the set of colourings of the edges of $K_n$
from the colour set $\{x,y\}$.

\mdef
We write $\Power(A)$ for the power set of set $A$.
%
\ignore{{
Observe that  $\Hom(K_n^1, \{x,y\})$ is in bijection with $\Power(K_n^1)$.
(A specific bijection
$$
\bb_y : \Hom(K_n^1, \{x,y\}) \stackrel{\sim}{\rightarrow} \Power(K_n^1)
$$
arises by choosing $x=0$, $y=1$ say.)
}}
%Observe that  $\Hom(A, \{x,y\})$ is in bijection with $\Power(A)$.
%(A specific bijection
Recall that the map
$$
\bb_y : \Hom(A, \{x,y\}) \stackrel{\sim}{\rightarrow} \Power(A)
$$
%arises by choosing $x=0$, $y=1$:
$\bb_y(f) = f^{-1}(y)$,  %contains the elements $a\in A$ with $f(a)=y$.)
is a bijection.

In turn the set $\Power(K_n^1)$ can be considered as the set of full subgraphs
(i.e. subgraphs retaining all vertices) of $K_n$.
Furthermore each subgraph $\gamma$ defines a partition
$\pig(\gamma) \in \PP(K_n^0)$ 
of the vertex set into
connected components.
That is, we have a map
$$
\pig: \Power(K_n^1) \rightarrow \PP(K_n^0)
$$

Note that an element $c$ of $\Hom(K_n^1, \{x,y\})$ gives an element
$\rrrr_y(c)$
of the set $\Power(K_n^0 \times K_n^0)$ of relations on $K_n^0$ by 
$(i,j) \in \rrrr_y(c)$ if $c(i,j)=y$.
The partition $\pig(\bb_y(c))$ is simply the
partition corresponding to the reflexive-symmetric-transitive closure
of $\rrrr_y(c)$.
%\ppm{-all bits lined up ok now paul?}

%}}}
%{{{ parted Lemma

\newcommand{\yy}{y} 
\newcommand{\xx}{x} 
\newcommand{\Homx}{\Hom_x}

\begin{lemma} \label{le:chip} 
(\roo\ Lemma)
An edge 2-colouring of $K_n$,
with colour set $\{ \xx,\yy \}$,
i.e. an element of $\Hom(K_n^1, \{ \xx,\yy \} )$,
is called \xx-{\em \chippy} if every triangle that
has two \yy's has three; i.e. if no triangle has a single \xx.
We write $\Homx(K_n^1, \{ \xx,\yy \} )$ for the set of  \xx-\chippy\ colourings.
\\
(I) The set of \xx-\chippy\ colourings is in bijection with the set of
partitions of the vertices.
In particular $\pig \circ \bb_y$ restricts to a bijection between these sets.
\\
(II) The subset of colourings where no triangle has three \xx's is in
bijection with the subset of partitions into two parts.
\end{lemma}

\proof
(I) This  %is simply
amounts to 
a rearrangement of the definition of equivalence relation,
where \yy\ on  edge $\{ v,v' \}$ means that $v \sim v'$.
\\
(II) This gives the subset where no triple has three vertices in
different parts.
\qed


\ignore{{

\mdef Remark.
Let $\lambda$ be the integer partition corresponding to a given set
partition of a set of order $n$.
Then note that the number of \xx's in the corresponding equivalence relation,
encoded as an \xx-\yy-colouring of $K_n$ as in Lemma~\ref{le:chip},
is
\beq
h(\lambda) = \frac{n^2 - \sum_i \lambda_i^2 }{2} 
\eq
For example $h(31) = (16-9-1)/2 =3$ while $h(22)=(16-4-4)/2=4$.

}}

%}}}
\subsection{Admissible configurations} $\;$ 
%{{{ Higgs

\mdef \label{de:Higgs}
A {\em (Higgs) \configuration} of $K_n$ is an assignment of a scalar to
each vertex;
and matrix to each edge,
so that each $K_2$ subgraph is assigned
from the set of six types
$\II = \{ \off, 0, \uppfii, \mfii, \uppai,\mai \} $
as in \eqref{pa:schema2}.
(Note that there are variables in all these components.)

By Proposition~\ref{pr:L2class2}
and Theorem~\ref{th:constraints}
a necessary condition for an element of $\Match^N(2,2)$
to give a braid representation is that it gives an \configuration\ of $K_N$.



\mdef \label{de:admissible}
A `ground state'
or `admissible'
configuration of $K_n$ is an \configuration\ such that every
triangle configuration is
in the orbit of 
one of those nine forms given in Proposition~\ref{pr:N3}.
(Note that variables are constrained by these conditions, as well as types.)


By Proposition~\ref{pr:N3}
and the form of the constraints in Theorem~\ref{th:constraints}
(from which we observe that the total constraint set is the union of constraint
sets across all $K_3$ subgraphs)
a necessary and sufficient condition for an element of $\Match^N(2,2)$
to give a braid representation is that it gives an admissible configuration of $K_N$.


%}}}
\subsection{The proof} $\;$ 
%{{{ proof

%\medskip\medskip

%Here we will enumerate groundstates
%(as varieties in the appropriate variables) in all ranks. That is, we will

We require to 
show that $\Rec(\SSS_N^\C)$ gives the set of % groundstates/
braid representations;
and by \eqref{de:admissible} this is the same as the set of groundstates.
That is, 
we require to show
\\
(I) that every solution is in  $\Rec(\SSS_N^\C)$,
and
\\
(II) that every element of  $\Rec(\SSS_N^\C)$ gives a solution.

For (I)
We proceed as follows. Suppose $\alphaa$ is a solution, i.e. an
admissible configuration.
We require to show that there is a $(p,q,\rho,s) \in \SSS_N$
and a point in $\C^{(p,q)}$ 
such that applying $\Rec$
to this germ
gives $ \alphaa$. % \ppm{for some -.}
First let us consider the data of the $\off$ edges.
For this (and in various guises hereafter) we will make use of
Lemma~\ref{le:chip}.
%\ppm{...}

%\ppm{(II) ...get the logic clear ...}


%}}}
%{{{ Lemmas applying the parted Lemma

%%\newcommand{\alphaa}{\ul{\alpha}} % I-config
%% prmoted to macros2
%\newcommand{\alphaa}{\pmb{\alpha}} % I-config

\newcommand{\partp}{\pi_{\mathsf{p}}}
\newcommand{\partq}{\pi_{\mathsf{q}}} 
\newcommand{\partr}{\pi_{\rho}} 
\newcommand{\parts}{\pi_s} 

\begin{lemma} \label{le:off1}
(I)
The $\off$ data of an admissible configuration
$\alphaa$ 
of $K_N$
induces a partition
$\partp(\alphaa)$ 
of the vertices (into `nations');
and in particular there is a $\off$ on an edge if and only if this edge is between
vertices in different parts.
\\ (II)
Furthermore, every $\off$ between the same two nations carries the same parameter.
\\ (III)
Thus a solution $\alphaa$ is partially characterised by
the partition $\partp(\alphaa)$ and the parameters it associates to the
edges of $K_{\partp(\alphaa)}$
(each vertex of  $K_{\partp(\alphaa)}$ represents a nation; and 
each edge of  $K_{\partp(\alphaa)}$ represents the collection of edges of
$K_N$ that are between the same two nations).
\\ (IV) The $\off$ data of $\alphaa$ agrees with what we obtain by applying
$\Rec$ to a germ with $p=\partp(\alphaa)$.
\end{lemma}

\proof
(I)
Observe from the list of allowed triangle configurations
in Prop.\ref{pr:N3}
that this
data is \chippy\ with $\off$ in the role of \xx\ 
and all other decorations together in the role of \yy.
Now apply the \roo\ Lemma.
\\ (II)
The parameter constraint comes from observing the configurations in
Prop.\ref{pr:N3} with exactly two $\off$s.
We see firstly that if two edges between nations meet then they carry the same
parameter. So now suppose
$\{v,v' \} $ are % be non-necessarily-
distinct vertices in one nation, and
$\{w,w'\}$ in another.
Thus $vw$ and $v'w'$ are edges between nations, hence $\off$ edges.
But of course so is $vw'$, and this has the same parameter as both.
\\
(III,IV) follow immediately. %  and
\qed


\begin{lemma} \label{le:0s}
(I)
Let $\alphaa$ be  an admissible configuration of $K_N$.
Consider a part of the partition
$\partp(\alphaa)$
induced by $\off$. 
Edge 0's induce an equivalence %, i.e. a partition,
on vertices
(i.e. a partition, of this nation into `counties')
---  in particular two vertices are in the same part if and only if their
common edge has a 0.
Thus overall we have a partition $\partq(\alphaa)$ refining $\partp(\alphaa)$.
And then %arrows as in \ref{what?}
`signs' (the bar-unbar data in the edges labeled from $\{ \pfii,\mfii,\pai,\mai\}$)
induce a `weak total'
order (i.e. a partial order that is a total order on equivalence
classes of the equivalence relation --- the counties in a nation).
Thus overall we have an order
$\partr(\alphaa)$. 
\\
In particular there is a total order on counties in each nation so that
if county $q_i$ is above $q_j$ in the order and vertex $v$ is in $q_i$
and vertex $w$ in $q_j$ then the $vw$ edge is +-type if $v<w$
and is $-$-type otherwise.
\\ (II) The $\off$, 0 and sign data of $\alphaa$ agrees with what we obtain by
applying $\Rec$ to a germ with
$p=\partp(\alphaa)$, $q=\partq(\alphaa)$ and $\rho=\partr(\alphaa)$. 
\end{lemma}

\proof
(I)
We see that
edge 0's induce an equivalence by comparing allowed triangle
configurations with the \roo\ Lemma.
Taking the county partition data across all nations we have
a refinement of
$\partp(\alphaa)$ --- call it $\partq(\alphaa)$.
A configuration induces a well-defined order
$\partr(\alphaa)$
on the quotient
--- the counties in each nation ---
since
triangles are never cyclic-ordered
%\ppm{-explain paul}
(we will give  illustrative examples next)
and triangles with a 0 `collapse'
consistently.

For example consider a triangle with vertices 2,5,9
(say, any triple will do --- note that our edge directions on $K_N$ will give
an `ambient' order on these vertices)
and suppose first in the same nation
but not the same county --- so decorated from $\{ \pfii,\mfii,\pai,\mai\}$.
For now we consider only the $\pm$ aspect of this.
The induced relation between 2,5 is 2<5 if + and 2>5 if - (abusing notation for now).
The relation between 5,9 is 5<9 if + and 5>9 if -.
From the 9-rule (in particular Figure~\ref{fig:sga1})
we see that if 2<5 and 5<9 then 2<9,
and so on, so this is an order.
Specifically, looking at the Figure, the top case is all-+ and so we use the
ambient order, which is of course acyclic.
Subsequent cases are generated by the
$\Sym_N$ action so, for example, if we perm 2,5 then this edge becomes - while the others
remain +, thus we have 5<2<9.
Meanwhile if instead we perm 2,9 then all signs are changed and we indeed have 9<5<2.
...
On the other hand suppose there is a 0 decoration.
Again from the 9-rule, which is given explicitly for ++0 cases, we see here that
if $5\sim 9$ then 2<5 and 2<9; and then the $\Sym_N$ action generating other cases
respects this consistent order.
%...
$\;$ (II) follows immediately.
\qed


%}}}
%{{{ 2-part partition stage etc

\begin{lemma}
Let $\alphaa$ be  an admissible configuration
%$\alphaa$
of $K_N$.
Consider a part $p_i$ of the partition
$\partp(\alphaa)$
induced by $\off$;
and the partition of the vertices of this part induced by 0,
as in Lemma~\ref{le:0s}. 
The $\pai\pfii$ edge decoration data induces a partition on the parts of $p_i$
%(hmm. need to explain what this gibberish means!)
%It is a partition
into (at most) two parts, %only because there is no aaa triangle.
with $\pai$ in the separating role;
with  two vertices from the same nation only having different parameter
if in different such parts, i.e. with edge label $\pai$.
To record this data as a single two-part partitioning across all nations,
we may order the two parts in each nation by the child-first order,
then simply combine all the first parts, and combine all the second parts.
Taken over all nations we thus have a two-part partition
$\parts(\alphaa)$.
%
Applying $\Rec$ to a germ with 
$(\partp(\alphaa),\partq(\alphaa),\partr(\alphaa),\parts(\alphaa))$
we obtain $\alphaa$.
%\\
\ppmx{-now explain the vertex variables - all the same if 0-connected
and same if f-connected. ...}
%\\ \ppm{And do the stage (II) thing!?}
\end{lemma}

\proof
This is  a matter of unpacking the definitions and then using
the \roo\ Lemma for a third (!) time, this time using part (II),
because there is no
$\pai\pai\pai$ triangle.
$\;$
The final point follows immediately from the $\Rec$ recipe.
\qed

\ignore{{
\mdef
In short then, a configuration $\alphaa$ should be organised firstly as a
partition according to $\off$ (we say a partition into `nations').
Then as a partition according to 0 (`counties').
Then 
...
\ppm{NEXT explain variables}
Now observe
from Proposition~\ref{pr:N3}
that any triangle between two nations, thus with exactly two $\off$s,
has the same variable on each of these edges.
Thus every edge between these two nations has the same variable.
\\
Similarly 
...
}}

%}}}
%{{{ stage II

\medskip

%We finish  by showing (II) that the $\Rec$ construction gives solutions. 
%%\\ (I) that every solution arises this way.
%%\\ \ppm{Paul, write it out now.}


(II) Let $(p,q,\rho,s) \in \SSS_N$ and consider $\Rec(-)$.
%Observe from \ref{de:Rec}
We require to check 
that every triangle is as in Prop.\ref{pr:N3}.


\begin{lemma} \label{le:IIi}
\ppmx{Paul, push this to a later Lemma?, since it belongs to stage (II)
of main proof:}
%(IV)
%%Furthermore, i
Suppose we have a configuration of $K_N$ constructed  %by forming
from
a partition of vertices %and then
$p$ by 
decorating each edge between the same two parts with a $\off$
carrying the same parameter (as in $\Rec$).
Then all the triangles involving $\off$ are in admissible configuration.
\end{lemma}

\proof  %(IV) again f
As before we write $i<j<k$ for the vertices and order the edges
$ij,ik,jk$.
If all three vertices lie in different nations then $\Rec$ gives
edge configuration $\off\off\off$, which is admissible.
If two vertices lie in the same nation then we have $\off\off *$,
$\off *\off $ or $*\off\off $, for some *, with the $\mu$ parameter the same
on the two $\off$ edges.
From inspection of cases in Prop.\ref{pr:N3} we see that all such
are admissible. 
\qed

\begin{lemma} \label{le:IIii}
%\ppm{Paul, push this to later Lemma? - Again its a stage (II) of main proof thing:}
%(II)
Suppose we have a configuration of $K_N$ constructed firstly as in
%Lemma~\ref{le:off1}(IV)
Lemma~\ref{le:IIi}
and then from a refinement of $p$ to $q$ by decorating
each edge within a county $q_i$ by 0;
and then from a
total ordering $\rho$ of the counties in each nation
by decorating each edge between counties in the nation as in $\Rec$
from \ref{pa:rec}.
Then
every edge is decorated from $\{\off,0,+,- \}$, and 
every triangle is  consistent at the level of orientation with
an admissible configuration.
\ppmx{...hmm, maybe better to already include the $s$ data now for this bit?
- perhaps then demoting this part of Lemma to next Lemma.
Or, sticking with $+-$, maybe we can get away with it here.}
\end{lemma}

\proof %(II) Again b
Triangles involving $\off$ involve more than one nation, and are
already admissible by Lemma~\ref{le:IIi},
so we need only check each triangle lying within a nation.
As before we write $i<j<k$ for the vertices and order the edges
$ij,ik,jk$.
If all three vertices lie in the same county then $\Rec$ gives
edge configuration 000, which is admissible.
If two of three vertices lie in the same county then $\Rec$ gives
a configuration like 0** or *0* or **0, with the *'s depending on $\rho$.
In the 0** case $i,j$ are in the same county.
If $\rho = (ij,k)$
(in the obvious shorthand) then $k$ is above both
in both the natural and the $\rho$ order, so we have 0++.
Comparing with  Prop.\ref{pr:N3} and the orbit table we see that
this is consistent with  admissibility.
(The cases shown in  Prop.\ref{pr:N3} are both $\rho=(i,jk)$ which is ++0.)
If $\rho = (k,ij)$ then we have $0--$ which is again consistent.
Finally for these cases note that $\Rec$ assigns the same parameters to
both edges as required.
It remains to consider the cases with three different counties,
such as $\rho = (i,j,k)$. This gives +++ with all edges assigned the
same parameters, which is again consistent.
The case  $\rho = (j,i,k)$ gives $-++$ (cf. Fig.\ref{fig:sga1})
and the rest of the orbit follows.
%... $\Rec$ assigns a decoration to every edge, so 
%By inspection from Prop.\ref{pr:N3}, for the moment only tracking
%the $\{\off,0 +,- \}$ data. ... ...
\qed

%}}}
%{{{ final lemma

\begin{lemma}
%\ppm{Finally, do the af bit...}
Suppose we have a configuration of $K_N$ constructed firstly as in
Lemma~\ref{le:IIii}
and then
from a partition $s$ of the vertices into two parts
by assiging vertex parameters and replacing $\pm$ labels with
corresponding $\pai,\pfii,\mai,\mfii$ labels as in $\Rec$.
Then every triangle is admissible.
%,continuing with the last (two?) steps of $\Rec$, ...
\end{lemma}
\proof
With regard to the $\pai\pfii$
labels, irrespective of signs, the admissibility conditions stipulate only
that configurations like $\pai\pfii 0$ and $\pai\pai\pai$ must not arise.
The former is impossible since $\Rec$ assigns the same edge label to
every edge between a given vertex and a county.
Since $s$ partitions counties in a nation into at most two parts
$\pai\pai\pai$ is not possible. \qed

%(I) ...

\medskip

Having established directions (I) and (II), 
 this concludes the proof of Theorem~\ref{th:mainx}. \qed

%}}}

A complete worked example can be found in \S\ref{sec:N4}. 

% the rest from here moved to reps-N4

\vspace{.21in}


\subsection{On further properties of orbits of solutions} $\;$ 
\ppmx{What has happened to the all-+ Lemma and the 6-rule in this version, paul?!}

Recall that our Theorem raises the question of the appropriate notion of
equivalence of representations in this setting.
As mentioned,
in large part this comes down to the symmetries intrinsic to the target.
In the next few steps we deal with these symmetries.

%{{{ non-- Lemmas

\newcommand{\Norb}{\Sigma_N \times \Zz_2}

\beff{}{{

%\mdef It will be convenient to refer to $f,a$ as $+$-oriented and $\ul{f},\ul{a}$ as $-$-oriented. 

\mdef
{\bf 6-rule}: if an oriented chain of two edges is signed with the same sign
in $F(\sigma)$
then the
`long' edge completing the triangle is signed with the same sign.
%\\
--- To see this check the 9-rule list
\ref{pr:N3}   %\ppm{\eqref{list of 9 allowed}}
and
the orbit of +++ in Table~\ref{tab:1ad}. %\ppm{\eqref{orbit of +++}. }
\\
{
(This is called 6-rule since it reduces the number of possible edge $\pm$-colourings
of a triangle from eight to six. It also reduces the number of $\pm0$-colourings.)
}
}}


\begin{lemma} \label{lem:no-}
Every $\Norb$ orbit of solutions contains an element with no $-$-orientation.
\\
Furthermore, in such a non-$-$ configuration the elements of a 0-part
(a county) 
are clustered with respect
to the natural order in their nation, i.e. they are consecutive. 
\end{lemma}

\prooff\ 
First we note that the claim holds if it holds for 1-nation solutions,
since there are perms that act non-trivially only on a single nation and the $\off$-edges
out of that nation, restricting to a complete set of perms on that nation.
So now consider a single nation.
We work by induction on $N$. The claim is true for $N<4$ by inspection of our explicit
solution sets.
Suppose true at level-$N$ and consider $N+1$.
WLOG by inductive assumption consider a configuration with all (signed) edges $+$
between
vertices $1,2,..,N$
(any non-signed edges are 0).
\ignore{{
Observe that configurations with 0s
on all these edges must have the same sign on all remaining edges, edges to $N+1$.
If all + then we are done. If all $-$ then
the transposition $(1 \; N\!+\! 1)$ \ppm{...} 
%can effectively be reduced to lower rank).
}}
Consider what configurations of edges to vertex $N+1$ are allowed here. % by the 6-rule.
Neglecting cases with 0s on the  edges to $N+1$ for a moment we have, say,
as on the left here:
%we may consider this:
\[
\includegraphics[width=5.4\ccm]{xfig/gon51.eps}
\hspace{.5\ccm}
\includegraphics[width=5.4\ccm]{xfig/gon52.eps}
\]
By the 6-rule, if the $i$ to $N+1$ edge is + then,
since the $i-1$ to $i$ edge is +,
the  $i-1$ to $N+1$ edge is also +.
Indeed this is also forced in the case where the $i-1$ to $i$ edge is 0.
Thus there are $N$ possible configurations of form $++...+--..-$
(NB all these arrows point to $N+1$).
The $i$-th of these configurations is taken to
$+++...+$ by the perm $(i...N)$, so we are done in these cases.
%\ppm{
In case of 0 on a long edge $i$ to $N+1$, the edges $j$ ($j<i$) to $i$ and
$j$ to $N+1$ must be the same, so these edges satisfy the no-$-$ claim.
Thus it remains only to address the edges after the last 0.
Suppose this last 0 is $i$ to $N+1$.
The edges $k$ to $N+1$ with $k>i$ will all be opposite to the corresponding
$i$ to $k$ edge (which is either + or 0), so either $-$ or 0.
Now apply the perm $(i\; N\!+\!1) $. This has the effect of making the $N+1$ vertex
the `new' $i$ vertex and incrementing $i$ et seq. Thus all the edges that were
$k$ to $N+1$ are reversed, so all the $-$s become +,
while the relative positions of all other vertices are preserved, so signs do not change
--- i.e. they remain non-$-$.
%...finish!!!}

The second claim follows from the 9-rule.
\qed



%}}}



\vspace{1cm}



==> reps-N2proof.tex <==
\module{reps-N2proof}

%{{{ proof

\beff{}{{
\mdef\label{proof of N2}
\noindent
{\bf Proof.}  of Prop. \ref{pr:L2class2}.

\noindent
Only the %first
%4
equations (\ref{eq:31xx0}-(\ref{eq:31xxx0})  (and their images under the action of $\Sigma_2$) are relevant for $N=2$.
\ppmx{[surely we don't need to write them again here??-]}
\ignore{{
\begin{eqnarray*}
&&a_{12} (a_{1}^2 -a_{12} a_{1} -b_{12} c_{12}) =0,\hspace{1cm}
a_{12} (a_{2}^2 -a_{12} a_{2} -b_{12} c_{12}) =0,\\
&&a_{12} c_{12} d_{12} = 0 = a_{12} b_{12} d_{12} ,\hspace{1cm}
a_{12} d_{12} (a_{12}-d_{12})=0.
\end{eqnarray*}
}}
Under the transposition $(1\/2) \in \Sym_2$ we obtain %the same
similar
equations %as above,
but with $a_{12}$ and $d_{12}$ interchanged,
so we take it
case by case %in cases
to find necessary and sufficient conditions for these constraints.

Observe that $a_1,a_2$ and $a_{12}d_{12}-b_{12}c_{12}$ are non-zero by invertibility. If $b_{12}c_{12}=0$ then $a_{12}d_{12}\neq 0$, so the equations
%above
imply $a_{12}=d_{12}=a_1=a_2$, which is case $0$.
It is routine to check that this is indeed a solution.

Now if $b_{12}c_{12}\neq 0$ then there are 3 cases to consider: $a_{12}=d_{12}=0$ or exactly one of $a_{12}$ or $d_{12}$ is non-zero.
In the first case all equations are satisfied, so that $a_1,a_2,b_{12},c_{12}$ may be chosen arbitrarily.
The X transformation then allows $b_{12}=c_{12}$.

\sout{First}
Next
suppose that $b_{12}c_{12}a_{12}\neq 0$, and $d_{12}=0$.  This implies that $b_{12}c_{12}=a_2(a_{12}-a_2)=a_1(a_{12}-a_1)$.
Now the characteristic polynomial of the $2\times 2$ matrix
(call it $A(1,2)$)
is $x^2-a_{12}x-b_{12}c_{12}$ so that $a_1$ and $a_2$ are eigenvalues of $A(1,2)$.  Let $\alpha,\beta$ be these eigenvalues.
Since $Tr(A(1,2))=a_{12}$ we have that $a_{12}=\alpha+\beta$, and
\ppm{similarly}\sout{since??}
$Det(A(1,2))=-b_{12}c_{12}=\alpha\beta$.
Using the X transformation we may assume that $b_{12}=-\alpha\beta$ and $c_{12}=1$.
Notice that the only restriction on $\alpha,\beta$ is that $\alpha+\beta\neq 0$. Now there are two cases, up to the obvious labeling ambiguity of $\alpha$ and $\beta$: either $a_1=a_2=\alpha$ (case $\mathbf{a}$) or $a_1=\alpha$ and $a_2=\beta$ (case $\mathbf{f}$).

The case $a_{12}=0$ is completely analogous: we find that $d_{12}=\alpha+\beta$, $b_{12}=-\alpha\beta$ and $a_1=a_2=\alpha$ (case $\underline{\mathbf{a}}$) or $a_1=\alpha$ and $a_2=\beta$ (case $\underline{\mathbf{f}}$).

%Note that
In
any of the last 4 cases it is possible that $\alpha=\beta$,
%in which case
whereupon
the $\mathbf{a}$ case prevails.
%
%}}}
%{{{ iffalse/qed
%
   \iffalse 
    
    %\ppm{fix $f,g$?}
\hspace{.1in}
%(scaling one eigenvalue to 1 by homogeneity of relations)
%where
%where, setting $f=1$ for a moment,



Invertibility requires that $\aaf,\aag \neq 0$ and
$ad \neq bc$, so 
if $bc=0$ then $ad \neq 0$.
The braid relations  %\eqref{eq:braidx}
require %firstly
%$abd=acd=0$, $(a-d)ad=0$.
\beq \label{eq:br1}
abd=acd=0, \;\; (a-d)ad=0   .
\eq
%Thus if $bc=0$ then noting invertibility we have $b=c=0$ and $a=d \neq 0$.
%Secondly
\beq \label{eq:br2}
\mbox{
  $a(\aag(\aag-a)-bc)=0$, \hspace{.1cm} $a(\aaf(\aaf-a)-bc)=0$,}
\eq \[
\mbox{
$d(\aag(\aag-d)-bc)=0$, \hspace{.1cm} $d(\aaf(\aaf-d)-bc)=0$.
}
\]

\noindent
(0)
If $bc=0$ we have $\aaf=a=d=\aag$ by invertibility, \eqref{eq:br1} and \eqref{eq:br2}.

\noindent
(1) If $bc \neq 0$ we have $ad=0$ by \eqref{eq:br1}.

\noindent
(1.0) If $a=d=0$ the conditions are immediately satisfied.

\noindent
(1.1)
%Assuming the functor $\FF_{}$ is not diagonal we have $ad=0$.
Taking $d=0$
%without significant loss of generality,
and  $a \neq 0$,
the remaining conditions are $bc=\aaf(\aaf-a)=\aag(\aag-a)$.
Thus $a=\aaf-bc/\aaf$ and the characteristic equation for the middle block
is $(\lambda - \aaf)(\lambda +bc/\aaf)=0$.
If $\aaf \neq \aag$ then $bc=-\aaf\aag$ and $a=\aaf+\aag$.
%%$\aaf^2 -\aaf a +(a-1)=0=(\aaf-1)(\aaf-(a-1))$.
%$f=1$ or $f=a-1$.
In either case, $\aaf$ and $a-\aaf$ are the eigenvalues
(with 
multiplicities 3 and 1 in (1.1ii) and 2 and 2 in (1.1i)).

\noindent (1.2) similar.

%(scaling one eigenvalue to 1 by homogeneity of relations)
\fi
\qed

}}

%}}}
\newcommand{\ques}[1]{ \medskip  \noindent Question. #1}
%{{{ ignore 2-eigenvalue cases

\ignore{{
Note that in either
`two-eigenvalue' 
case $b,c$ are only constrained through $bc$.
Thus we may take $b=c$ or for example $c=1$; and we may continuously
vary between these. This is a variant of the classical
semi-normal/normal isomorphism and for $\Bcat$ itself these
representations are generally classed together.
However we are interested in extension to $\LBcat$,
and it is not true in general that conjugations in
images of $\Bcat$ commute
with  extension. Thus we should treat them separately. 
}}

%$a(bc-1+a)=0$, $a(bc-f^2+af)=0$.
%\ppm{finish me}

%\newcommand{\ques}[1]{ \medskip  \noindent Question. #1}

%\ques{  What happens to 4 ev case restricted to 2 evs?
%  (Now answered in main doc.)  }

%}}}

\ignore{{
%{{{ naming of names of symbols

\medskip

{\em Notation}:
In what follows we will write simply $/$ for case $(1.0)$ of the
classification;
and
$+_i, +_{ii}, -_i, -_{ii}$ for cases (1.1i), (1.1ii), (1.2i), (1.2ii)
respectively.

%}}}
\subsection{On classification transversals}
%{{{ jobs

\ppm{JOBS:} Give transversals with respect to the above and the
consequent natural functional classification schemes...
(thus the Rittenberg and the `$sl_2$' etc will come up as transversal elements).

%}}}
}}


\medskip


==> reps-N4.tex <==

\module{reps-N4}

%%\newcommand{\ova}{\rfloor} 
%%\newcommand{\ova}{\!\int\!} 
%%\newcommand{\ova}{\!\langle\!} 
%%\newcommand{\ova}{\!\succ\!} 
%\newcommand{\ova}{\prime\hspace{.051em}}  % promoted to macros2


\section{Enumeration of representations up to discrete symmetries}
\subsection{One-nation combinatorics}
%{{{ one-nation

Since solutions can be resolved
(albeit with some subtleties)
into the collection of their nation components,
it is useful to classify one-nation solutions. 

For enumeration specifically of one-nation solutions
the $P$-symmetry
from (\ref{de:flip1})
yields directly that we have larger orbits (than just $\Sigma_N$)
and hence smaller transversals.
However the $P$-symmetry acts globally, so
{\em per se} it cannot be applied independently to nations in a multination solution.
So here we enumerate weak orders without
automatically
imposing $P$.
This is a mild redundancy here
(cf. \cite{Andrews21}), but simplifying later.

%}}}
%{{{ tree


%\medskip

%\mdef
We will first enumerate the weak orders we need here - equivalently compositions
of $N$ for each $N$.
(We must then $af$-label edges in the underlying chain;
then lift this to the graph.)
As noted in (\ref{de:laml1}),
an easy way to list all weak orders here is with %Pascal's triangle.
a bifurcating tree. %, as in
See Figure~\ref{fig:cwo1}.
Recall the bifurcation is: add-1 to the last part or add-1 to a new part.


%}}}
%{{{ fig

\newcommand{\bif}{\ar[dl] \ar[dr]}
\newcommand{\biff}{\ar[dll] \ar[drr]}
\newcommand{\bifo}{}

\begin{figure}
\[
\xymatrix@C=3pt{
&&&&&&&1 \ar[dllll] \ar[drrrr]
\\
&&&2\biff&&&&&&&&1\ova 1\biff
\\
&3\bif&&&&2\ova 1 \bif&&&& 1\ova 2\bif &&&& 1\ova 1\ova 1\bif
\\
4\bifo&&3\ova 1\bifo&&2\ova 2\bifo&&2\ova 1\ova 1\bifo&&1\ova 3\bifo
   &&1\ova 2\ova 1\bifo&&1\ova 1\ova 2\bifo&&1\ova 1\ova 1\ova 1
}
\]
\caption{Compositions and weak orders. \label{fig:cwo1}}
\end{figure}

%}}}
%{{{ Details 1/1/1 -> 1/2/1

Note that in our chosen transversal,
from Lemma~\ref{lem:no-},
the elements of a county are consecutive in the nominal order,
so the weak order is a chain of counties.
The $af$ edge labelling comes from a partition of the vertices of the chain
into at most two parts
(edge labelling in the chain
lifts to a complete labelling - if counties are not all singletons -
in an obvious way:
 all edges from one county to another have the same label). 
%\ppm{-so you say Paul, but unpack a bit!}).
In this sense, we only need to enumerate two-part partitions of chains of each
length. In principle all other solutions then arise by the lift.
(This is the strategy. We will illustrate with some details.)

\mdef
The enumeration of
rank-$N$ one-nation
solutions (in our transversal)
whose weak order is a chain of singletons - thus of length $N$ -
is given simply by partitioning the vertices into at most two parts.
The parts are not ordered (\ppm{right?}{ swapping just changes the names
of the indeterminate variables})
so there are $2^{N-1}$ such partitions.
They can be organised so that the smaller part has size
$i=0,1,..., \lfloor{N/2}\rfloor$.
In other words the combinatoric here is as in one
%side
half
of Pascal's triangle (one side, and half the middle term in even ranks). 
In detail this (and the lift to non-singleton counties) proceeds as follows.
\\
For a chain of length-1 (the left-hand case in each row of
Fig.\ref{fig:cwo1}) there is nothing to do, so a single solution.
\\
For chain length-2 we have either a single part,
thus an $f$ edge; or two parts, thus an $a$ edge.
(Note that this indeed reproduces our 1-nation solutions in  case $N=2$.
In case $N=3$ these become $ff$ and $aa$ respectively, thus altogether either
$0ff$ and $0aa$ or $ff0$ and $aa0$.)
\\
For length-3 we have: a single part, thus $fff$;
or two parts with the elements of the two-element part `adjacent',
thus $faa$ (or $aaf$);
or two parts with the two-element part split, thus $afa$.
(At this point we know
%everything
all one-nation solutions
for $N=3$. See below for a tabulation of
this case.)
\\
For length-4 we have: a single part, thus $ffffff$;
or  partition 31
and elements of the 3-element part consecutive, thus $fffaaa$ (or $aaafff$);
or partition 31 with the 3-element part split, thus $faaffa$ (or $...$);
or partition 22 with the first part either $\{ 1,2\}$ or $\{1,3\}$ or $\{1,4\}$,
thus $faaaaf$ or $afaafa$ or $afafaa$ respectively.
\\
For length-5 we have the (up to) 2-part partitions 5, 41 and 32.
The number of solutions
(in our transversal)
in each case is the number of ways of choosing
the second part, thus ${N}\choose{i}$ for $i=0,1,...,\lfloor{N-1/2}\rfloor$
(and $\frac{1}{2} {{N}\choose{N/2}}$ in even ranks).
Thus 1+5+10 or $2^{N-1}$ here in total.
The first of these is $ffffffffff$.
\\
The general pattern will now be clear.
For length-6 we have 6, 51, 42 and 33 giving 1+6+15+10.
\\
\ppm{-Do you agree with all this Eric? The claim is that we already used most
of the symmetry getting into the sign transversal, so these guys are distinct
...for us.
%In particular the $N=4$ table below needs some additions...
}
%... \ppm{finish me Paul!}


%}}}
%{{{ N=3

%\newcommand{\ova}{\rfloor} 

\mdef
The table below gives the $\Sigma_N$-orbits of one-nation solutions for $N=3$,
using the non-$-$ transversal as per Lemma~\ref{lem:no-}
(note the $a\ova b\ova c$ notation for single-nation weak orders):
%\[ ... \]
%}}}
%{{{ N=3 table
\[
%\hspace{-1.1cm}
\begin{array}{|c|c|cc|cc|ccc|c|c|cccc}
\hline
\mbox{0-induced partition} &
3 & \multicolumn{2}{c|}{21} & \multicolumn{2}{c|}{111}   & 
\\ \hline
\mbox{weak order}&
3 & \multicolumn{2}{c|}{2\ova 1 \hspace{.432in} 1\ova 2}
  & \multicolumn{2}{c|}{1\ova 1\ova 1} &
\\ \hline
0+ &
000 & \multicolumn{2}{c|}{0++\hspace{.432in}++0}
     & \multicolumn{2}{c|}{+++} &
\\ \hline
\mbox{$f$-induced partition} &
3 & \;\; 21\;\;\;\;\; 3 & \;\;\;\;21\;\;\;\;\; 3 &   \;\;\;\;  21  & 3 &
\\ \hline
\mbox{$fa$-config of soln.} &
000 &
  \multicolumn{2}{c|}{
    \begin{array}{c} 0aa \hspace{.321in} \\ \hspace{.31in} 0ff \end{array}
\;\;    \begin{array}{c} aa0 \hspace{.321in} \\ \hspace{.31in} ff0 \end{array}
    }
     &  \multicolumn{2}{c|}{
    \begin{array}{c}
    aaf \hspace{.321in} \\
    afa \hspace{.321in} \\
    faa \hspace{.321in}
              \\ \hspace{.54321in} fff \end{array}}
     &  
\\
\hline
\end{array}
\]

%}}}
%{{{ Recall
Recall we cannot have $+0+$ (confer Table~\ref{tab:1}
and Lemma~\ref{lem:sundry0s}(II),
and Lemma~\ref{lem:no-}).
If $N=3$ then this size-3 nation is the only nation and $P$-symmetry makes
$1\ova 2$ redundant.
{\em This leaves the six one-nation solutions from the last two lines of \ref{}
as required.}

%}}}
%{{{ N=4


\mdef Now we give $N=4$ in the same style.
We omit the chains $1\ova 3$ and $1\ova 1\ova 2$ in order to fit the table on a line.
They can be reconstructed by applying $P$ to $3\ova 1$ and
$2\ova 1\ova 1$ respectively.


%}}}
%{{{ arrays \nu=4

%\ppm{Finish conforming this to the above style! 4s (now done) and an 8:}
\[
\hspace{-1.1cm}
\begin{array}{|c|c|cc|cc|ccc|c|c|cccc}
\hline
0-pt & 4 & \multicolumn{2}{c|}{31} & \multicolumn{2}{c|}{22} & \multicolumn{4}{c|}{211} & 1111 & 
\\ \hline
weak  & 4 & \multicolumn{2}{c|}{3\ova 1^*} & \multicolumn{2}{c|}{2\ova 2} &
   \multicolumn{3}{c}{2\ova 1\ova 1^*}
   & \multicolumn{1}{c|}{1\ova 2\ova 1} & 1\ova 1\ova 1\ova 1 &
\\ \hline
0+ & 000000 & \multicolumn{2}{c|}{000+++}
     & \multicolumn{2}{c|}{0++++0} &
           \multicolumn{3}{c}{0+++++} & \multicolumn{1}{c|}{++0+++} & ++++++
\\ \hline
f-pt & 4 & 31 &4 &     22  & 4 & 22 & 31 & 4 &     22 \;\; 31\;\; 4 &  22 \;\; 31\;\; 4 &
\\ \hline
fa & 000000 &
  \multicolumn{2}{c|}{
    \begin{array}{c} 000aaa \hspace{.21in} \\ \hspace{.1in} 000fff \end{array}}
     &  \multicolumn{2}{c|}{
    \begin{array}{c} 0aaaa0 \hspace{.21in} \\  \hspace{.21in} 0ffff0 \end{array}}
     &  \multicolumn{3}{c|}{
    \begin{array}{c}
    0\ul{aa}\,\ul{aa}f  \hspace{.321in} \\
    0\ul{ff}\ul{aa}a  \hspace{.021in} \\
    0\ul{aa}\ul{ff}a \\  \hspace{.21in}
                     0\ul{ff}\,\ul{ff}f \end{array}}
     & \multicolumn{1}{c|}{
    \begin{array}{c}
    \ul{aa}0f\ul{aa}  \hspace{.321in} \\
     \ul{aa}0a\ul{ff}  \hspace{.021in} \\
     \ul{ff}0a\ul{aa} \\  \hspace{.21in} \ul{ff}0f\ul{ff} \end{array}} 
  &   \begin{array}{c}
  faaaaf  \hspace{.21in} \\
  afaafa \hspace{.21in} \\
  afafaa \hspace{.21in} \\
  fffaaa  \\
  aaafff  \\
  faaffa  \\
  afafaf \\
  \hspace{.21in} ffffff \end{array} &  
\\
\hline
\end{array}
\]
Here $0\ul{aa}\,\ul{aa}f  $ indicates the edges that are forced equal by the 0s.
Thus $0\ul{aa}\,\ul{aa}f $ is derived from $aaf$, and so on.

%}}}
%{{{ Total

\mdef
Observe that the total enumeration, organised as in a row of the tree
(the row for rank $N$ say), is obtained from
 the previous row by taking the same number if we step left; and doubling
 if we step right.
 Observe that this means that the sum for the right half of the tree is twice
 that for the left half.
And the sum for the left half is the same as for the whole previous row.
We have established:
\\
{\bf{Theorem}}.
%Thus t
The total number of one-nation solutions in the transversal
(of $\Sigma_N$ orbits) is
$3^{N-1}$.
\qed

%}}}
\subsection{Complete enumeration examples} \label{sec:N4} 
%{{{ Since we may

\ppmx{Paul: fix the minor anachronisms here.}
As noted, 
since we may work up to the action of $\Sym_N$  %the symmetric group
permuting
the vertices, the set partitions (into nations) are effectively indexed by the
corresponding integer partitions. 
So for example in rank 4 we have nation-partitions 4, 31, 22, 211,
1111
(in the obvious shorthand).

\ignore{{
Case 4 has no $\off$s.
The possible partitions according to 0s
(i.e. of the single nation into counties)
are 4, 31, 22, 211, 1111,
which give weak orders 4, 3/1, 2/2, 2/1/1 and 1/2/1, 1/1/1/1
respectively
(in the obvious shorthand), 
which correspond to 000000, 000+++, 0++++0, 0+++++ and ++0+++, ++++++, 
respectively.
Then the f-level partitions are 4 (trivially);
31 and 4, corresponding to 000aaa and 000fff;
22 and 4, corresponding to 0aaaa0 and 0ffff0;
22 and 31 and 4, corresponding to 0aaaaf and 0aaffa and 0fffff;
...respectively.
}}

%}}}
%{{{ arrays \nu=4

%Here is % take 1 of
%a tabulation for Case 4.
We already gave the one-nation tabulation for $N=4$.
%Then below that
Below we give the nation-partitions 31 then 22 then 211 then 1111.
%{{{ ignore
\ignore{{
\[
\hspace{-2.1cm}
\begin{array}{|c|c|cc|cc|ccc|cccccc}
\hline
0-pt & 4 & \multicolumn{2}{c|}{31} & \multicolumn{2}{c|}{22} & \multicolumn{4}{c|}{211} & 1111 & 
\\ \hline
weak  & 4 & \multicolumn{2}{c|}{3/1} & \multicolumn{2}{c|}{2/2} &
   \multicolumn{3}{c}{2/1/1} & \multicolumn{1}{c|}{1/2/1} & 1/1/1/1 &
\\ \hline
0+ & 000000 & \multicolumn{2}{c|}{000+++}
     & \multicolumn{2}{c|}{0++++0} &
           \multicolumn{3}{c}{0+++++} & \multicolumn{1}{c|}{++0+++} & ++++++
\\ \hline
f-pt & 4 & 31 &4 &     22  & 4 & 22 & 31 & 4 & 
\\ \hline
fa & 000000 & 000aaa & 000fff &  0aaaa0 & 0ffff0
     & 0aaaaf & 0aaffa & 0fffff & 
\\
\hline
\end{array}
\]

Here is take 2:
}}
%}}}
\ignore{{ %% a better version of this is now given above %%
\[
\hspace{-1.1cm}
\begin{array}{|c|c|cc|cc|ccc|c|c|cccc}
\hline
0-pt & 4 & \multicolumn{2}{c|}{31} & \multicolumn{2}{c|}{22} & \multicolumn{4}{c|}{211} & 1111 & 
\\ \hline
weak  & 4 & \multicolumn{2}{c|}{3\ova 1} & \multicolumn{2}{c|}{2\ova 2} &
   \multicolumn{3}{c}{2\ova 1\ova 1} & \multicolumn{1}{c|}{1\ova 2\ova 1}
   & 1\ova 1\ova 1\ova 1 &
\\ \hline
0+ & 000000 & \multicolumn{2}{c|}{000+++}
     & \multicolumn{2}{c|}{0++++0} &
           \multicolumn{3}{c}{0+++++} & \multicolumn{1}{c|}{++0+++} & ++++++
\\ \hline
f-pt & 4 & 31 &4 &     22  & 4 & 22 & 31 & 4 &     22 \;\; 31\;\; 4 &  22 \;\; 31\;\; 4 &
\\ \hline
fa & 000000 &
  \multicolumn{2}{c|}{
    \begin{array}{c} 000aaa \hspace{.21in} \\ \hspace{.1in} 000fff \end{array}}
     &  \multicolumn{2}{c|}{
    \begin{array}{c} 0aaaa0 \hspace{.21in} \\  \hspace{.21in} 0ffff0 \end{array}}
     &  \multicolumn{3}{c|}{
    \begin{array}{c} 0aaaaf  \hspace{.21in} \\
                     0aaffa \\  \hspace{.21in} 0fffff \end{array}}
     & \multicolumn{1}{c|}{
    \begin{array}{c} aa0faa  \hspace{.21in} \\
                     ff0aaa \\  \hspace{.21in} ff0fff \end{array}} 
  &   \begin{array}{c} faaaaf  \hspace{.21in} \\
  fffaaa  \\  \hspace{.21in} ffffff \end{array} &  
\\
\hline
\end{array}
\]
}}

%}}}
%{{{ \nu=31


%...Next need to do the corresp 3$\off$ ones, then 4,5,6. Case 31 has 3 $\off$s.
\[
\hspace{-1.1cm}
\begin{array}{|c|c|cc|cc|ccc|c|c|cccc}
\hline
0-pt & 3|1 & \multicolumn{2}{c|}{21|1} & \multicolumn{2}{c|}{111|1}   & 
\\ \hline
weak  & 3|1 & \multicolumn{2}{c|}{2\ova 1|1 \hspace{.84in} 1\ova 2|1}
            & \multicolumn{2}{c|}{1\ova 1\ova 1|1} &
\\ \hline
0+ & 000\off\off\off & \multicolumn{2}{c|}{0++\off\off\off
                             \hspace{.4in} ++0\off\off\off}
     & \multicolumn{2}{c|}{+++\off\off\off} &
\\ \hline
f-pt & 3|1 & 21|1 \;\;\;\;\; 3|1\;\;&\;\;\;21|1\;\;\;\;\;3|1 &     21|1  & 3|1 &
\\ \hline
fa & 000\off\off\off &
  \multicolumn{2}{c|}{
    \begin{array}{c} 0aa\off\off\off \hspace{.321in} \\ \hspace{.31in} 0ff\off\off\off \end{array}
    \;\;
       \begin{array}{c} aa0\off\off\off \hspace{.321in} \\ \hspace{.31in} ff0\off\off\off \end{array}}
     &  \multicolumn{2}{c|}{
    \begin{array}{c} aaf\off\off\off \hspace{.6321in}
\\ afa\off\off\off \hspace{.6321in}
\\ faa\off\off\off \hspace{.6321in}
\\  \hspace{.421in} fff\off\off\off \end{array}}
     &  
\\
\hline
\end{array}
\]

%}}}
%{{{ 22 and 211 and 1111

The bar notation $\nu | \nu'$ indicates separation into nations.
Thus in particular  $\nu | \nu'$ and  $\nu' | \nu$ indicate
the same $\Sigma_N$-orbit.
Here if $\nu$ is simply  a partition,
written  $21$, for example, then this just
indicates the sizes of the counties.
%
On the other hand $2\ova 1|1$ indicates that the first nation has two counties,
ordered with a county of size 2 before a county of size 1.
This is not in the same $\Sigma_N$ orbit as $1\ova 2|1$.
(It is in the same $P$ orbit, but see later.)

%Case 22 has 4 $\off$s. Case $2|1|1$ has 5 $\off$s. Case 1111 ...
\[
\hspace{-1.1cm}
\begin{array}{|c|c|cc|cc||c|cc||c|ccccc}
\hline
0-pt & 2|2 & \multicolumn{2}{c|}{11|2} & \multicolumn{2}{c||}{11|11}
&
 2|1|1 & \multicolumn{2}{c||}{11 |1 |1} & 1|1|1|1 &
\\ \hline
weak  & 2|2 & \multicolumn{2}{c|}{1\ova 1|2}
      & \multicolumn{2}{c||}{1\ova 1|1\ova 1} &
2|1|1 & \multicolumn{2}{c||}{1\ova 1 | 1 | 1} &  1|1|1|1 &
\\ \hline
0+ & 0\off\off\off\off 0& \multicolumn{2}{c|}{+\off\off\off\off 0}
     & \multicolumn{2}{c||}{+\off\off\off\off +} &
     0\off\off\off\off\off & \multicolumn{2}{c||}{+\off\off\off\off\off}
     &\off\off\off\off\off\off&
\\ \hline
f-pt & 2|2 & 11|2 &2|2 &     11|11  & 2|11 \;\;\; 2|2 &
2|1|1 & 11|1|1 & 2|1|1 & 1|1|1|1&
\\ \hline
fa & 0\off\off\off\off 0&
  \multicolumn{2}{c|}{
    \begin{array}{c} a\off\off\off\off 0\hspace{.321in} \\ \hspace{.31in} f\off\off\off\off 0\end{array}}
     &  \multicolumn{2}{c||}{
    \begin{array}{c} a\off\off\off\off a \hspace{.321in} \\
  \hspace{.001in} f\off\off\off\off a \\
  \hspace{.4321in} f\off\off\off\off f
  \end{array}}
     &
     0\off\off\off\off\off &
      \multicolumn{2}{c||}{
    \begin{array}{c} a\off\off\off\off \off \hspace{.321in} \\
  \hspace{.4321in} f\off\off\off\off \off
  \end{array}}
  &\off\off\off\off\off\off&
\\
\hline
\end{array}
\]

%}}}
%{{{ more

Note that the $\Sigma_N$ action includes  moves that bodily permute
nations without changing orders within a nation.
Thus for example the orbits with weak order
$1\ova 1|2$ and $2|1\ova 1$ are the same.
And also the orbits of $f\off\off\off\off a$ and
$a\off\off\off\off f$ are the same.


\ppm{%Presumably need to fix the 31 with afa/// and faa///.   \\ And
ideally we push on a bit further below so $2/1|1/2$ appears?}

%}}}

%\inputt tex/reps-N4signature  %% used to be here. 


%\vspace{1cm}



==> tex-eric/algorithm.tex <==

\module{algorithm}

\section{Algorithm}
To produce all (generic) solutions up to X-equivalence in practice one may proceed as follows. We define $\M(\alpha,\beta)=\begin{pmatrix}\alpha+\beta& \beta\\ -\alpha&0 \end{pmatrix}$, $\D(\alpha)=\alpha\cdot Id_2$, and $\A(x)=\begin{pmatrix} 0 & x\\x& 0\end{pmatrix}$.
First, apply a permutation to ensure that all signed edges are labeled by a $+$.
\ppm{[-I don't understand. Apply to what? Do you mean all solutions up to X and perms?]}
We then partition into connected components where we delete all $/$ edges.  Since any triangle has either 0, 2 or 3 $/$-labeled edges by Lemma \ref{lem:slash} this provides a partition.  By again applying a permutation as necessary we may assume that the first $k_1$ labels are in component 1 etc.
\ppm{[-I dont understand.]}
As above call each component a \emph{nation}. Within each nation observe that any 0-labeled edges form $j$-simplices for $j\geq 2$: this follows from the fact  that any triangle has either 0, 1 or 3 $0$-labeled edges (see Lemma \ref{le:0s}(I)) . For nation $i$:
\begin{enumerate}
 \item[0.] Choose a variable $\alpha_i$.
 \item[1a.] If nation $i$ is a single vertex, set the corresponding vertex value to $\alpha_i$. Continue to nation $i+1$ or stop this subroutine if the vertex label is $N$.
 \item[1b.] If nation $i$ is not a single vertex, choose a variable $\beta_i\neq -\alpha_i$. Set each $+$ edge value to $\M(\alpha_i,\beta_i)$.
 \item[2.] For each $0$-labeled $j$-simplex (where necessarily $j\geq 2$) arbitrarily give all such edges value $\D(\alpha_i)$ or $\D(\beta_i)$.
 \item[3.] For each vertex incident to a $0$-labeled edge, assign the value as $\alpha_i$ or $\beta_i$ depending on the corresponding value $\D(\alpha_i)$ or $\D(\beta_i)$ of the $0$-labeled edge.
 \item[4.] For each vertex not incident to any $0$-labeled edge, assign value $\alpha_i$ or $\beta_i$ arbitrarily.
 \item[5.] Repeat steps [1-4] until all vertices have been assigned values (and all edges internal to a nation have been assigned values).
 \item[6.] For each pair of nations choose a variable $z_{ij}$.  For each $/$-labeled edge between nations $i$ and $j$, assign value $\A(z_{ij})$.
\end{enumerate}

While this algorithm will provide all solutions, we may also prescribe the vertex labels, which will then determine the edge values for labels $0$ and $+$.
\ppm{[I dont understand.]}

%\medskip
\subsection{On notions of equivalence of solutions} \label{ss:notionsequiv}

The follow examples illustrate some of the subtleties that arise when considering various notions of equivalence of solutions.

In terms of computational complexity,
we note that determining if two matrices are similar is  %computationally
straightforward
-- a polynomial time algorithms exist.
On the other hand, to decide if two matrices are similar via a permutation matrix is potentially harder: determining if the adjacency matrices of two graphs are permutation-similar is equivalent to the question of whether the graphs are isomorphic (see, eg. \cite[Lemma 8.1.1]{GodsilRoyle}), a problem for which no polynomial-time algorithm is currently known.  We also do not know an easy way of deciding if two $N^2\times N^2$ matrices are \emph{locally similar}, i.e. if they are similar via a matrix of the form $Q\otimes Q$.

(The most natural choice of equivalence from our perspective is the one we have given: locally permutation-similar, which we have used throughout.)

\begin{example}\label{ex:wedgevee} Let us compare the $N=3$ solutions associated with the graphs $\stackrel{\beta}{{}_\alpha\bigwedge_\alpha}$ and $\stackrel{{}^\alpha\bigvee^\alpha}{{}_\beta}$.  Since these are single nations we obtain, in our abbreviated notation:
$$R_\vee:=(\beta,\alpha,\alpha,\M(\alpha,\beta),\M(\alpha,\beta),\D(\alpha))$$
and 
$$R_\wedge:=(\alpha,\alpha,\beta,\D(\alpha),\M(\alpha,\beta),\M(\alpha,\beta)),$$ respectively.   Now clearly these two matrices are related by a permutation of rows/columns--in fact the permutation matrix $P$ associated with changing between the two Kronecker product conventions for matrices followed by a local permutation will do the trick. However, an easy (computer) calculation reveals that the are not locally similar, i.e. there is no invertible $3\times 3$ matrix $Q$ such that $(Q\otimes Q)R_\vee(Q\otimes Q)^{-1}=R_\wedge $.
\end{example}

\begin{example} Now let us consider the $N=4$ solutions associated with the graphs $\stackrel{\bigvee}{|}$ and $\stackrel{\bigwedge}{\bigvee}$.
Taking all vertex labels to be $\alpha$ we obtain:
$$R^1:=(\alpha,\alpha,\alpha,\alpha,\D(\alpha),\M(\alpha,\beta),\M(\alpha,\beta),\M(\alpha,\beta),\M(\alpha,\beta),\M(\alpha,\beta))$$ 
and $$R^2:=(\alpha,\alpha,\alpha,\alpha,\M(\alpha,\beta),\M(\alpha,\beta),\D(\alpha),\M(\alpha,\beta),\M(\alpha,\beta),\M(\alpha,\beta))$$ respectively.
One may show that $R^1$ and $R^2$, while similar as $16\times 16$ matrices, are not locally similar.  Such a global similarity transformation can be achieved by a permutation of rows/columns, (explicitly by interchanging rows/columns $2\leftrightarrow 7$ and $5\leftrightarrow 10$), but this cannot be achieved by applying the permutation matrix $P$ followed by some local permutations.
\end{example}



==> tex-eric/combinatoric.tex <==
\module{tex-eric/combinatoric}

\section{A Combinatorial Interpretation and Future Directions}













%\newcommand{\seteric}[1]{[#1]}  %% Eric's version of \set{} %%
\newcommand{\seteric}[1]{\set{#1}}  %% Eric's version of \set{} conformed %%
%%% - we need to conform these notations!  %%% DONE!

\subsection{A Combinatorial Bijection}
We produce a somewhat surprising connection between charge-conserving solutions to
the constant Yang-Baxter equation
and a combinatorial structure.  Although our proof does not rely upon this bijection, it was an inspiration for our classification scheme, so we record it here.

A \emph{hierarchy structure} on $\seteric{N} :=\{1,\ldots, N\}$
%\ppm{-standardise notation?}
is a partition $\mathcal{P}$ of $\seteric{N}$
with a weak ordering
chosen on each block $X\in \mathcal{P}$.  A weak order is a ranking of a set that allows for ties, formally we
first partition the elements and then order the partitions.

\iffalse
Here a \emph{strict} weak ordering is
%one
\ppm{a weak ordering [-define this? so far we have defined weak total order
- is it the same thing? that name can be changed as needed.]}
for which incomparability is an equivalence relation.
\fi

For a given hierarchy structure we will write $i|j$ to denote that $i$ and $j$ are in distinct blocks.  If $i,j$ are in the same block we will write $i\rightarrow j$ (equivalently, $j\leftarrow i$) if $i$ is great than $j$ in the weak ordering and $i\sim j$ if they are equivalent, i.e., neither $i\rightarrow j$ nor $j\rightarrow i$ \cite{SloaneWieder}. Thus, for each $i\neq j$ we have $i\Box j$ where $\Box$ is exactly one of $|,\sim,\rightarrow,\leftarrow$. One may think of such a structure as partitioning a population of $N$ individuals into some number of `nations' and then weakly ordering
the members of each nation.
The equivalence relation induced by $\sim$ yields a refinement
{of}
the nations into `counties'. Clearly there are exactly 4 hierarchy structures on a set of size $2$, and one can easily check explicitly that there are 23 hierarchy structures on a set of size $3$.  Moreover, one can show that verifying an assignment of $|,\sim,\rightarrow,\leftarrow$ to each pair $i<j$ is a hierarchy structure can be achieved by checking it ``locally'' i.e. on each subpopulation of size $3$, as follows:

\begin{theorem} \label{thm: 3 suffice hierarchy}
An arbitrary choice of $|,\sim,\rightarrow,\leftarrow$ for
$\Box$ in $i\Box j$ for each pair $i<j\in\seteric{N}$
is a hierarchy structure if, and only if, the restriction to each triple
$i,j,k\in \seteric{N}$ is such a structure.
\end{theorem}
\begin{proof} It is clear that restricting a hierarchy structure to any 3 individuals must remain a hierarchy structure.  To see that we have a hierarchy structure as soon as it holds for each triple $i,j,k$ we first observe that the relation induced by $i\equiv j$ if $i=j,i\sim j,i\rightarrow j$ or $j\rightarrow i$ is an equivalence relation.  The hierarchy structure on triples proves transitivity and symmetry and reflexivity are clear.  This provides a partition on
$\seteric{N}$.
Thus we may assume that the partition consists of a single set.  To show that an assignment of $i\Box j$ for each pair $i<j\in\seteric{N}$
for $\Box\in \{\sim,\rightarrow,\leftarrow\}$ is a weak ordering it is enough, by definition, to check:
 irreflexivity, asymmetry and transitivity of $\rightarrow$ and 
transitivity of $\sim$.
These are immediate for any triple, by assumption.
Since each of these postulates involve at most 3 elements we see that the weak ordering on
$\seteric{N}$
follows from the hierarchy structure on each triple
-- note that if no partition contains 3 members this is vacuously true.
\end{proof}





For a given hierarchy structure we may permute the individuals,
which
{may}
yield a different hierarchy.
Thus $\Sigma_N$ acts on the collection of hierarchy structures. For example if we have $1|2\rightarrow 3$ and interchange $1$ and $3$ we obtain $1\leftarrow 2|3$.  Another useful symmetry is that  we may  simply reverse all of the $\rightarrow$ and $\leftarrow$.  For example, $1\rightarrow 3|2\leftarrow 4$ becomes $1\leftarrow 3|2\rightarrow 4$.  We hasten to point out that this latter symmetry is not superfluous: the hierarchies $1\rightarrow 2\sim 3$ and $1\sim 2\rightarrow 3$ are not in the same $\Sigma_N$ orbits, since $i\rightarrow j\sim k$ always has one individual greater than the other two, while $i\sim j\rightarrow k$ always has one individual below the other two.  However, reversing the arrow does achieve this symmetry.

In this setting it is natural to consider symmetries where one reverses all arrows in some nations but not others.
{That is, to consider the action of flipping the nation containing $i$,
for each $i$.}
\ppm{
However, this does not seem to have a natural counterpart for charge-conserving Yang-Baxter operators (however, see Example \ref{ex:wedgevee} below, which illustrates the `reverse all arrows' ).  The only `global' symmetries are those that come from permuting the local bases and the $\mathbeef_i\otimes \mathbeef_j\rightarrow\mathbeef_j\otimes \mathbeef_i$ symmetry induced from the flip operator P in  (\ref{de:flip1}).  A symmetry that transposes, say, $ \mathbeef_1\otimes \mathbeef_2$ and $\mathbeef_2\otimes \mathbeef_1$ but not the other $\mathbeef_i\otimes \mathbeef_j$ will surely disrupt the form of some hierarchies.}


Let us define an \emph{admissible (N-)form} to be a sequence of ${\binom{N}{2}}$ abbreviated edge decorations from $\{0,/,\Up,\Do\}$ corresponding to a solution as in (\ref{pa:rec}).  Note we are ignoring the vertex decorations.
A consequence of our analysis is the following:

\begin{theorem} There is a bijection between admissible forms in $\{0,/,\Up,\Do\}^{\binom{N}{2}}$ and hierarchy structures on
$\seteric{N}$, determined by the assignments in Table \ref{bij}.
\end{theorem}
 
\begin{table}\begin{tabular}{|c|c|}\hline
decoration & $i\Box j$ \\\hline\hline
$0$ & $i\sim j$\\
\hline
$/$ & $i|j$\\
\hline
$\Up$ & $i\rightarrow j$\\
\hline
$\Do$ &$i\leftarrow j$\\
\hline

\end{tabular}\caption{Bijection on pairs $i<j$ \label{bij}}\end{table}






\begin{proof}
By Theorem \ref{thm: 3 suffice hierarchy} it is enough to show that the bijection holds for $\seteric{3} =\{1,2,3\}$.
A routine check show that the 23 forms in Table \ref{tab:1ad} correspond to these 23 hierarchy structures. For example, the admissible $3$-form $(/,\Do,/)$ yields the hierarchy structure $1\leftarrow 2|3$, while $(\Up,0,\Do)$ corresponds to $1\sim 3\rightarrow 2$.  For a non-example consider $(/,0,+)$ which would have $1|2$, $1\sim 3$ and $2\rightarrow 3$ which are incompatible.We illustrate these in Table \ref{all23} by orbits.

\begin{table}\begin{tabular}{|c|c|}\hline
$(M(1,2),M(1,3),M(2,3))$ & hierarchy on $\{i,j,k\}=\{1,2,3\}$
\\\hline\hline
$(\Up,\Up,\Up)$ orbit (size 6) & $i\rightarrow j\rightarrow k$ (permute) \\
\hline
$(/,/,\Up)$ orbit (size 6) & $i|j\rightarrow k$ (permute) \\
\hline
$(0,\Up,\Up)$ orbit (size 6) & $i\sim j\rightarrow k$ (choose $k$ and $\rightarrow/\leftarrow$)\\
\hline
$(0,/,/)$ orbit (size 3) & $i\sim j|k$ (choose $k$)\\
\hline
$(0,0,0)$ orbit (size 1) & $i\sim j\sim k$\\
\hline 
$(/,/,/)$ orbit (size 1) & $i|j|k$\\
\hline

\end{tabular}\caption{Bijection: $N=3$  forms and hierarchies\label{all23}}\end{table}
\end{proof}
\ppm{
We remark that there are only 6 admissible forms for $N=3$, while there are 10 inequivalent cases the the `9-rule' Proposition \ref{pr:N3}.  This is because including vertex labels breaks some symmetry.}



\iffalse    %%% see future.tex

\subsection{Future Directions}

Several natural questions for future study spring to mind.
\begin{enumerate}
\item 
The Andruskiewitsch-Schneider classification program for pointed Hopf algebras takes as input a solution $(R,V)$ to the YBE to produce Nichols algebras which can potentially be lifted via bosonization. The $4\times 4$ solutions were addressed \cite{AndruskGiraldi2018}. Do our solutions lead to finite-dimensional Nichols algebras?
\item
One of our original motivations was to construct representations of the loop braid group \cite{DamianiMartinRowell}.
Which of our solutions lift to loop braided vector spaces \cite{kadar2016local}?
%\ppm{-is that a thing?}
\item Turaev \cite{Turaev1988} developed a method for constructing link invariants from solutions to the Yang-Baxter equation. Of course the well-known $4\times 4$ $R$-matrix associated with the $U_q\mathfrak{sl}_2$ provide link invariants (essentially the Jones polynomial), and many of our solutions generalize these solutions so we certainly expect interesting invariants.
\item
It is noteworthy that the verification of a $N^2\times N^2$ solution comes down to verifying  constraints on $2$-indexed scalars for all $3$-element subsets.  This bears some similarity to the verification of associativity in a monoidal category: it is sufficient by Mac Lane coherence \cite{MacLane} to verify constraints involving $4$-indices on scalars with 3 indices.  This suggests a higher category connection, see \cite{KapVoev}.
\item
Also natural is the question of generalisations to other targets besides $\Match^N$,
for example generalised 8-vertex model
(in the sense of \cite{Hietarinta:1992}) instead of the 6-vertex model.
\end{enumerate}

\fi



\iffalse


\begin{enumerate}
\item Suppose that each of the $A_{i,j}$ matrices have a zero on the off-diagonal. There are \emph{a priori} $8$ possibilities corresponding to whether the left or right coordinates of $(b,c),(p,j)$ and $(s,m)$ is zero.   After applying the symmetries above, we find that there are two orbits of these choices and we may assume that $b=p=0$.  Thus there are two cases to consider coming from $sm=0$.  These lead to constant solutions.
\item Suppose that none of the $A_{i,j}$ matrices have a zero on the off-diagonal.  Similarly as above, we may assume that $a=r=0$.  There are two cases to consider, coming from $kv=0$.
\item Suppose that exactly two of the $A_{i,j}$ have a zero entry on the off-diagonal.  We may assume it is the first two.  Further computations will show that this gives no solutions.
\item If exactly one of the $A_{i,j}$ has an off-diagonal zero entry, we may assume it is $A(1,2)$.  Moreover, we may further assume that $b=0$. This gives $4$ cases, depending on $kv=0$ and $hr=0$.
\end{enumerate}

\fi


















\iffalse
For the $(0,*,*)$ case we follow a similar approach. The $(0,\Up,\Up)$ form implies that $a_{8,8}=a_{7,7}=a_{4,2}=a_{2,4}=0$ while $a_{3,3}$ and $a_{6,6}$ are non-zero.  The Gr\"obner basis algorithm yields the following polynomial consequences:

\begin{eqnarray} &&a_{{8,8}},a_{{7,7}},a_{{4,4}}-a_{{5,5}},a_{{4,2}},a_{{3,3}}-a_{{6,6}}
,\\&&a_{{2,4}},a_{{2,2}}-a_{{5,5}},a_{{1,1}}-a_{{5,5}},a_{{6,6}}a_{{9,9}}+
a_{{6,8}}a_{{8,6}}-{a_{{9,9}}}^{2},\\&&a_{{3,7}}a_{{7,3}}+a_{{6,6}}a_{{9,9
}}-{a_{{9,9}}}^{2}, \left( a_{{5,5}}-a_{{9,9}} \right)  \left( a_{{5,5
}}-a_{{6,6}}+a_{{9,9}} \right)\end{eqnarray}
The resulting 2 families of solutions are:

$$\left[ \begin {array}{ccccccccc} a_{{5,5}}&0&0&0&0&0&0&0&0
\\ \noalign{\medskip}0&a_{{5,5}}&0&0&0&0&0&0&0\\ \noalign{\medskip}0&0
&\alpha+\beta&0&0&0&-{\frac {\beta\,\alpha}{a_{{7,3}}}}&0&0
\\ \noalign{\medskip}0&0&0&a_{{5,5}}&0&0&0&0&0\\ \noalign{\medskip}0&0
&0&0&a_{{5,5}}&0&0&0&0\\ \noalign{\medskip}0&0&0&0&0&\alpha+\beta&0&-{
\frac {\beta\,\alpha}{a_{{8,6}}}}&0\\ \noalign{\medskip}0&0&a_{{7,3}}&0
&0&0&0&0&0\\ \noalign{\medskip}0&0&0&0&0&a_{{8,6}}&0&0&0
\\ \noalign{\medskip}0&0&0&0&0&0&0&0&\beta\end {array} \right]
$$ where $a_{5,5}\in\{\alpha,\beta\}$.
 


The $(0,/,/)$ case yields the following constraints:

\begin{eqnarray}&&a_{{8,8}},a_{{7,7}},a_{{6,6}},a_{{4,4}}-a_{{5,5}},\\&&a_{{4,2}},a_{{3,3}}
,a_{{2,4}},a_{{2,2}}-a_{{5,5}},a_{{1,1}}-a_{{5,5}},\\&&a_{{3,7}}a_{{7,3}}-
a_{{6,8}}a_{{8,6}}\end{eqnarray}

This gives a single family of solutions:

$$ \left[ \begin {array}{ccccccccc} a_{{5,5}}&0&0&0&0&0&0&0&0
\\ \noalign{\medskip}0&a_{{5,5}}&0&0&0&0&0&0&0\\ \noalign{\medskip}0&0
&0&0&0&0&{\frac {a_{{6,8}}a_{{8,6}}}{a_{{7,3}}}}&0&0
\\ \noalign{\medskip}0&0&0&a_{{5,5}}&0&0&0&0&0\\ \noalign{\medskip}0&0
&0&0&a_{{5,5}}&0&0&0&0\\ \noalign{\medskip}0&0&0&0&0&0&0&a_{{6,8}}&0
\\ \noalign{\medskip}0&0&a_{{7,3}}&0&0&0&0&0&0\\ \noalign{\medskip}0&0
&0&0&0&a_{{8,6}}&0&0&0\\ \noalign{\medskip}0&0&0&0&0&0&0&0&a_{{9,9}}
\end {array} \right]
$$

\fi
\iffalse
\begin{eqnarray}&&
a_{{8,8}},a_{{7,7}},a_{{4,4}},a_{{3,3}},a_{{2,2}},\\&&a_{{6,6}}a_{{9,9}}+
a_{{6,8}}a_{{8,6}}-{a_{{9,9}}}^{2}, \left( a_{{5,5}}-a_{{9,9}}
 \right)  \left( a_{{5,5}}-a_{{6,6}}+a_{{9,9}} \right) ,\\&&a_{{2,4}}a_{{4
,2}}-a_{{3,7}}a_{{7,3}}
\end{eqnarray}

This yields the following two families of solutions:
$$ \left[ \begin {array}{ccccccccc} \tau&0&0&0&0&0&0&0&0
\\ \noalign{\medskip}0&0&0&\delta&0&0&0&0&0\\ \noalign{\medskip}0&0&0&0
&0&0&\eta&0&0\\ \noalign{\medskip}0&{\frac {\eta\,\xi}{\delta}}&0&0&0&0
&0&0&0\\ \noalign{\medskip}0&0&0&0&a_{{5,5}}&0&0&0&0
\\ \noalign{\medskip}0&0&0&0&0&\alpha+\beta&0&\gamma&0
\\ \noalign{\medskip}0&0&\xi&0&0&0&0&0&0\\ \noalign{\medskip}0&0&0&0&0
&-{\frac {\alpha\,\beta}{\gamma}}&0&0&0\\ \noalign{\medskip}0&0&0&0&0&0
&0&0&\beta\end {array} \right]
$$
where $a_{5,5}\in\{\alpha,\beta\}$.  The eigenvalues of $R$ are $ \tau,
\alpha,\pm\sqrt {\eta\,\xi},
\beta$, so that, generically, there are 5 distinct such.


The same approach for the remaining three families of forms for $(*,*,*)$ do not yield any solutions: the Gr\"obner basis algorithm returns an empty variety.
\fi
\appendix

\section{Algorithm}
To produce all (generic) solutions up to X-equivalence in practice one may proceed as follows. We define $\M(\alpha,\beta)=\begin{pmatrix}\alpha+\beta& \beta\\ -\alpha&0 \end{pmatrix}$, $\D(\alpha)=\alpha\cdot Id_2$, and $\A(x)=\begin{pmatrix} 0 & x\\x& 0\end{pmatrix}$.
First, apply a permutation to ensure that all signed edges are labeled by a $+$.  We then partition into connected components where we delete all $/$ edges.  Since any triangle has either 0, 2 or 3 $/$-labeled edges by Lemma \ref{lem:slash} this provides a partition.  By again applying a permutation as necessary we may assume that the first $k_1$ labels are in component 1 etc.  As above call each component a \emph{nation}. Within each nation observe that any 0-labeled edges form $j$-simplices for $j\geq 2$: this follows from the fact  that any triangle has either 0, 1 or 3 $0$-labeled edges (see Lemma \ref{le:0s}(I)) . For nation $i$:
\begin{enumerate}
 \item[0.] Choose a variable $\alpha_i$.
 \item[1a.] If nation $i$ is a single vertex, set the corresponding vertex value to $\alpha_i$. Continue to nation $i+1$ or stop this subroutine if the vertex label is $N$.
 \item[1b.] If nation $i$ is not a single vertex, choose a variable $\beta_i\neq -\alpha_i$. Set each $+$ edge value to $\M(\alpha_i,\beta_i)$.
 \item[2.] For each $0$-labeled $j$-simplex (where necessarily $j\geq 2$) arbitrarily give all such edges value $\D(\alpha_i)$ or $\D(\beta_i)$.
 \item[3.] For each vertex incident to a $0$-labeled edge, assign the value as $\alpha_i$ or $\beta_i$ depending on the corresponding value $\D(\alpha_i)$ or $\D(\beta_i)$ of the $0$-labeled edge.
 \item[4.] For each vertex not incident to any $0$-labeled edge, assign value $\alpha_i$ or $\beta_i$ arbitrarily.
 \item[5.] Repeat steps [1-4] until all vertices have been assigned values (and all edges internal to a nation have been assigned values).
 \item[6.] For each pair of nations choose a variable $z_{ij}$.  For each $/$-labeled edge between nations $i$ and $j$, assign value $\A(z_{ij})$.
\end{enumerate}

While this algorithm will provide all solutions, we may also prescribe the vertex labels, which will then determine the edge values for labels $0$ and $+$.
The follow examples illustrate some of the subtleties that arise when considering various notions of equivalence of solutions.  We note that determining if two matrices are similar is computationally straightforward--a polynomial time algorithms exist.  On the other hand, to decide if two matrices are similar via a permutation matrix is potentially harder: determining if the adjacency matrices of two graphs are permutation-similar is equivalent to the question of whether the graphs are isomorphic (see, eg. \cite[Lemma 8.1.1]{GodsilRoyle}), a problem for which no polynomial-time algorithm is currently known.  We also do not know an easy way of deciding if two $N^2\times N^2$ matrices are \emph{locally similar}, i.e. if they are similar via a matrix of the form $Q\otimes Q$.  The most natural choice of equivalence from our perspective is the one we have given: locally permutation-similar, which we have used throughout.
\begin{example}\label{ex:wedgevee} Let us compare the $N=3$ solutions associated with the graphs $\stackrel{\beta}{{}_\alpha\bigwedge_\alpha}$ and $\stackrel{{}^\alpha\bigvee^\alpha}{{}_\beta}$.  Since these are single nations we obtain, in our abbreviated notation:
$$R_\vee:=(\beta,\alpha,\alpha,\M(\alpha,\beta),\M(\alpha,\beta),\D(\alpha))$$
and 
$$R_\wedge:=(\alpha,\alpha,\beta,\D(\alpha),\M(\alpha,\beta),\M(\alpha,\beta)),$$ respectively.   Now clearly these two matrices are related by a permutation of rows/columns--in fact the permutation matrix $P$ associated with changing between the two Kronecker product conventions for matrices followed by a local permutation will do the trick. However, an easy (computer) calculation reveals that the are not locally similar, i.e. there is no invertible $3\times 3$ matrix $Q$ such that $(Q\otimes Q)R_\vee(Q\otimes Q)^{-1}=R_\wedge $.
\end{example}

\begin{example} Now let us consider the $N=4$ solutions associated with the graphs $\stackrel{\bigvee}{|}$ and $\stackrel{\bigwedge}{\bigvee}$.
Taking all vertex labels to be $\alpha$ we obtain:
$$R^1:=(\alpha,\alpha,\alpha,\alpha,\D(\alpha),\M(\alpha,\beta),\M(\alpha,\beta),\M(\alpha,\beta),\M(\alpha,\beta),\M(\alpha,\beta))$$ 
and $$R^2:=(\alpha,\alpha,\alpha,\alpha,\M(\alpha,\beta),\M(\alpha,\beta),\D(\alpha),\M(\alpha,\beta),\M(\alpha,\beta),\M(\alpha,\beta))$$ respectively.
One may show that $R^1$ and $R^2$, while similar as $16\times 16$ matrices, are not locally similar.  Such a global similarity transformation can be achieved by a permutation of rows/columns, (explicitly by interchanging rows/columns $2\leftrightarrow 7$ and $5\leftrightarrow 10$), but this cannot be achieved by applying the permutation matrix $P$ followed by some local permutations.
\end{example}


==> tex-eric/intro-eric-old.tex <==

\module{tex-eric/intro-eric}



\section{Introduction }
\newcommand{\Aut}{\mathrm{Aut}}
\newcommand{\uN}{\underline{N}}

Classification of braid representations \cite{Birman} is a major open problem ---
except that it is impossibly wild.
For applications, conceding this impossibility is not an acceptable outcome.
So we  % need
seek a framework for a paradigm change.
{Clues for this can be found, for example, in}
higher representation theory
(works such as
\cite{MazorchukMiemietz14,RumyninWendland,KapVoev,DamianiMartinRowell}
and many others);
%\cite{KapVoev}.
and in higher lattice gauge theory (works such as
\cite{MartinsPicken11,Pfeiffer,baez_schreiber}
and %many
many others).
Armed with such ideas, %amongst others,
we are indeed able to
make a paradigm change that yields 
%provide
a \sout{solution} \ppm{breakthrough}.\ppm{Tone it down? \emph{some solutions}?}
\ppm{[ppm: hmm. I don't think any of these work. I see the possible problem,
but I probably prefer the original. How about:]
a solution for monoidal functors to a suitable target category.}

\newcommand{\nNn}{N}  %% N   not n 

One %\sout{source} 
{formulation} \ppm{family? Not all reps come this way...}
of such braid representations is invertible solutions to the
constant ({also known as} quantum)
%\ppm{-what do the brackets signify?}
Yang-Baxter equation (YBE), i.e., $R\in \mathrm{Aut}(V^{\otimes 2})$ satisfying
\[ R_1\otimes R_2\otimes R_1=R_2\otimes R_1\otimes R_2
\]
where $R_1=R\otimes I_V$ and $R_2=I_V\otimes R$
and $V=\C^\nNn$
\cite{Baxter,Jimbo86}.
 This YBE has been a well-spring of deep and beautiful mathematics from its origins in Baxter's approach to finding exactly solvable models in statistical mechanics and Yang's construction of 2-dimensional quantum field theories \cite{Yang67}, to Drinfeld and Jimbo's \cite{drinfeld,Jimbo86} discovery
%
of quantum groups and the field of quantum topology generalizing Jones' celebrated polynomial link invariant \cite{Jones85} in the 1980s.
 Formally the $\nNn$-dimensional YBE is a  system of $\nNn^6$
 cubic polynomial equations in $\nNn^4$ variables--a formidable problem in symbolic computation for even modest values of
 $\nNn$.
 Indeed, while a classification of the solutions $(R,\mathbb{C}^2)$ for $\nNn=2$ have been known for almost 30 years \cite{Hietarinta:1992} the cases
 $\nNn\geq 3$
 remain wide open. Finding and classifying Yang-Baxter operators (YBOs) 
 %$R\in\mathrm{Aut}(V^{\otimes 2})$
  remain important classical problems with myriad applications.

An alternative strategy
%\ppm{-alternative to what? symbolic computation?}
to classifying solutions by incrementing the dimension is to seek to generalise the forms of the solutions for
$\nNn=2$. Generalising the permutation-matrix solutions are the important set-theoretical solutions described in \cite{Etingof99}.
For another example we can point to the isolated solution
$\begin{pmatrix} 1 & 0&0&1\\ 0& 1 & 1& 0\\
0& -1 & 1& 0\\ -1 & 0&0&1\end{pmatrix}$ which can be naturally generalised to every dimension as the so-called Gaussian solutions \cite{GoldschmidtJones:1989,RowellWang:2010}.   Of course there is some ambiguity in the interpretation of how we generalize, and we should employ available symmetries such as local basis changes to reduce the complexity of the problem and the solution description.

\newcommand{\mathbeef}{\mathfrak{e}}  %% hook for basis els

Recently with Damiani \cite{DamianiMartinRowell} we were led to consider $4\times 4$ spin-chain representations of the braid group,
\ppm{in particular, with only limited basis change symmetry},
in our study of certain finite dimensional quotients of
the loop braid group {algebra}.
The matrices we encountered have the same form as the 
universal $R$-matrix for the quantum supergroup $U_q\mathfrak{sl}_{1|1}$. A salient feature these YBOs share with the $U_q\mathfrak{sl}_2$ $R$-matrix is that they are \emph{charge conserving} in the sense that the subspaces spanned by tensor products of standard basis vectors
$\mathbeef_i\otimes \mathbeef_j$ and $\mathbeef_j\otimes \mathbeef_i$ are invariant under $R$ (here for $i,j\in\{1,2\}$),
i.e. of the general form $\begin{pmatrix} a_1& 0&0 & 0\\
0 & a_{12} & b_{12} &0\\
0 & c_{12} & d_{12} &0\\
0&0&0& a_2
\end{pmatrix}$.
This suggests that an appropriate higher dimensional generalization of these
$4\times 4$ solutions should be
$\nNn^2\times \nNn^2$ charge conserving solutions to the YBE.  



In this article we \sout{completely}
classify charge conserving YBOs up to symmetries \ppm{[-what does this mean?]}.
\sout{This}
\ppm{The problem?}
is first framed in terms of monoidal functors $F$ from the braid category $\Bcat$ to the category $\Match^N$ of $N^2\times N^2$ charge conserving matrices.  The automorphisms in this target category confer symmetries upon the space of solutions, represented as images of the monoidal generator $\sigma$ of the category $\Bcat$ under $F$.  We then characterize all such functors in terms of polynomial constraints.  Taken in tandem, these symmetries and constraints yield a blueprint for a complete classification.  The description of all solutions is facilitated by a remarkably simple combinatorial encoding of a transversal of the orbits of all solutions under the action of the group of symmetries.  

The tractability of the problem is a consequence of special
\ppm{`miracles'}
that do not apply universally to YBOs, principally:
\begin{enumerate}
\item[(a)] Lemma \ref{lem:3 suffice}: An operator $R\in \Aut(V^{\otimes 2})$ is a charge conserving YBO if, and only if, the restriction $R^{ijk}$ of $R$ to the subspace of $V^{\otimes 2}$ spanned by tensor products of $3$ basis vectors $\mathbeef_i,\mathbeef_j,\mathbeef_k$ is also a charge conserving YBO, for all triples $\{i,j,k\}$.
\item[(b)] $X$-symmetry
\ref{?}:
Conjugation of a charge conserving YBO $R$ by \emph{any} diagonal matrix $X\in\Aut(V^{\otimes 2})$ again yields a a charge conserving YBO.
\item[(c)] Restricted Symmetry
\ref{?}:
\ppm{Note that}
General local basis changes of the form $R\mapsto (Q\otimes Q)R(Q\otimes Q)^{-1}$ \emph{do not} preserve charge conjugation.
\ppm{However,}
Together with $X$-symmetry it is enough
\ppm{[-enough in order to achieve what?]}
to consider the simultaneous basis permutation action of $\Sigma_N$.
\end{enumerate}
The upshot of (a) is that it suffices to first find all solutions with $N=3$ and then
\ppm{figure out how to}
glue them together, while (b) and (c) provide
\sout{the} symmetries that reduce the complexity of the problem.
\ppm{[-the two parts of this sentence seem to have a very different flavour?
Not sure I understand it yet.]}

Our combinatorial description of solutions begins with an encoding of general charge conserving operator $T\in\Aut(V^{\otimes 2})$ as $N$ scalars $a_i$ associated with the $1$-dimensional spaces $\C\mathbeef_i\otimes\mathbeef_i$ and ${N\choose 2}$ $2\times 2$ matrices $A(i,j)$ associated with the $2$ dimensional spaces spanned by $\mathbeef_i\otimes \mathbeef_j$ and $\mathbeef_j\otimes \mathbeef_i$ for $i<j$.  This can be conveniently visualised as a directed complete graph $K_N$ on $N$ vertices, with the vertices decorated with the $a_i$ and the edges by $A(i,j)$.  


Next, we \ppm{briefly} describe versions of the combinatorial objects to which we associate solutions.
(In order to
\ppm{work with and}
\sout{properly} count the solutions we will use a \sout{slightly} more refined construction in the main text.)
Let $\underline{N}:=\{1,\ldots, N\}$ be a set of $N$ individuals.
We construct a \sout{multi}set
of bi-colored generalized
\ppm{[-or skew?]}
Young tableaux from $\underline{N}$ as follows:
\begin{enumerate}
\item First partition $\uN$ into $m$ `nations' $n_1,\ldots,n_m$ respecting the natural order on $\uN$, so that $1,\ldots,|n_1|$ lie in $n_1$;
\ppm{$|n_1|+1,\ldots,|n_1|+|n_2|$ lie in $n_2$,} 
etc.
\item Next partition each nation $n_i$ into $\ell_i$ `counties' $c_{i,1},\ldots, c_{i,\ell_1}$, again respecting the natural ordering on individuals.  
\item Finally,
\ppm{[-if the target is tableau then this step is not final?]}
color each county white or blue, such that the first county in each nation is always white.
\end{enumerate}
Each nation can be visualised as a bi-colored generalized Young tableau with the counties stacked on top of each other.   Here is an example of a full configuration for $N=11$:

%%% The way the following was set broke left-justification in the document!
%%% Is it ok now?
%%% (We could just use  \[ ... \]  )
\begin{centering}

%\centering
\includegraphics[width=3.7cm]{xfig/tree012ex10bbb1XI.eps}


\end{centering}

For each nation $n_i$ fix two non-zero parameters $\alpha_i,\beta_i$ such that $\alpha_i+\beta_i\neq 0$, and for each pair of nations $n_i,n_k$ fix a non-zero parameter $\mu_{ij}$.  To describe a solution it is enough to specify the scalars $a_1,\ldots,a_N$ and matrices $A(j,k)$, which depend on the relationship between the counties/nations that individuals $i<j$ reside in, as well as the color of their respective counties.  Specifically:

\begin{enumerate}
\item If $i$
\ppm{[-maybe, if possible, separate out a bit the variable names used for nations and individuals?]}
resides in county $c_{k,s}$ then if the county is red,
\ppm{white?}
$a_i=\alpha_k$ otherwise $a_i=\beta_k$.
\item If $i$ is in nation $n_k$ and $j$ is in nation $n_t$ then $A(i,j)=\begin{pmatrix} 0 & \mu_{k,t}\\ \mu_{k,t} &0\end{pmatrix}$.
\item If $i$ and $j$ are in the same nation $n_k$ but different counties $c_{k,x}$ and $c_{k,y}$ (here we have $x<y$ by construction), then $A(i,j)=\begin{pmatrix} \alpha_k+\beta_k & \beta_k\\ -\alpha_k & 0\end{pmatrix}$
\item If $i$ and $j$ are in the same county $c_{k,s}$ then
$A(i,j)=\begin{pmatrix} x_k &0\\0&x_k\end{pmatrix} $
\ppm{[something not quite right?]}
where $x=\alpha_k$ if $c_{k,s}$ is white and $x=\beta_k$ otherwise.
\end{enumerate}
Our main results imply that matrices so constructed are indeed charge conserving YBOs and any charge conserving YBO may be transformed to a solution of this form by means of the symmetries (b) and (c) described above.

Here is a more
\ppm{less?}
detailed description of the contents of this paper.
In section \ref{ss:braid} we describe the braid category.
\sout{, and in}
In
section \ref{ss:target} we focus on functors to the target category $\Match^N$
\ppm{considered representation theoretically,}
\ppm{[to contradistinguish with the generalist perspective above]}
and set up our approach to the main theorem, including the $N=2$ case.
The main Theorem \ref{th:mainx} is found in section  \ref{ss:main} which includes a detailed description of the classification in terms of our combinatorial encoding.
Section \ref{section: first steps?? key?} contains a sequence of lemmas covering the crucial $N=3$, which are then applied in section \ref{ss:proofend} to finish the proof of the main theorem.  We close with a brief discussion of some future directions in the last section.



%Here is a more detailed description of the paper.  

\noindent 
{\bf{Acknowledgements}.}
We thank Lizzy Rowell for the braid laboratory.
We thank Celeste Damiani
for useful conversations.
PM thanks Paula Martin and Nicola Gambino %and Fiona Torzewska
for useful conversations. The research of ECR was partially supported by the US NSF grant DMS-1664359.

\medskip






==> tex-eric/intro-eric.tex <==

\module{tex-eric/intro-eric}



\section{Introduction }
\newcommand{\Aut}{\mathrm{Aut}}
\newcommand{\uN}{\underline{N}}

Classification of braid representations \cite{Birman} is a major open problem ---
except that it is impossibly wild.
For applications, conceding this impossibility is not an acceptable outcome.
So we  % need
seek a framework for a paradigm change.
{Clues for this can be found, for example, in}
higher representation theory
(works such as
\cite{MazorchukMiemietz14,RumyninWendland,KapVoev,DamianiMartinRowell}
and many others);
%\cite{KapVoev}.
and in higher lattice gauge theory (works such as
\cite{MartinsPicken11,Pfeiffer,baez_schreiber}
and %many
many others).
Armed with such ideas, %amongst others,
we are indeed able to
make a paradigm change that yields 
%provide
a solution for monoidal functors to a suitable target category.

\newcommand{\nNn}{N}  %% N   not n 

One %\sout{source} 
\ppm{natural formulation of a suitable target category
[I think I am not understanding this wording yet. The YBE does not itself lead to Match
does it? I think it says at most that things are monoidal, but we have already said that.
So I might lean towards reverting this wording to how it was?]
comes from}
\sout{of such braid representations is} invertible solutions to the
constant ({also known as} quantum)
%\ppm{-what do the brackets signify?}
Yang-Baxter equation (YBE), i.e., $R\in \mathrm{Aut}(V^{\otimes 2})$ satisfying
\[ R_1R_2 R_1=R_2 R_1 R_2
\]
where $R_1=R\otimes I_V$ and $R_2=I_V\otimes R$
and $V=\C^\nNn$
\cite{Baxter,Jimbo86}.
\ppm{[-by the way, if we refer to categories in this para then it might be best to
say what $\otimes$ means? - just in the sense that using the word raises the level
of formality a notch.]}
 This YBE has been a well-spring of deep and beautiful mathematics from its origins in Baxter's approach to finding exactly solvable models in statistical mechanics and Yang's construction of 2-dimensional quantum field theories \cite{Yang67}, to Drinfeld and Jimbo's \cite{drinfeld,Jimbo86} discovery
%
of quantum groups and the field of quantum topology generalising Jones' celebrated polynomial link invariant \cite{Jones85} in the 1980s.
 Formally the $\nNn$-dimensional YBE is a  system of $\nNn^6$
 cubic polynomial equations in $\nNn^4$ variables--a formidable problem in symbolic computation for even modest values of
 $\nNn$.
 Indeed, while a classification of the solutions $(R,\mathbb{C}^2)$ for $\nNn=2$ have been known for almost 30 years \cite{Hietarinta:1992} the cases
 $\nNn\geq 3$
 remain wide open. Finding and classifying Yang-Baxter operators (YBOs) 
 %$R\in\mathrm{Aut}(V^{\otimes 2})$
  remain important classical problems with myriad applications.

An alternative strategy
%\ppm{-alternative to what? symbolic computation?}
to classifying solutions by incrementing the dimension is to seek to generalise the forms of the solutions for
$\nNn=2$. Generalising the permutation-matrix solutions are the important set-theoretical solutions described in \cite{Etingof99}.
For another example we can point to the isolated solution
$\begin{pmatrix} 1 & 0&0&1\\ 0& 1 & 1& 0\\
0& -1 & 1& 0\\ -1 & 0&0&1\end{pmatrix}$ which can be naturally generalised to every dimension as the so-called Gaussian solutions \cite{GoldschmidtJones:1989,RowellWang:2010}.   Of course there is some ambiguity in the interpretation of how we generalize, and we should employ available symmetries such as local basis changes to reduce the complexity of the problem and the solution description.

\newcommand{\mathbeef}{\mathfrak{e}}  %% hook for basis els

Recently with Damiani \cite{DamianiMartinRowell} we were led to consider $4\times 4$ spin-chain representations of the braid group,
{in particular, with only limited basis change symmetry},
in our study of certain finite dimensional quotients of
the loop braid group {algebra}.
The matrices we encountered have the same form as the 
universal $R$-matrix for the quantum supergroup $U_q\mathfrak{sl}_{1|1}$. A salient feature these YBOs share with the $U_q\mathfrak{sl}_2$ $R$-matrix is that they are \emph{charge conserving} in the sense that the subspaces spanned by tensor products of standard basis vectors
$\mathbeef_i\otimes \mathbeef_j$ and $\mathbeef_j\otimes \mathbeef_i$ are invariant under $R$ (here for $i,j\in\{1,2\}$),
i.e. of the general form $\begin{pmatrix} a_1& 0&0 & 0\\
0 & a_{12} & b_{12} &0\\
0 & c_{12} & d_{12} &0\\
0&0&0& a_2
\end{pmatrix}$.
This suggests that an appropriate higher dimensional generalization of these
$4\times 4$ solutions should be
$\nNn^2\times \nNn^2$ charge conserving solutions to the YBE.  



In this article we
classify charge conserving YBOs.
The problem
is first framed in terms of monoidal functors $F$ from the braid category $\Bcat$ to the category $\Match^N$ of $N^2\times N^2$ charge conserving matrices.  The automorphisms in this target category confer symmetries upon the space of solutions, represented as images of the monoidal generator $\sigma$ of the category $\Bcat$ under $F$.  We then characterize all such functors in terms of polynomial constraints.  Taken in tandem, these symmetries and constraints yield a blueprint for a complete classification.  The description of all solutions is facilitated by a remarkably simple combinatorial encoding of a transversal of the orbits of all solutions under the action of the group of symmetries.  

The tractability of the problem is a consequence of special
{`miracles'}
that do not apply universally to YBOs, principally:
\begin{enumerate}
\item[(a)] Lemma \ref{lem:3 suffice}: An operator $R\in \Aut(V^{\otimes 2})$ is a charge conserving YBO if, and only if, the restriction $R^{ijk}$ of $R$ to the subspace of $V^{\otimes 2}$ spanned by tensor products of $3$ basis vectors $\mathbeef_i,\mathbeef_j,\mathbeef_k$ is also a charge conserving YBO, for all triples $\{i,j,k\}$.
\item[(b)] $X$-symmetry, Lemma
\ref{lem:Xeq}:
Conjugation of a charge conserving YBO $R$ by \emph{any} diagonal matrix $X\in\Aut(V^{\otimes 2})$ again yields a a charge conserving YBO.
\item[(c)] Restricted Symmetry, Lemma 
\ref{lem:chacon1}:
Note that
general local basis changes of the form
$R\mapsto (Q\otimes Q)R(Q\otimes Q)^{-1}$
\emph{do not} preserve charge
\ppm{conservation}. %conjugation.
Together with $X$-symmetry, the simultaneous basis permutation action of $\Sigma_N$ yields all local basis changes that preserve charge conservation.
\end{enumerate}
The upshot of (a) is that it suffices to first find all solutions with $N=3$ and then
figure out how to
glue them together for $N>3$.  Statements (b) and (c) provide enough
symmetries to organise the cases and ultimately gain purchase on the $N=3$ case.
\ppm{[-the two parts of this sentence seem to have a very different flavour?
Not sure I understand it yet.]}

Our combinatorial description of solutions begins with an encoding of general charge conserving operator $T\in\Aut(V^{\otimes 2})$ as $N$ scalars $a_i$ associated with the $1$-dimensional spaces $\C\mathbeef_i\otimes\mathbeef_i$ and ${N\choose 2}$ $2\times 2$ matrices $A(i,j)$ associated with the $2$ dimensional spaces spanned by $\mathbeef_i\otimes \mathbeef_j$ and $\mathbeef_j\otimes \mathbeef_i$ for $i<j$.  This can be conveniently visualised as a directed complete graph $K_N$ on $N$ vertices, with the vertices decorated with the $a_i$ and the edges by $A(i,j)$.  


Next, we {briefly} describe versions of the combinatorial objects to which we associate solutions.
(In order to
{work with and}
 count the solutions we will use a more refined construction in the main text.)
Let $\underline{N}:=\{1,\ldots, N\}$ be a set of $N$ individuals.
We construct a set
of bi-coloured \ppm{skew [?]}
Young tableaux from $\underline{N}$ as follows:
\begin{enumerate}
\item First partition $\uN$ into $m$ `nations' $n_1,\ldots,n_m$ respecting the natural order on $\uN$, so that $1,\ldots,|n_1|$ lie in $n_1$;
{$|n_1|+1,\ldots,|n_1|+|n_2|$ lie in $n_2$,} 
etc.
\item Next partition each nation $n_s$ into $\ell_s$ `counties' $c_{s,1},\ldots, c_{s,\ell_s}$, again respecting the natural ordering on individuals. 
\item Next,
\ppm{[-if the target is tableau then this step is not final?]}
color each county white or blue, such that the first county in each nation is always white.
\item Finally observe that each nation can be visualised as a bi-coloured skew Young tableau with the counties stacked on top of each other,
and the collection
\ppm{of?}
nations is our set of bicoloured skew Young tableaux.
\end{enumerate}
  Here is an example of a full configuration for $N=11$:

%%% The way the following was set broke left-justification in the document!
%%% Is it ok now?
%%% (We could just use  \[ ... \]  )
\begin{centering}

%\centering
\includegraphics[width=3.7cm]{xfig/tree012ex10bbb1XI.eps}


\end{centering}

For each nation $n_s$ fix two non-zero parameters $\alpha_s,\beta_s$ such that $\alpha_s+\beta_s\neq 0$, and for each pair of nations $n_s,n_t$ with $s<t$ fix a non-zero parameter $\mu_{s,t}$.  To describe a solution it is enough to specify the scalars $a_1,\ldots,a_N$ and matrices $A(i,j)$, which depend on the relationship between the counties/nations that individuals $i<j$ reside in, as well as the color of their respective counties.  Specifically:

\begin{enumerate}
\item If $i$
\ppm{[-maybe, if possible, separate out a bit the variable names used for nations and individuals?]}
resides in county $c_{s,z}$ (which is in nation $n_s$) then if the county is 
{white}
$a_i=\alpha_s$ otherwise $a_i=\beta_s$.
\item If $i$ is in nation $n_s$ and $j$ is in nation $n_t$ with $s\neq t$ then $A(i,j)=\begin{pmatrix} 0 & \mu_{s,t}\\ \mu_{s,t} &0\end{pmatrix}$.
\item If $i$ and $j$ are in the same nation $n_s$ but different counties $c_{s,x}$ and $c_{s,y}$ (here we have $x<y$ by construction), then $A(i,j)=\begin{pmatrix} \alpha_s+\beta_s & \beta_s\\ -\alpha_s & 0\end{pmatrix}$
\item If $i$ and $j$ are in the same county $c_{s,z}$ then
$A(i,j)=\begin{pmatrix} x_s &0\\0&x_s\end{pmatrix} $
\ppm{[something not quite right?]}
where $x_s=\alpha_s$ if $c_{s,z}$ is white and $x_s=\beta_s$ otherwise.
\end{enumerate}
Our main results imply that matrices so constructed are indeed charge conserving YBOs and any charge conserving YBO may be transformed to a solution of this form by means of the symmetries (b) and (c) described above.  In particular we obtain a count of orbits of
\ppm{varieties of}
solutions by rank as $1, 4, 13, 46, 154,\ldots$ which is precisely sequence A104460 in \cite{sloane1}.

Here is a summary of the contents of this paper.
In section \ref{ss:braid} we describe the braid category.

In
section \ref{ss:target} we focus on functors to the target category $\Match^N$
\ppm{considered representation theoretically,}
\ppm{[to contradistinguish with the generalist perspective above]}
and set up our approach to the main theorem, including the $N=2$ case.
The main Theorem \ref{th:mainx} is found in section  \ref{ss:main} which includes a detailed description of the classification in terms of our combinatorial encoding.
Section \ref{section: the proof} contains a sequence of lemmas covering the crucial $N=3$ case, which are then applied in section \ref{ss:proofend} to finish the proof of the main theorem.  We close with a brief discussion of some future directions in the last section.



%Here is a more detailed description of the paper.  

\noindent 
{\bf{Acknowledgements}.}
We thank Lizzy Rowell for the braid laboratory.
We thank Celeste Damiani
for useful conversations.
PM thanks Paula Martin and Nicola Gambino %and Fiona Torzewska
for useful conversations. The research of ECR was partially supported by the US NSF grant DMS-1664359.

\medskip






==> tex-eric/intro-ericp.tex <==

\module{tex-eric/intro-eric}



\section{Introduction }
\newcommand{\Aut}{\mathrm{Aut}}
\newcommand{\uN}{\underline{N}}

Classification of braid representations \cite{Birman} is a major open problem ---
except that it is impossibly wild.
For applications, conceding this impossibility is not an acceptable outcome.
So we  % need
seek a framework for a paradigm change.
{Clues for this can be found, for example, in}
higher representation theory
(works such as
\cite{MazorchukMiemietz14,RumyninWendland,KapVoev,DamianiMartinRowell}
and many others);
%\cite{KapVoev}.
and in higher lattice gauge theory (works such as
\cite{MartinsPicken11,Pfeiffer,baez_schreiber}
and %many
many others).
Armed with such ideas, %amongst others,
we are indeed able to
make a paradigm change that yields 
%provide
a solution for monoidal functors to a suitable target category.

\newcommand{\nNn}{N}  %% N   not n 

One %\sout{source} 
formulation
\ppmx{natural formulation of a suitable target category
[I think I am not understanding this wording yet. The YBE does not itself lead to Match
does it? I think it says at most that things are monoidal, but we have already said that.
So I might lean towards reverting this wording to how it was?]
comes from}% 
{exemplifying  %of
such braid representations is given by}
invertible solutions to the
constant ({also known as} quantum)
%\ppm{-what do the brackets signify?}
Yang-Baxter equation (YBE), i.e., $R\in \mathrm{Aut}(V^{\otimes 2})$ satisfying
\[ R_1R_2 R_1=R_2 R_1 R_2
\]
where $R_1=R\otimes I_V$ and $R_2=I_V\otimes R$
and $V=\C^\nNn$
\cite{Baxter,Jimbo86}.
\ppmx{[-by the way, if we refer to categories in this para then it might be best to
say what $\otimes$ means? - just in the sense that using the word raises the level
of formality a notch.]}
 This YBE has been a well-spring of deep and beautiful mathematics from its origins in Baxter's approach to finding exactly solvable models in statistical mechanics and Yang's construction of 2-dimensional quantum field theories \cite{Yang67}, to Drinfeld and Jimbo's \cite{drinfeld,Jimbo86} discovery
%
of quantum groups and the field of quantum topology generalising Jones' celebrated polynomial link invariant \cite{Jones85} in the 1980s.
 Formally the $\nNn$-dimensional YBE is a  system of $\nNn^6$
 cubic polynomial equations in $\nNn^4$ variables--a formidable problem in symbolic computation for even modest values of
 $\nNn$.
 Indeed, while a classification of the solutions $(R,\mathbb{C}^2)$ for $\nNn=2$ have been known for almost 30 years \cite{Hietarinta:1992} the cases
 $\nNn\geq 3$
 remain wide open. Finding and classifying Yang-Baxter operators (YBOs) 
 %$R\in\mathrm{Aut}(V^{\otimes 2})$
  remain important classical problems with myriad applications.

An alternative strategy
%\ppm{-alternative to what? symbolic computation?}
to classifying solutions by incrementing the dimension is to seek to generalize the forms of the solutions for
$\nNn=2$. Generalising the permutation-matrix solutions are the  %important
set-theoretical solutions described
for instance
in \cite{Etingof99}.
For another example we can point to the isolated solution
$\begin{pmatrix} 1 & 0&0&1\\ 0& 1 & 1& 0\\
0& -1 & 1& 0\\ -1 & 0&0&1\end{pmatrix}$ which can be naturally generalised to every dimension as the so-called Gaussian solutions \cite{GoldschmidtJones:1989,RowellWang:2010}.   Of course there is some ambiguity in the interpretation of how we generalize, and we should employ available symmetries such as local basis changes to reduce the complexity of the problem and the solution description.

\newcommand{\mathbeef}{\mathfrak{e}}  %% hook for basis els

Recently with Damiani \cite{DamianiMartinRowell} we were led to consider $4\times 4$ spin-chain representations of the braid group,
{in particular, with only limited basis change symmetry},
in our study of certain finite dimensional quotients of
the loop braid group {algebra}.
The matrices we encountered have the same form as the 
universal $R$-matrix for the quantum supergroup $U_q\mathfrak{sl}_{1|1}$. A salient feature these YBOs share with the $U_q\mathfrak{sl}_2$ $R$-matrix is that they are \emph{charge conserving} in the sense that the subspaces spanned by tensor products of standard basis vectors
$\mathbeef_i\otimes \mathbeef_j$ and $\mathbeef_j\otimes \mathbeef_i$ are invariant under $R$ (here for $i,j\in\{1,2\}$),
i.e. of the general form $\begin{pmatrix} a_1& 0&0 & 0\\
0 & a_{12} & b_{12} &0\\
0 & c_{12} & d_{12} &0\\
0&0&0& a_2
\end{pmatrix}$.
This suggests that an appropriate higher dimensional generalization of these
$4\times 4$ solutions should be
$\nNn^2\times \nNn^2$ charge conserving solutions to the YBE.  



In this article we
classify charge conserving YBOs.
The problem
is first framed in terms of monoidal functors $F$ from the braid category $\Bcat$ to
%the
a category $\Match^N$   of  % $N^2\times N^2$
charge conserving matrices.  The automorphisms in this target category confer symmetries upon the space of solutions, represented as images of the monoidal generator $\sigma$ of the category $\Bcat$ under $F$.  We then characterize all such functors in terms of polynomial constraints.  Taken in tandem, these symmetries and constraints yield a blueprint for a complete classification.  The description of all solutions is facilitated by a remarkably simple combinatorial encoding of a transversal of the orbits of all solutions under the action of the group of symmetries.  

The tractability of the problem is a consequence of special
{`miracles'}
that do not apply universally to YBOs, principally:
\begin{enumerate}
\item[(a)] Lemma \ref{lem:3 suffice}: An operator $R\in \Aut(V^{\otimes 2})$ is a charge conserving YBO if, and only if, the restriction $R^{ijk}$ of $R$ to the subspace of $V^{\otimes 2}$ spanned by tensor products of $3$ basis vectors $\mathbeef_i,\mathbeef_j,\mathbeef_k$ is also a charge conserving YBO, for all triples $\{i,j,k\}$.
\item[(b)] $X$-symmetry, Lemma
\ref{lem:Xeq}:
Conjugation of a charge conserving YBO $R$ by \emph{any} diagonal matrix $X\in\Aut(V^{\otimes 2})$ again yields a  charge conserving YBO.
\item[(c)] Restricted Symmetry, Lemma 
\ref{lem:chacon1}:
Note that
general local basis changes of the form
$R\mapsto (Q\otimes Q)R(Q\otimes Q)^{-1}$
\emph{do not} preserve charge
conservation. %conjugation.
Together with $X$-symmetry, the simultaneous basis permutation action of $\Sigma_N$ yields all local basis changes that preserve charge conservation.
\end{enumerate}
The upshot of (a) is that it suffices to first find all solutions with $N=3$ and then
figure out how to
glue them together for $N>3$.  Statements (b) and (c) provide enough
symmetries to organise the cases and ultimately gain purchase on the $N=3$ case.
\ppmx{[-the two parts of this sentence seem to have a very different flavour?
Not sure I understand it yet.]}

Our combinatorial description of solutions begins with an encoding of general charge conserving operator $T\in\Aut(V^{\otimes 2})$ as $N$ scalars $a_i$ associated with the $1$-dimensional spaces $\C\mathbeef_i\otimes\mathbeef_i$ and ${N\choose 2}$ $2\times 2$ matrices $A(i,j)$ associated with the $2$ dimensional spaces spanned by $\mathbeef_i\otimes \mathbeef_j$ and $\mathbeef_j\otimes \mathbeef_i$ for $i<j$.  This can be conveniently visualised as a directed complete graph $K_N$ on $N$ vertices, with the vertices decorated with the $a_i$ and the edges by $A(i,j)$.  


Next, we {briefly} describe versions of the combinatorial objects to which we associate solutions.
(In order to
{work with and}
 count the solutions we will use a more refined construction in the main text.)
Let $\underline{N}:=\{1,\ldots, N\}$ be a set of $N$ individuals.
We construct a set
of bi-coloured
{\em composition tableaux}  %skew Young tableaux
from $\underline{N}$ as follows:
\begin{enumerate}
\item First partition $\uN$ into $m$ `nations' $n_1,\ldots,n_m$ respecting the natural order on $\uN$, so that $1,\ldots,|n_1|$ lie in $n_1$;
{$|n_1|+1,\ldots,|n_1|+|n_2|$ lie in $n_2$,} 
etc.
\item Next partition each nation $n_s$ into $\ell_s$ `counties' $c_{s,1},\ldots, c_{s,\ell_s}$, again respecting the natural ordering on individuals. 
\item Next,
\ppmx{[-if the target is tableau then this step is not final?]}%
colour  %each county white or
a subset of counties blue,
such that the first county in each nation is always
uncoloured.  %white.
\item Finally observe that each nation can be visualised as a
bi-coloured
{composition tableau}
%skew Young tableau
with the counties stacked on top of each other,
and the collection of nations is our set of bicoloured
%skew Young tableaux.
{composition tableaux}.
\end{enumerate}
  Here is an example of a full configuration for $N=11$:

%%% The way the following was set broke left-justification in the document!
%%% Is it ok now?
%%% (We could just use  \[ ... \]  )
\begin{centering}

%\centering
\includegraphics[width=3.7cm]{xfig/tree012ex10bbb1XI.eps}


\end{centering}

For each nation $n_s$ fix two non-zero parameters $\alpha_s,\beta_s$ such that $\alpha_s+\beta_s\neq 0$, and for each pair of nations $n_s,n_t$ with $s<t$ fix a non-zero parameter $\mu_{s,t}$.  To describe a solution it is enough to specify the scalars $a_1,\ldots,a_N$ and matrices $A(i,j)$, which depend on the relationship between the counties/nations that individuals $i<j$ reside in, as well as the colour of their respective counties.
Specifically:

\begin{enumerate}
\item If $i$
\ppmx{[-maybe, if possible, separate out a bit the variable names used for nations and individuals?]}
resides in county $c_{s,z}$ (which is in nation $n_s$) then if the county is 
uncoloured %{white}
$a_i=\alpha_s$ otherwise $a_i=\beta_s$.
\item If $i$ is in nation $n_s$ and $j$ is in nation $n_t$ with $s\neq t$ then $A(i,j)=\begin{pmatrix} 0 & \mu_{s,t}\\ \mu_{s,t} &0\end{pmatrix}$.
\item If $i$ and $j$ are in the same nation $n_s$ but different counties $c_{s,x}$ and $c_{s,y}$ (here we have $x<y$ by construction),
then $A(i,j)=\begin{pmatrix} \alpha_s+\beta_s & \beta_s\\ -\alpha_s & 0\end{pmatrix}$.
\item If $i$ and $j$ are in the same county $c_{s,z}$ then
$A(i,j)=\begin{pmatrix} x_s &0\\0&x_s\end{pmatrix} $
\ppmx{[something not quite right?]}
where $x_s=\alpha_s$ if $c_{s,z}$ is
uncoloured  %white
and $x_s=\beta_s$
if blue.  %otherwise.
\end{enumerate}
Our main results imply that matrices so constructed are indeed charge conserving YBOs and any charge conserving YBO may be transformed to a solution of this form by means of the symmetries (b) and (c) described above.  In particular we obtain a count of orbits of
varieties of 
solutions by rank as $1, 4, 13, 46, 154,\ldots$ which,
pleasingly,
is  precisely
sequence A104460 in \cite{sloane1}.

\medskip

Here is a summary of the contents of this paper.
In section \ref{ss:braid} we describe the braid category.
%
In
section \ref{ss:target} we focus on functors to the target category $\Match^N$
{considered representation theoretically,}
\ppmx{[to contradistinguish with the generalist perspective above]}
and set up our approach to the main theorem, including the $N=2$ case.
The main Theorem \ref{th:mainx} is found in section  \ref{ss:main} which includes a detailed description of the classification in terms of our combinatorial encoding.
Section \ref{section: the proof} contains a sequence of lemmas covering the crucial $N=3$ case, which are then applied in section \ref{ss:proofend} to finish the proof of the main theorem.
We close with a brief discussion of some future directions in the last section.
(Appendices \ref{ss:repthy},\ref{ss:Xeqa}
briefly discuss various intriguing points raised by,
but not internal to, this work.
Appendices \ref{ss:deets},\ref{ss:figs} contain further details on
various aspects treated with brevity in the main text.) 


%Here is a more detailed description of the paper.  

\noindent 
{\bf{Acknowledgements}.}
We thank Lizzy Rowell for the braid laboratory.
We thank Celeste Damiani
for useful conversations.
PM thanks Paula Martin and Nicola Gambino %and Fiona Torzewska
for useful conversations. The research of ECR was partially supported by the US NSF grant DMS-1664359.

\medskip






==> tex/abstractV1orig.tex <==

\module{abstract}

\begin{abstract}


A braid representation is a monoidal functor from the braid category $\Braid$.
Given a monoidal category $\mathsf{C}$,
a rank-$N$ \cc\ representation,
%(or {\em spin-chain} representation)
or {\em spin-chain} representation,
is a monoidal functor from
$\mathsf{C}$  %some monoidal category
to the category $\Match^N$ of rank-$N$ \cc\ matrices
(see %\S\ref{todo}
below
for definition).
In this work we construct all
  spin-chain braid representations,
and classify up to suitable notions of isomorphism.
%up to isomorphism.


\end{abstract}



==> tex/abstractV2.tex <==

\module{abstractV2}

%{{{ ABSTRACT
%\newcommand{\KMRW}{Kadar-Martin-Rowell-Wang:2016}  % bib rationalisation
\begin{abstract}


In this work we construct and completely classify all
  spin-chain braid representations, that is, charge conserving solutions to the constant Yang-Baxter equation.
Here a braid representation is a monoidal functor from the braid category $\Braid$.
Given a monoidal category $\mathsf{C}$,
a rank-$N$ \cc\ representation,
%(or {\em spin-chain} representation)
or {\em spin-chain} representation,
is a monoidal functor from
$\mathsf{C}$  %some monoidal category
to the category $\Match^N$ of rank-$N$ \cc\ matrices
(see %\S\ref{todo}
below
for definition).
A description of the symmetries is facilitated by this categorical perspective and yields a complete characterisation of the solutions.
%up to isomorphism.


\end{abstract}
%}}}



==> tex/braid-theorem.tex <==
% $Id: intro.tex,v 1.1 $
\module{braid-theorem}

\section{Constructions for the main Theorem}
%{{{ Aside

\beff{On classification theorems}{{
    
\subsection{ %    \xxx{%Aside.
      How to read  the classification  %following
      Theorem~\ref{th:mainx}:
      } $\;$ 
      
      An example of a classification theorem
  is of course Young's classification of
  irreducible representations of the symmetric group over $\C$.
  Here one says that {\em irreducible} representations may be classified
  up to {\em isomorphism} by the set of {\em integer partitions}
  (a set that is relatively well-understood).
  Each of the three aspects of this formulation flags  challenges that we
  must address in our problem.

Firstly, %And finally,
  analogously
to the integer partitions
we will need to introduce  %notation for
some %further relatively-straightforward
  combinatorial structures.
  (Our Theorem also gives a {\em construction}.
  We will introduce notation for this too.)


Secondly,
group/algebra representations form an additive category
in a natural way.
The category property yields a `good' notion of isomorphism.
The additive property
simultaneously implies that there are unboundedly many
classes of representations,
but also that these can be effectively
classified by classifying their additive components.
%
%Secondly, %  Firstly,
%  the natural notion of homomorphism of representations in the group/algebra setting
%contains a natural notion of isomorphism.
There is no canonical lift of these properties to the monoidal category setting
(confer for example \cite{MazorchukMiemietz16,MazorchukMiemietz14,RumyninWendland,KapVoev}),
so our lift  % will
sheds new light on this aspect of higher representation theory.

And finally, %Secondly,
  treated individually symmetric group algebras over algebraically closed
  fields are Artinian, so the Jordan--Holder property tells us that every
  representation has a decomposition series with irreducible factors.
  Indeed in the complex case the decomposition multiplicities characterise a
  representation up to isomorphism.
  There is no canonical lift of this property to monoidal categories
either
(roughly since decomposition series are additive decompositions,
  while the monoidal structure is multiplicative).
  This is one of the places where the rigidity of the $\Match^N$
  target categories
  saves the day --- we will be able to classify {\em all} representations directly.


%Secondly

  

}}

%\newpage

\medskip

%}}}
%{{{ notation preamble


\befff{Classification: Notation}{{

    %Here
    Next
    we construct two sets for each $N\in \N$.
    One is the set $\SSS_N$ to which we may apply an
    algorithm (given below) to construct all varieties of solutions.
    The other gives a transversal of this set under the $\Sigma_N$ action
    from (\ref{restriction-and-symmetries})
    (and frames the effect of the $\Zz_2$ action),
    thus addressing the classification up to isomorphism.
}}

%}}}
\subsection{Notation for index sets} $\;$ 
%{{{ notation

%% promoted to macros.tex
%\newcommand{\modelss}{\models^{\!\!\!\!\!\circ}} 
%\newcommand{\gaml}{\gamma^l} 
%\newcommand{\gamr}{\gamma^r} 

%\beff{Notation}{{ We will need some notation.}}

\beff{Integer partitions and compositions}{{


  We write $\Lambda_N$ for the set of integer partitions of $N$.
  We may write $\lambda \vdash N$ for $\lambda\in \Lambda_N$. 


\mdef
We write $\Gamma_N$ for the set of compositions of $N$.
  For a composition (or partitition)
  $\lambda=(\lambda_1, \lambda_2, ..., \lambda_L)$
  we sometimes write
  $\lambda=\lambda_1 \lambda_2 \cdots\lambda_L$
or %  and sometimes write
$\lambda=\lambda_1 +\lambda_2 +\cdots+ \lambda_L$.
\\
Note that there is a lexicographic order on $\Gamma_N$.
For example
$\Gamma_2 = \{ 11, 2 \}$ and
$\Gamma_3 = \{ 111, 12, 21, 3 \}$ are written in the lex order.


\mdef
  If $\lambda=\lambda_1 \lambda_2 \cdots \lambda_L$ is a composition then we write
  $\Gamma_\lambda$ for the set
  \[
\Gamma_\lambda = \times_{i=1}^{L} \Gamma_{\lambda_i}
\]
Example: $\Gamma_{22} = \{ (11,11), (11,2), (2,11), (2,2) \}$.
We may write $\mu \models \lambda$ for $\mu \in \Gamma_{\lambda}$. 
\\
If $\lambda$ is a partition
we write $\Gamma'_\lambda$ for the subset of $\Gamma_\lambda$ 
of multicompositions $\mu$
such that if there are parts of $\lambda$ of tied order then
their compositions appear in $\mu$ in (weak) lex order.
\\
Example $\Gamma'_{22} = \{  (11,11), (11,2), (2,2) \}$.
We may write $\mu \modelss \lambda$ for $\mu \in \Gamma'_{\lambda}$. 


\medskip

%\newcommand{\gaml}{\gamma^l} 
%\newcommand{\gamr}{\gamma^r} 

\mdef \label{de:laml1}
Let $\lambda=\lambda_1 \lambda_2 \cdots \lambda_L \in \Gamma_N$
be a non-empty composition.
We define
$$
\gaml(\lambda) =\lambda_1 \lambda_2 \cdots (\lambda_L+1)
$$
and
 $\gamr(\lambda) =\lambda_1 \lambda_2 \cdots \lambda_L 1$.
Observe that both
$\gaml$ and $\gamr$
define injective functions from $\Gamma_N$ to  $\Gamma_{N+1}$,
and that $\gaml(\Gamma_N) \cap \gamr(\Gamma_N) = \emptyset$.
Thus in particular
\[
| \Gamma_N | = 2^{N-1}
\]
and the orders of all $\Gamma_\lambda$s follow.

}}

%}}}
\medskip
%{{{ notation set partitions

\beff{Set partitions}{{

\mdef
  Given a set $S$ we will write $\PP(S)$ for the set of partitions;
  and $\PP_2(S)$ for the set of partitions into at most 2 parts.
  If $N \in \N$ then $\PP(N) = \PP(\ul{N})$.

``Children-first order'':
  Given a partition $p$ of $\{ 1,2,...,N \}$
  (or any subset thereof),
we will order the parts according to their lowest numbered element;
and write $p_i$ for the $i$th such part.


\mdef
A refinement of set partition $p$ is a further partition of the parts of
$p$ into possibly smaller parts.
We will write $p<q$ (or $q>p$) if $q$ is a refinement of $p$.
\\
We may write $q|p_i$ for the restriction of $q$ to the partition of $p_i$.


\newcommand{\PPu}{\PP^u}
\newcommand{\PPm}{\PP^{-}}

\mdef
Note that there  are natural bijections between the following sets:
\\
$\{ (p,q) \; | \; p,q \in \PP(S), p<q \}$,  $\;\;$
$\{ (q,p) \; | \; p,q \in \PP(S), p<q \}$,  $\;\;$
\\
$ \{ (q,p') \; | \; q \in \PP(S), \; p' \in \PP(q) \}$
and
$$
%\PP(\PP(S))
\PPu(S) =
 \bigcup_{q \in \PP(S)} \PP(q) = 
 \{ p' \; |  \; p' \in \PP(q), \; \mbox{for some } q \in \PP(S) \}
$$
%and $ \{ (q,p') \; | \; q \in \PP(S), \; p' \in \PP(q) \}$.
 \\
 The map from first to second is simply to flip the pair.
 The map from second to third uses that $p<q$ has elements that are unions of
 parts from $q$, so we obtain a $p'$ by partitioning $q$ according to this data.
 Finally
 given $p' \in \PP(q)$ we can recover $q$ by taking the union over parts,
 so the $q$ is redundant.
 That is we can map $(q,p') \mapsto p'$.
 
 %To see this
 Note that $\PP$ has a kind of inverse $\PPm$ that takes an element of
any $\PP(S)$ and forms the union, thus restoring $S$
(caveat: this construction does not play well with the convention that
the result of a function applied to a subset of the domain is the set of images,
since here it may not be clear if an argument is a subset of the domain or an
element of it).
\\
Example:
%$$ \PP(\PP(\{1,2\})) = \PP(\{ \{\{1,2\}\}, \{ \{1\},\{2\}\} \}) $$
$$
\PPu(\{1,2\})=
\PP(\{ \{1,2\}\}) \cup \PP(\{ \{1\},\{2\}\})
  = \{ \{\{\{1,2\}\}\}, \{\{ \{1\},\{2\}\}\}, \{ \{\{1\}\},\{\{2\}\}\} \}
$$
  

\ignore{{
Sequences of form $(p,q,r,...)$ with $p<q<r<...$
(any length of sequence, $l$)
are sometimes called ramified partitions.
}}


\mdef
  Given a  %partition $q$
  finite set $S$ then 
  $Perm(S)$ %  $Perm(q)$
  is the set of total orders of the  %parts
  elements, i.e.
%  $Perm(q) = Hom^{iso}(q,\ul{|q|})$,
  $Perm(S) = Hom^{iso}(S,\ul{|S|})$,
  the set of isomorphisms
  (although we express elements simply by giving the order).
%(with equal length parts indistinguishable). 
  %%^ really not sure what this means now!
%\\ \whisper{ -should give an example in case $S$ is $q$, a set partition,...}
\\
If $p<q$ as above
then $Perm_p(q)$ means to total order the elements of $q$ in each $p_i$ without
imposing an overall total order:
$$
Perm_p(q) = %\prod_{i=1}^{|p|}
            \prod_{p_i \in p}  Perm(q|p_i)
$$ %\\
Example:
$$
Perm_{ \{ \{1\},\{2,3\}\}}( \{ \{1\},\{2\},\{3\}\}) =
\{  \{ (\{1\}),(\{2\},\{3\}) \} , \{ (\{1\}),(\{3\},\{2\}) \} \}
$$ 

}}

%}}}
%{{{ set to int notation


\beff{Notation}{{

\mdef
Given an integer partition, or indeed a composition,
$\lambda = (\lambda_1, \lambda_2, ..., \lambda_m )$ of $N$
we have a partition of
$\ul{N} = \{1,2,...,N \}$ into
`nations':
$$
\ppp(\lambda) = \{
\{ 1,2,...,\lambda_1 \},
\{ \lambda_1 +1, \lambda_1 +2, ..., \lambda_1 + \lambda_2 \},
\hspace{1.65in}$$ $$\hspace{.65in}
\{ \lambda_1  + \lambda_2+1, \lambda_1  + \lambda_2+2, ..., \lambda_1  + \lambda_2+ \lambda_3 \},
...,
\{ %\lambda_1 +\lambda_2 +...+\lambda_{m-1}+1
\left(\sum_{i=1}^{m-1} \lambda_i \right)+1
, ..., N \}\}
$$


\mdef
Given a set partition $p$ of a set $S$ of order $N$ we write $|p|$ for the integer partition
of $N$ given by the orders of the parts of $p$.
\\
(NB This does not require $S$ to be ordered.
If $S$ is ordered, then we may also extract
a {\em composition} $||p||$.) 

}}


%}}}
\subsection{Constructions for solutions} $\;$ 
%{{{ SSS_N pic
\beff{Classification: first schematic}{{

\mdef
For $N \in \N$:
\[
\SSS_N =
\{ (p,q,\rho, s) \; | \; p<q \in \PP(N);\; \rho\in Perm_p(q); \; s \in \PP_2(q)   \}
\]
%
We call the partition $p$ a partition into `nations';
and refinement $q$ a partition into `counties'.
Schematically
(neglecting only $s$ for now)
elements
of $\SSS_N$ 
can be depicted:
    \[
    \includegraphics[width=2.52\ccm]{xfig/reg10gon7.eps}
\hspace{.71\ccm}    \leadsto
%    \raisebox{-1\ccm}{   \includegraphics[width=4.9\ccm]{xfig/SN2.eps}   }
 %   \hspace{-1\ccm}
     \hspace{.41\ccm}
%     \raisebox{-1\ccm}{   \includegraphics[width=7.9\ccm]{xfig/SN3cc.eps} }
     \raisebox{-1\ccm}{   \includegraphics[width=7.9\ccm]{xfig/SN3ccc.eps} }
\]
This example has $N=10$
(here we will use $X$ as symbol for vertex 10).
In the schematic the separation of vertices indicates $p$, thus
\\
$p= \{ \{\{ 1,2,3,4,5\},\{6,7,8,9\}, \{X\}\}$.
The coloured bars indicate $q$, thus
\\
$q=\{\{ 1,2 \},\{3,4\},\{5\}, \{6,7\}, \{8,9\}, \{X\}\}$.
And from the numbering
\\
$Perm_p(q) = \{ (\{ 1,2 \},\{5\},\{3,4\}),( \{8,9\},\{6,7\}),( \{X\})
\}$.
%Formally $Perm(q)$ totally orders $q$ but, as we will see next,
%for us only the induced orders within each $p_i$ will play a role.

%}}}
%{{{ \SSS_2

\newcommand{\ovb}{\overbrace}

\mdef
Example:
\\ $
\SSS_2 = \{ \;
(\; \ovb{\{\{1,2\}\}}^p, \; \ovb{\{\{ 1,2 \}\}}^q, \;\;\; \ovb{(\{1,2\})}^\rho ,
 \;\;\; \ovb{\{\{1,2\}\}}^s ),
$\\ $ { } \hspace{1.3\ccm}
(\; \{\{1,2\}\}, \{\{ 1\},\{2 \}\}, (\{1\},\{2\}), \{\{1,2\}\}), \;
$ \\ $ { } \hspace{1.3\ccm}
(\; \{\{1,2\}\}, \{\{ 1\},\{2 \}\}, (\{2\},\{1\}), \{\{1,2\}\}), \;
$ \\ $ { } \hspace{1.3\ccm}
(\; \{\{1,2\}\}, \{\{ 1\},\{2 \}\}, (\{1\},\{2\}), \{\{1\},\{2\}\}), \;
$ \\ $ { } \hspace{1.3\ccm}
(\; \{\{1,2\}\}, \{\{ 1\},\{2 \}\}, (\{2\},\{1\}), \{\{1\},\{2\}\}),
$ \\ $ { } \hspace{1.3\ccm}
(\{\{1\},\{2\}\}, \{\{ 1\},\{2 \}\}, (\{1\},\{2\}), \{\{1\},\{2\}\})
\}
$
\\
For the enumeration we first vary over `nation' partitions
$P(2) = \{ \{ \{1,2\}\}, \{\{1\},\{2\}\} \}$. 
For the single-nation $p =  \{ \{1,2\}\} $
cases we then have two possible refinements into counties,
again given by $P(2)$.
Here each county partition has two total orders; and there are two possible $s$
partitions.
Finally we have
an element with 
two nations, each a singleton so the other components are forced
(at least once we work with $Perm_p(q)$).

\medskip
The rest of our exposition %the talk
  amounts to showing $\SSS_N$ yields an index scheme for all
varieties of 
representations.

}}

%}}}
%{{{ X-lemma before thm

\ppmx{done: promote X-Lemma here. (but proof must remain after nec Theorem)}

\mdef {\bf{Lemma}}. \label{lem:Xeq} (X Lemma)
{\em
Let $\FF:\Bcat\rightarrow\Match^N$ be a braid representation, hence given by
$\FF(\sigma)$.
Let $X$ be a diagonal invertible matrix in $\Match^N(2,2)$.
Then $\FF'(\sigma)= X \FF(\sigma) X^{-1}$ also gives a representation.

\newcommand{\simm}{\stackrel{-}{\sim}}

Consider the relation $\FF\simm\FF'$
if there exists any such diagonal invertible $X$
relating $\FF$ and $\FF'$ as above.
This is an equivalence relation.
%and then we say that $\FF$ and $\FF'$ are X-equivalent.
}

\medskip

{
\newcommand{\simm}{\stackrel{-}{\sim}}

%We call this
The relation $\simm$ is here called {\em X-equivalence}.
}

\medskip

\newcommand{\mum}[1]{\mu^{(#1)}} 
\newcommand{\mumm}[1]{\overline{\mu}^{(#1)}}
\newcommand{\FFS}{F(\sigma)}  %% R-matrix

\noindent
We state the X Lemma here because we need the notation.
The analogue of this Lemma in classical representation theory is
stronger, and is elementary. Here in the monoidal setting it is not elementary.
The proof is in \S\ref{section: the proof}.
We note that general solutions to the Yang-Baxter equation are
not stable under conjugation by diagonal matrices.
\ppm{--- Meaning that a solution
$F: \Bcat \rightarrow \Mat^N$
given in the form $F(\sigma)$ is not
necessarily taken to another solution unless $X=\mu\otimes\mu$
(i.e. $F=\cC^\mu$).}
However, since diagonal matrices are charge conserving, the set of
charge conserving matrices is stable under conjugation by diagonal matrices.
\ppm{[-so what? I think we need to say a bit more here?
the condition is something like the following, right?
(I am just going to temporarily give this a bit of room to breath.
I guess we'll delete it all again once we are done.)
Formally a conjugating functor associates a suitable invertible matrix
$\mum{m}$ to each object $m$, and transforms morphism according to:
$f \mapsto \mum{s(f)} f \mumm{t(f)}$, where $s,t$ are the source and tail
functions.
This obviously behaves well under category composition (so gives a functor),
but not necessarily under monoidal composition (so does not give a monoidal
functor in general).
A necessary condition is that it acts on the whiskerings of
$\FFS \in \Match^N(2,2)$
like
$\mum{3} \FFS\otimes 1 \mumm{3} = \mum{2} \FFS \mumm{2} \otimes 1 $
and
$\mum{3} 1\otimes \FFS \mumm{3} = 1\otimes \mum{2} \FFS \mumm{2} $.
This of course holds if $\mum{m} = \mu^{\otimes m}$ as before - the `local' solution;
but we are looking for something more.
The question is if this can be made to work with some degree of generality,
or if the only possibilities arise when we pass all the way to the constraints
coming from the YBE.
...]}
Explicitly, taking the  in-line form as in (\ref{eq:alconv1})
\[
\alpha(A) =
(a_1, a_2, \ldots, a_N, \mat{cc} a_{12} & b_{12} \\ c_{12} & d_{12} \tam,\ldots),\] conjugation by an invertible diagonal matrix defined by 
$X(\e_i\otimes \e_j)=y_{ij}(\e_i\otimes \e_j)$ gives
\[
\alpha( XAX^{-1} ) =
(a_1, a_2, \ldots, a_N, \mat{cc} a_{12} &x_{12}b_{12} \\ c_{12}/x_{12} & d_{12} \tam,\ldots)
\]
%\ppm{-need $\alpha$ in some way?}
where $x_{ij}:=\frac{y_{ij}}{y_{ji}}$ for $i<j$.  From this and the X Lemma we see that we may simultaneously and independently rescale the off-diagonal entries $(b_{ij},c_{ij})$ of each of the $2\times 2$ matrices to any pair of the form $(xb_{ij},c_{ij}/x)$.
\medskip


%}}}
\inputt reps-N2
\moduler{braid} 
%{{{ recipe

\newcommand{\vi}{v}
\newcommand{\vj}{w}
\newcommand{\offmat}{\mat{cc} 0&1\\1&0\tam}
\newcommand{\omat}{\mat{cc} 1&0\\0&1\tam}
\newcommand{\Rec}{{\mathsf R}}     %% recipe function
%\newcommand{\Cpq}{\C^{(p,q,\rho,s)}}
\newcommand{\Cpq}{\C^{(p,q)}}
\newcommand{\germ}{\SSS^\C}
\newcommand{\Cx}{\C^{\times}} 


\befs{20}{Recipe for solutions from $\SSS_N$}{{

\ignore{{
%And now to reiterate:

\mdef
    For $N \in \N$:
\[
\SSS_N =
\{ (p,q,\rho, s) \; | \; p<q \in \PP(N);\; \rho\in Perm(q); \; s \in \PP_2(q)   \}
\]
}}

\mdef
Given   $(p,q,\rho,s) \in \SSS_N$,
we call the parts of $p$ `nations' and order/number as above.
Consider the complete graph $K_p$ on the ordered set $p$.
We associate
a variable  $\mu_{ij}$ to each edge, i.e. to each pair  %of notations
$p_i, p_j \in p$ with $i<j$;
and a  variable $\alpha_i$ to each vertex $p_i$;
and a  variable $ \beta_i $ to each vertex
$p_i \in p$
containing more than one part of $q$.

The {\em type-space}
$\Cpq$
of  $(p,q,\rho,s) \in \SSS_N$ is the space whose elements
give an evaluation of each variable to an element of $\Cx$,
a nonzero complex number, such that $\beta_i \neq -\alpha_i$.
\ignore{{
thus each $\mu_{ij} \map
consist of a nonzero
complex number $\mu_{ij}$ for each distinct pair  %of notations
$p_i, p_j \in p$;
and a  nonzero complex number $\alpha_i$ for each $p_i$,
and a  nonzero complex number $ \beta_i \neq -\alpha_i$ for each
$p_i \in p$
containing more than one part of $q$.
}}
That is the complex space of variables excluding only the variety
$\prod_{ij} \mu_{ij} \prod_i \alpha_i \beta_i (\alpha_i +\beta_i)$. 
\\
A {\em germ} is a pair consisting of an element   $(p,q,\rho,s) \in \SSS_N$
and and element from $\Cpq$.
Write $\germ_N$ for the set of germs.


\mdef \label{pa:rec}
The recipe
\[
%\Rec: \SSS_N \rightarrow \Match^N(2,2)
\Rec: \germ_N \rightarrow \Match^N(2,2)
\]
for constructing  % a variety of solutions (or rather of
elements of $\Match^N(2,2)$ (that we shall prove later are all solutions)
from $(p,q,\rho,s) \in \SSS_N$ is as follows.
\\
\ignore{{
(Strictly speaking our target here is  $\Match^N(2,2)$ over a ring with 
indeterminates as indicated below; and we pass to $\C$ by a free choice of non-zero
evaluation of each.)
\\
}}
%We call the parts of $p$ `nations' and order/number as above.
Each edge that is between nation $i$ and nation $j$ is decorated with
$\off_{\mu_{ij}} = \mu_{ij}\offmat$.

We call the parts of $q$ `counties'.
Each vertex is (in the obvious sense) in one of the two parts of $s\in\PP_2(q)$.
Note that $s\in\PP_2(q)$ restricts to an element $s_i$ of $\PP_2(q|p_i)$
partitioning the counties of each nation.
Simply for definiteness in naming conventions, we order the two parts.
For vertices in the first %(resp. second)
part in $s_i$ %$\PP_2(q|p_i)$
we decorate with $\alpha_i$; % (resp. $\beta_i$), where $i$ is the nation.
and otherwise with $\beta_i$.
Note that the decoration  $x\in\{ \alpha_i, \beta_i \}$, say,
is the same on all vertices %at either end of an between edges
in the same county.
Each edge between vertices in the same county
is decorated with %$0 $, representing
$ x\omat$ where $x\in\{ \alpha_i, \beta_i \}$
is the common vertex decoration.
(We may abbreviate to the symbol 0 for this edge decoration.) 

The remaining edges ---
between vertices in different counties in the same nation are decorated as
follows.
If the order on counties given by $\rho$ places vertex $\vi$ before $\vj$
and also $\vi < \vj$ in the natural order then the $\vi\vj$
edge is +; otherwise it is $-$.
Next for each vertex in nation $i$ if it is in the first part in $s$ decorate
this vertex with $\alpha_i$, else decorate with $\beta_i$.
Finally for each signed edge, if it is $+$ (resp. -)
and the end vertices are %the same
both $\alpha_i$
then
decorate with $\fii_{\beta_i}$ (resp. $\mfii_{\beta_i}$);
or both $\beta_i$
then
decorate with $\fii_{\alpha_i}$ (resp. $\mfii_{\alpha_i}$);
else if end vertices are different then
decorate with $\ai$ (resp. $\mai$).
See % below
Fig.\ref{fig:N2}
for the matrix implications of these decorations.


%\whisper{ The above is still a bit glib. The precise formulation will emerge presently. }

}}

%}}}
%{{{ Examples

\befs{25}{Examples for elements $(p,q,\rho,s)$}
     {{
         \mdef Examples.
         Consider a nation of size 6 in some complete graph.
         Say the first nation here:
         $ p =\{ \{ 1,3,4,5,7,9 \}, \{2,6,...\},\{ 8,...\}, ...,\{...\}, ... \}$

         A $q$ refining this starts
         $q=\{\{ 1,5,7 \}, \{ 3,9 \}, \{ 4\},... \}$ --- writing out just the counties
         of the first nation.

         For the  order $\rho$ of these counties let us consider the written order
(which happens to be the nominal children-first order).
         Then we have the following signs
         in the first nation:
         
\[
\includegraphics[width=6cm]{\figdir hexa321a01.eps}
\hspace{1.591\ccm}
%\includegraphics[width=6cm]{\figdir hexa321a03.eps}
\includegraphics[width=6cm]{\figdir hexa321a04.eps}
%\hspace{.95\ccm}
%\includegraphics[width=6cm]{\figdir hexa321a0.eps}
\]
Thus for {example} the 35 edge is $-$ because 3 is higher in the nominal order but 5
comes first in the chosen county order.

Finally for $s$ let us lump the first two counties together:
$s = \{\{1,5,7,3,9\},\{4 \}\}$ (restricting here only to the first nation). 
Then the vertex variables are as shown on the right above - where some of the f/a labels
are also shown.

     }}

%}}}
\subsection{The main Theorem} $\;$ 
%{{{ higgs

\newcommand{\KK}{\ul{K}}
\newcommand{\GGG}{\ul{G}}
\newcommand{\III}{\ul{\II}} 


\beff{Theorem}{{

\mdef
A {\em (Higgs) \configuration} of $K_n$ is an assignment of a scalar
from $GL_1(\C)$ to each vertex;
and matrix from $GL_2(\C)$ to each edge,
so that each $K_2$ subgraph is assigned
from the set of six types
$\II = \{ \off, 0, \uppfii, \mfii, \uppai,\mai \} $
as in \eqref{pa:schema2}.
%(Note that there are variables in all these components.)

We observe  %will prove 
from {Proposition}~\ref{pr:L2class2}
that
a necessary condition for an element of $\Match^N(2,2)$
to give a braid representation is that it gives an \configuration\ of $K_N$.

Write $\hom(\KK_N,\GGG)$ for the set of \configuration s of $K_N$.
Note that the $K_2$ subgraphs of $K_N$ are in bijection with  the edges.
Define
$$
\III : \hom(\KK_N,\GGG) \rightarrow \hom(K_N^1 , \II )
$$
by mapping each $K_2$ configuration to its type
in the obvious way.
Observe then that there is a (possibly empty) fibre of solutions over each element
$\alphaa$ of
$\hom(K_N^1 , \II )$.
More generally the fibre $\III^{-1}(\alphaa)$ consists of the possible choices of
the parameters in each matrix.
\\
Remark: note that there is no {\it ab initio} guarantee here that there are
{\em any} solutions in ranks above two,
even before imposing higher-rank constraints,
since the $K_2$-subgraphs of $K_N$  %interlock
overlap with each other.


\iffalse
%}}}
%{{{ (old) X-lemma before thm

\ppmx{done: promote X-Lemma here. (but proof must remain after nec Theorem)}

\mdef {\bf{Lemma}}. \label{lem:Xeq}
{\em
Let $\FF:\Bcat\rightarrow\Match^N$ be a braid representation, hence given by
$\FF(\sigma)$.
Let $X$ be a diagonal invertible matrix in $\Match^N(2,2)$.
Then $\FF'(\sigma)= X \FF(\sigma) X^{-1}$ also gives a representation.

\newcommand{\simm}{\stackrel{-}{\sim}}

Consider the relation $\FF\simm\FF'$
if there exists any such diagonal invertible $X$
relating $\FF$ and $\FF'$ as above.
This is an equivalence relation.
%and then we say that $\FF$ and $\FF'$ are X-equivalent.
}

\medskip

{
\newcommand{\simm}{\stackrel{-}{\sim}}

%We call this
The relation $\simm$ is here called {\em X-equivalence}.
}

\medskip

\noindent
We state the Lemma here because we need the notation.
The analogue of this Lemma in classical representation theory is
stronger, and is elementary. Here in the monoidal setting it is not elementary.
The proof is in \S\ref{section: the proof}.  
\fi

%}}}
%{{{ thm

\begin{theorem} \label{th:mainx}

For each $N \in \N$ the
  %following
set
$\Rec(\germ_N)$ gives a complete set 
%$\SSS_N$ indexes %gives
%a transversal of the set
of charge-conserving braid representations
up to X-equivalence. 

\ppmx{-need to say what this is - from X-Lemma}
%natural equivalence:
\ignore{{\\
\ppm{Task: I have demoted it, but I think
Eric wants to include here the construction of
a transversal of the symmetry actions. We can do this.}
%{{{ ignore A1-4 etc

\\
A1. Pick a partition
$\lambda = (\lambda_1, \lambda_2, ..., \lambda_m )$ of $N$ and hence a partition of
$\ul{N} = \{1,2,...,N \}$ into
`nations',
$$
\ppp(\lambda) = \{
\{ 1,2,...,\lambda_1 \},
\{ \lambda_1 +1, \lambda_1 +2, ..., \lambda_1 + \lambda_2 \},
\hspace{1.65in}$$ $$\hspace{1.65in}
\{ \lambda_1  + \lambda_2+1, \lambda_1  + \lambda_2+2, ..., \lambda_1  + \lambda_2+ \lambda_3 \},
..., \{ ..., N \}\}
$$
\\ 2. Pick a partition of each nation into counties.
Thus we have a refinement $(\ppp(\lambda),q)$.
(Note that $q$ includes a partition, $q(i)$ say, of each nation.)
\\ 3. Pick a total order $\orr$ on counties $q(i)_j$ in each nation.
(For definiteness the
arbitrary labelling
$j$ order can be given by a convention, and the total order then
given in terms of this.)
\\ 4. Pick a partition $r$ of counties in each nation into two parts.
\\ B1. Form a $K_N$-configuration and hence a matrix
from $(\ppp(\lambda),q,\orr, r)$
as follows.
\\
...}}
%}}}
%\\ \whisper{...We will conclude the construction once we have some
%  machinery from the $N=2,3$ cases.}
%\\
\ppmx{paul improve this. recall/cite I set and define a controlling map
from configs in MatchN22 to solutions; and use to state theorem cleanly.}
\end{theorem}

\begin{remark}
As noted in Section~\ref{ss:target},
if $V$ is the target category then
isomorphisms in the functor category $(V,V)$ induce isomorphisms
in our representation category $(\Bcat,V)$.
Thus in our case
the action of the symmetric group $\Sym_N$ leads to a decomposition of $\germ_N$ into orbits.  In this way we may access all solutions from a much smaller set, called $\TTT_N$ below, via the $\Sigma_N$ action.  In fact, we can also use the symmetry $P$ induced from the Kronecker product ambiguity to reduce further (and often do).
See Section~\ref{ss:transversal} for details.
\end{remark}


%}}}
%{{{ proof outline

%\medskip

\vspace{.41\ccm}

\noindent
Outline of proof. $\;$
The proof is in Section~\ref{section: the proof}.
We first give a Theorem formulating sufficient conditions for a solution.
Then we solve these conditions in ranks 2 and 3.
Then  we will need a couple of Lemmas exploiting some magic in these solutions.

}}

%}}}

%{{{ Local Variables

% Local Variables:
% End:

%}}}


==> tex/braid-theorem0.bak.tex <==
% $Id: intro.tex,v 1.1 $
\module{braid-theorem0}

%% From the internet for making bar roman numerals %%
%\def\barroman#1{\sbox0{#1}\dimen0=\dimexpr\wd0+1pt\relax
\def\barroman#1{\sbox0{#1}\dimen0=\dimexpr\wd0+.1pt\relax
  \makebox[\dimen0]{\rlap{\vrule width\dimen0 height 0.06ex depth 0.06ex}%
    \rlap{\vrule width\dimen0 height\dimexpr\ht0+0.03ex\relax 
            depth\dimexpr-\ht0+0.09ex\relax}%
    \kern.5pt#1\kern.5pt}}


\section{Constructions for the main Theorem}
%{{{ notation

%% promoted to macros.tex
%\newcommand{\modelss}{\models^{\!\!\!\!\!\circ}} 
%\newcommand{\gaml}{\gamma^l} 
%\newcommand{\gamr}{\gamma^r} 

%\beff{Notation}{{ We will need some notation.}}

%\beff{Integer partitions and compositions}{{


  We write $\Lambda_N$ for the set of integer partitions of $N$.
  We may write $\lambda \vdash N$ for $\lambda\in \Lambda_N$. 

%}}}
%{{{ Aside/subsection How to read

\beff{On classification theorems}{{
    
\subsection{ %    \xxx{%Aside.
      How to read  the classification  %following
      Theorem~\ref{th:mainx}:
      } $\;$ 
      
An example of a classification theorem
is of course Young's classification of
irreducible representations of the symmetric group over $\C$.
Here one says that {\em irreducible} representations
of $\Sym_n$ may be classified
up to {\em isomorphism} by the set
$\Lambda_n$.
%of {\em integer partitions} of $n$.
%%(a set that is %relatively
%%well-understood).
Each of the three aspects of this formulation flags  challenges that we
must address in our problem.

Firstly, %And finally,
  analogously
to the integer partitions
we will need to introduce  %notation for
some %further relatively-straightforward
  combinatorial structures.
  (Our Theorem also gives a {\em construction}.
  We will introduce notation for this too.)


Secondly,
group/algebra representations form an additive category
in a natural way.
The category property yields a `good' notion of isomorphism.
The additive property
simultaneously implies that there are unboundedly many
classes of representations,
but also that these can be effectively
classified by classifying their additive components.
%
%Secondly, %  Firstly,
%  the natural notion of homomorphism of representations in the group/algebra setting
%contains a natural notion of isomorphism.
There is no canonical lift of these properties to the monoidal category setting
(confer for example \cite{MazorchukMiemietz16,MazorchukMiemietz14,RumyninWendland,KapVoev}),
so our lift  % will
sheds new light on this aspect of higher representation theory.

And finally, %Secondly,
  treated individually symmetric group algebras over algebraically closed
  fields are Artinian, so the Jordan--Holder property tells us that every
  representation has a decomposition series with irreducible factors.
  Indeed in the complex case the decomposition multiplicities characterise a
  representation up to isomorphism.
  There is no canonical lift of this property to monoidal categories
either
(roughly since decomposition series are additive decompositions,
  while the monoidal structure is multiplicative).
  This is one of the places where the rigidity of the $\Match^N$
  target categories
  saves the day --- we will be able to classify {\em all} representations directly.


%Secondly

  

}}

%\newpage

\medskip

%}}}
%{{{ notation preamble


\befff{Classification: Notation}{{

    %Here
    Next
    we construct two sets for each $N\in \N$.
    One is the set $\SSS_N$ to which we may apply an
    algorithm (given in (\ref{pa:rec}))
    to construct all varieties of solutions
    at level-$N$.
    The other gives a transversal of this set under the $\Sigma_N$ action
    from (\ref{restriction-and-symmetries})
    (and frames the effect of the $\Zz_2$ action),
    thus addressing the classification up to isomorphism.
}}

%}}}
%\subsection{Notation for index sets} $\;$ 
\subsection{Braid representations
            from multisets of row-2-coloured Young diagrams} $\;$ 
\newcommand{\jjj}{{\mathsf j}}  %% j function hook
%{{{ Just as

Just as
%integer partitions
%%(indexing $\Sym_N$ representations) can be
%-
multisets of integers -
represented as Young diagrams %,
-
index $\Sym_N$ representations,
we will see that
for braid representations we can use
multisets of row-2-coloured Young diagrams.
In fact these are a natural combinatorial generalisation of $\Lambda_N$.
%
First we explain this combinatoric;
then we show how each diagram leads to
a class of charge-conserving braid representations;
then we prove that this construction
exhausts the set of all such braid representations. 

%}}}
%{{{ J_N

\newcommand{\staro}{*}  %% the one we use! might be * to get +1 right!

\mdef
Given a set $\Omega$ and a map $\psi\in \Setcat(\Omega,\N)$ define
the
sets of multisets
of total degree $N$:
\[
J_N(\Omega) = J_N(\Omega,\psi) =
\{ f \in \Setcat(\Omega,\N_0) \; | \; \sum_{w\in\Omega} f(w) \psi(w) =N \}
\]
Thus for example
%Example.
if $\Omega=\N$ and $\psi(n)=n$ then $J_N(\N) = \Lambda_N$.

\mdef
For $S$ a set, define $\psi: S^\staro \rightarrow \N$
by $\psi(w) = length(w) +1$.
(Cf. (\ref{de:Set}).)
%[note we need to fix +1 convention, so using $\staro$ not $\star$...]
%One can c
Observe %it will be clear
that
up to isomorphism
$J_N(S^\staro)$ depends only on the cardinality of $S$.
Consider $J_N(S^\staro)$ for $S=\{1\}$, $\{1,2\},\{1,2,3\}$
and so on.

Of course $\psi : \{1\}^\staro \stackrel{\sim}{\rightarrow} \N$.
So
%Then firstly
$J_N(\{1\}^\staro ) $  is a realisation of $\Lambda_N$.
%Specifically, the function
For example
$f \in \Setcat(\{1\}^\star,\N_0)$
given by
$f(1)=1$; $f(11)=2$; $f(w)=0$ otherwise,
becomes
$(3,3,2)\vdash 8$.
%\raisebox{-.1in}{\includegraphics[width=.81cm]{xfig/y332.eps}}.

In this $J_N(S^\staro)$ notation,
%$\{1,2\}^\star  $
$\{1,2\}^N  $
%$J_N(\{1,2\}^\star ) $
encodes the set $\Gamma_N$ of %multisets of
{\em compositions} of %total degree
$N$ (via the $\jjj$-function given just below);
and $\{1,2\}^\staro  $
encodes the set $\Gamma$ of all compositions;
so $J_N(\{1,2\}^\staro ) $
encodes the set  of multisets of
compositions of total degree $N$.

%And finally t
The set we need ---
of multisets of row-2-coloured Young diagrams/compositions ---
is $J_N(\{1,2,3\}^\staro ) $. 
The construction works as follows.  %in (\ref{todo}).
Firstly $\Gamma^2$ denotes the set of 2-coloured compositions,
whose elements are compositions together with a two-part partition
of the components.
We may draw this as a stack of rows of boxes, where the top row is unshaded
but other rows can be unshaded or shaded
(in the first or second part respectively).
%Thus f
For example:
\raisebox{-.1in}{\includegraphics[width=.783cm]{xfig/y223.eps}}
$\in\Gamma^2_7$.
%
{(This box formulation  %will be
is useful, but
%these are not really Young diagrams as
note
%the
{\em columns} have % alignment has
no significance,
%unlike
cf. ordinary Young diagrams%
.)}

%}}}
%{{{ j functions

%\newcommand{\jjj}{{\mathsf j}}  %% j function hook

\mdef \label{de:j}
Given a 2-coloured composition
or equivalently a row-2-coloured Young diagram
$\lambda\in\Gamma_N^2$
then diagram
$\jjj_1(\lambda)\in\Gamma_{N+1}^2$ is obtained by adding a box to the last row;
$\jjj_2(\lambda)\in\Gamma_{N+1}^2$ is obtained by adding a box in a new unshaded row;
and
$\jjj_3(\lambda)\in\Gamma_{N+1}^2$ is obtained by adding a box in a new shaded row.
Starting with the one-box (unshaded) diagram,
a word  %$w \in J_N(\{1,2,3\}^\star ) $
$w \in \{1,2,3\}^*   $
then defines a row-2-coloured diagram by applying
the $\jjj_i$ maps in the sequence given by $w$.
That is
%$j : \{1,2,3\}^\star \rightarrow \Gamma^2$
$\jjj : \{1,2,3\}^n \rightarrow \Gamma_{n+1}^2$
is given by
$w_1 w_2 ... w_n \mapsto
 \jjj_{w_n} \circ ... \circ \jjj_{w_2} \circ \jjj_{w_1} (\square)$.
Thus $\jjj(121311) $ is given by
$\square
\stackrel{\jjj_1}{\mapsto}
\includegraphics[width=.53cm]{xfig/y2.eps}
\stackrel{\jjj_2}{\mapsto} 
\includegraphics[width=.53cm]{xfig/y21.eps}
\stackrel{\jjj_1}{\mapsto} 
\includegraphics[width=.53cm]{xfig/y22.eps}
\stackrel{\jjj_3}{\mapsto} 
\includegraphics[width=.53cm]{xfig/y221.eps}
\stackrel{\jjj_1}{\mapsto} 
\includegraphics[width=.53cm]{xfig/y222.eps}
\stackrel{\jjj_1}{\mapsto} 
\includegraphics[width=.783cm]{xfig/y223.eps}
%\mapsto  ...
$
and so on.   % \ppm{[fix the N shift convention]}

%}}}
%{{{ ignored order

\ignore{{
\mdef
\ppm{[time for bed, but in the morning the idea is that
part of this para will come
after the following one (!) just to give a definite order...,
and the rest deleted.]}
It will be convenient to have a total order on $\Gamma^2$.
We can pull one through from a total order on $\{1,2,3\}^*$
using the isomorphism $\jjj$.
For $\{1,2,3\}^*$
let us say firstly that longer sequences come before shorter ones:
$111<11<1$ and so on;
and for equal-length sequences we use dictionary order,
that is $111<112<113<121<...<333$.

Armed with this order, we have a way of
writing out a sequence of diagrams corresponding to a multiset
$f \in J_N(\{1,2,3\}^*)$. We use the above order, and the multiplities from $f$.
We can now assign vertices of $K_N$ to the $N$ boxes
in a multiset of 2-coloured compositions by filling the boxes with the
vertex numbers.
We fill the first diagram starting with  %from
1 in the top left corner then
increasing by 1 along rows and then down columns.
Then continue with the next diagram; and so on.

Thus for example:
\[
\includegraphics[width=3.494cm]{xfig/tree012ex10bbb1XI.eps}
%...like below but the first order...
\]

}}

%}}}
%{{{ \SSS_N

\mdef
Note that %Thus
$f \in J_N(\{1,2,3\}^\staro )$ assigns a multiplicity $f(w)$ to each
word $w$ and hence
diagram $\jjj(w)$,
such that the total degree is $N$.
We will show how
each such $f$ corresponds to an equivalence class of varieties of
configurations on $K_N$, and hence
matrices
that % we will show
give the functors $\FF:\Bcat\rightarrow\Match^N$.

%To obtain these configurations from $f$ we need
Firstly we
arrange %draw %assemble
2-coloured composition diagrams in multiplicities as given by $f$,
so that we have $N$ boxes altogether.
For example
with $f$ given by $f(1321)=1$, $f(131)=1$, $f(\emptyset)=2$ and
$f(w)=0$ otherwise we obtain an 11-box composite diagram such as:
\beq \label{eq:54110}
\jjj(f) \; =\;\;
\raisebox{-.21in}{
\includegraphics[width=2.94cm]{xfig/tree012ex10bbb1XI0.eps}
}
\eq
%And then secondly to
Secondly we
assign %associate
the $N$ vertices of $K_N$ to these $N$ boxes.
For example:
\beq \label{eq:5411}
\jjj(f) \; \mapsto\;\;
\raisebox{-.21in}{
\includegraphics[width=3.494cm]{xfig/tree012ex10bbb1XI.eps}
}
\eq

%We can do this assignment in any way.
Write
$\SSS_N$
for the set of {\em all} assignments
{\em up to the order within each row}.
Thus
\beq \label{eq:SSS2}
\SSS_2 = \{\;
\includegraphics[width=.8cm]{xfig/tree012ex2aab.eps}\;,\;\;
\includegraphics[width=.41cm]{xfig/tree012ex2ab1b.eps}\;,\;\;
\includegraphics[width=.41cm]{xfig/tree012ex2ba1b.eps}\;,\;\;
\includegraphics[width=.41cm]{xfig/tree012ex2abb.eps}\;,\;\;
\includegraphics[width=.41cm]{xfig/tree012ex2bab.eps}\;,\;\;
\includegraphics[width=1.03cm]{xfig/tree012ex2acb.eps}\;
\}.
\eq
%We can do this assignment in any way.
We can choose any such assignment for each $f$.
But 
%To do {\em this}
it will be convenient to have a prefered assignment,
of vertices in `book' order as in (\ref{eq:5411}).
This requires the diagrams in a composite to be written in a specific
sequence. We can do this using
%via
a declared  total order on
$\Gamma^2$ (or equivalently on $\{1,2,3\}^\staro $)
%Armed with such an order, we have a prescribed way of
%writing out a {\em sequence} of diagrams corresponding to
%$f$     %%the multiset $f \in J_N(\{1,2,3\}^*)$.
%%We use the  order, and the multiplicities from $f$,
 --- noting that identical diagrams are indistinguishable.
%Our example above is thus an example using some prescribed order.

\newcommand{\bbbbb}{{\mathsf b}}  %% book order injection hook

%For our choice of
%To give
For
a total order on
%$\Gamma^2$, let us use one on $\{1,2,3\}^*$ via the isomorphism $\jjj$.  For
$\{1,2,3\}^*$
let us say firstly that longer sequences come before shorter ones:
$111<11<1$ and so on;
and for equal-length sequences we use dictionary order,
that is $111<112<113<121<...<333$.
Then
we get our example
$\jjj(f)$ 
in (\ref{eq:54110}) above,
and hence (\ref{eq:5411}), on the nose.
Write
$\bbbbb : \jjj(J_N(\{1,2,3\}^*)) \rightarrow \SSS_N $
for the book order assignment.
Define $\TTT_N = \bbbbb( \jjj(J_N(\{1,2,3\}^*)) )$.
For example
$\TTT_2 =
\{\;
\includegraphics[width=.8cm]{xfig/tree012ex2aab.eps}\;,\;\;
\includegraphics[width=.41cm]{xfig/tree012ex2ab1b.eps}\;,\;\;
%\includegraphics[width=.41cm]{xfig/tree012ex2ba1b.eps}\;,\;\;
\includegraphics[width=.41cm]{xfig/tree012ex2abb.eps}\;,\;\;
%\includegraphics[width=.41cm]{xfig/tree012ex2bab.eps}\;,\;\;
\includegraphics[width=1.03cm]{xfig/tree012ex2acb.eps}\;
\}
$.
%}}}
%{{{ ignored good stuff and a reminder
\ignore{{
for example, with $f$ given by $f(1321)=1$, $f(131)=1$, $f(\emptyset)=2$ and
$f(w)=0$ otherwise we obtain an 11-box diagram:
\[
\includegraphics[width=2.94cm]{xfig/tree012ex10bbb1XI0.eps}
\]
}}
\ignore{{
We can now assign vertices of $K_N$ to the $N$ boxes
`in' $f$ % a multiset of 2-coloured compositions
by filling the boxes with the
vertex numbers.
We fill the first diagram starting with  %from
1 in the top left corner then
increasing by 1 along rows and then down columns.
Then continue with the next diagram; and so on:
\[
\includegraphics[width=3.494cm]{xfig/tree012ex10bbb1XI.eps}
\]
}}
%\ppm{[-my idea is to demote the treatment of other orders to the proof.]}

%}}}
%\input tex/notation-partition  %% moved from here.
%{{{ summary

\medskip
{There is a correspondence between $\SSS_2$ and our classification
for $N=2$ in Prop.\ref{pr:L2class2}.}
The rest of our exposition 
  amounts to showing $\SSS_N$ yields an index scheme for all
varieties of 
representations.
%%
%\sout{
%The next step is, via a suitable notion of equivalence, to deal with $N=2$.}
%%Via
Noting
Lemma~{\ref{lem:chacon1}(III)}, the
$N=2$ solutions
also give the possible edge configurations 
for all $N$.




%}}}

\input tex/notation-partition  %% 
%%\input Xlemma
%%%\inputt XlemmaNotes
%%%\inputt reps-N2

%{{{ Local Variables
% Local Variables:
% End:
%}}}


==> tex/constrainteq.tex <==

\vspace{.1in}

\section{Constraint equations: explicit orbits}
%Lemma~\ref{le:}
Theorem~\ref{th:constraints}
gives a transversal of the set of constraint equations,
but it is also  useful to have the complete orbits explicitly for a single $K_3$,
so we give these here.

%{{{ main Lemma

\begin{lemma} \label{lem:constraints}
Let $F:\Bcat\rightarrow\Mat^N$ be a level-$N$ charge-conserving
monoidal functor, thus determined by $F(\sigma)$.
  For $\NL=3$ the braid relations in the form \eqref{eq:braidx} imply % are sastisfied by
  the following
  constraints on entries in the `$abcd$ form' of $F(\sigma)$.
%{{{ eqs abcd version
The pure 12 sector:
%{{{ pure 12, 13 
\beq \label{eq:31xx}
a_{12} (a_{11}^2 -a_{12} a_{11} -b_{12} c_{12}) =0,
\hspace{1cm}
a_{12} (a_{22}^2 -a_{12} a_{22} -b_{12} c_{12}) =0,
\eq \beq \label{eq:31xxx}
\hspace{1cm}
a_{12} c_{12} d_{12} = 0 = a_{12} b_{12} d_{12} ,
\hspace{1cm}
a_{12} d_{12} (a_{12}-d_{12})=0,
\eq \beq \label{eq:31ixx} 
d_{12}(a_{22}^2 -d_{12} a_{22} -b_{12} c_{12})=0,
\hspace{1cm}
d_{12}(-a_{11}^2 +d_{12} a_{11} +b_{12} c_{12})=0
\eq
The pure 13 and 23 sectors are equivalent (substitute the appropriate $a_{ij}$s etc).
%(--- NB this is simply substitution, from the $abcd$ form of $F(\sigma)$;  %\eqref{eq:}.
%not via the diagonal $S_\NL$ action {\em per se}. But see also later.)

\ignore{{   %%% IGNORE STARTS!...
\beq \label{eq:32x} %\hspace{1cm}
h (g^2 -hg -jp) =0,
\hspace{1cm}
%, \hspace{1cm}
h(-w^2 +hw +jp)=0,
\hspace{1cm}
hpr=hjr=hr(h-r)=0
\eq
\beq \label{eq:32ix}
r(gr+jp  -g^2 )=0,
\hspace{1cm}
r( w^2 -rw  -jp)=0  %, \hspace{1cm} j(hv-av+ar)=0
\eq
}}
%}}}
\ignore{{
%{{{ pure 23
\beq \label{eq:38x}
k(f^2 -fk-ms)=0,
\hspace{1cm}
k(w^2 -kw -ms)=0,
\hspace{1cm}
ksv=kmv=kv(k-v)=0
\eq 
\beq \label{eq:311x}
v(-f^2 + fv + ms)=0,
\hspace{1cm}
%\]\[
v(w^2 -vw -ms)=0  %, \hspace{1cm}
\eq
%}}}
}}
Next we have twelve 3-term combinations from 123 (where $\bc_{ij}$ means either $b_{ij}$ or $c_{ij}$):
%
%{{{ 3-term mixed
\beq \label{eq:34xx}  %\hspace{1cm} \Or{c_{12}}{b_{12}} replaced by (b|c)_{12}
\bc_{12} (d_{13} d_{23} -d_{12} d_{23} -a_{12} d_{13})=0,
\hspace{1cm}
\bc_{12} (- a_{13} a_{23} +a_{12} a_{23} +d_{12} a_{13})=0  %, \hspace{1cm} b(-hk+ak+dh)=0
\eq
\beq \label{eq:36xx} 
\bc_{23} (-a_{23} d_{13} +d_{12} a_{23} -d_{12} a_{13})=0,
\hspace{1cm}
%p_j
\bc_{13} (a_{13} d_{23} -a_{12} d_{23} +a_{12} d_{13})=0
\eq
\beq \label{eq:38xx}
%s_m
\bc_{23}  (- a_{13} d_{23} -a_{12} a_{23} +a_{12} a_{13}) =0,
\hspace{1cm}
%s_m
\bc_{23}  (d_{12} d_{23}+ a_{23} d_{13} -d_{12} d_{13})=0  %, \hspace{1cm}
%\eq \[ m(dv+kr-dr)=0 
\eq
%}}}
Finally six 4-term combinations from 123:
%
%{{{ 4-term mixed
\beq \label{eq:35x} 
% m (- h  v - a_{12} k  + a_{12} h ) =0 , \hspace{1cm}
-a_{13} d_{23}^2 + a_{13}^2 d_{23} -a_{12} b_{23} c_{23}
               + a_{12} b_{13} c_{13} =0
, \hspace{1cm}  %\eq \beq
%\label{eq:37x}
 -b_{13} a_{23} c_{13}
 +b_{12} c_{12} a_{23} -d_{12} a_{13}^2 +d_{12}^2 a_{13} =0  %, \hspace{1cm} p(-kr+dk-dh)=0
\eq
%\ignore{{
\beq \label{eq:33x}
-a_{13} b_{23}c_{23}- a_{12} a_{23}^2 +a_{12}^2 a_{23} +b_{12} c_{12} a_{13} =0 , \hspace{1cm} %\eq \[
b_{13}c_{13}d_{23} -b_{12} c_{12} d_{23} +a_{12} d_{13}^2 -a_{12}^2 d_{13} =0
\eq %, \hspace{1cm} %\] \[
%\ignore{{
%dms-kr^2 +k^2 r -djp =0 \]
\beq \label{eq:310x}
d_{12}b_{23}c_{23}-a_{23}d_{13}^2 +a_{23}^2 d_{13} -d_{12}b_{13}c_{13} =0, \hspace{1cm}
d_{12}d_{23}^2 - d_{12}^2 d_{23} +b_{23}d_{13}c_{23} -b_{12}c_{12}d_{13} =0 %,\hspace{1cm}
\eq
\ignore{{
%}}}
}}  %%% ...IGNORE ENDS!
%}}}
\end{lemma}
\noindent Proof. Direct calculation.
%(generalising the proof of Prop.\ref{pr:L2class}).
\qed

%{{{ SYMMETRIES
%(--
%Note the  %interesting
%symmetries under $\Sym_\NL$.
%See Lemma~\ref{lem:sym1} for more on these. %)

The following describes the symmetries under $\Sym_N$, which we have used to 
give a more abbreviated form in Theorem \ref{th:constraints}.

\ignore{{
We should recall the action of $S_{\NL}$ (from Eric's notes!).
We claim for example that elementary transposition $(12)$ behaves
like: $(12) a_{11} = a_{22}$;
$(12) a_{12} = d_{12}$;
$(12) b_{12} = c_{12}$;
$(12) b_{23} = b_{23}$ and so on.
We should get a good check of all these relations by applying
symmetry!
For example applying $(12)$ to
the first of the four equations given in
\eqref{eq:34xx} we get: the second.
Applying $(23)$ we get the first from \eqref{eq:36xx}.
...}}

%}}}

%}}}
%{{{ SYMMETRY LEMMA

\medskip  %\[ \] 

\begin{lemma} \label{lem:sym1}
%  Claim (moving from inside Lemma~\ref{lem:constraints}):
  Elementary transpositions in
the $\Sym_\NL$ action permute matrix entries and hence act on equations
(\ref{eq:31xx}-\ref{eq:310x}). Altogether the action can be expressed as $\omega a_i = a_{\omega(i)}$
and 
$$
\omega a_{ij} = a_{\omega(i) \omega(j)}   ,
$$
where it is understood that $a_{ij}=d_{ji}$
and $b_{ij} = c_{ji}$.


\iffalse
\\
First we have the formality %(important) triviality
of encoding in our
$abcd$ notation. Thus $(12)$ acts by:
\\
$(12) a_{11} = a_{22}$; $\;$ 
$(12) a_{12} = d_{12}$; $\;$ 
$(12) b_{12} = c_{12}$; $\;$ 
\\
$(12) b_{23} = b_{13}$
%(naively might expect different here, so explain this one Paul!:
($b_{23} = F(\sigma)_{23,32}$ so
$(12)  F(\sigma)_{23,32}= F(\sigma)_{13,31} = b_{13}$)
%--- looks like I got this one wrong ...)
and so on:
\[
\begin{array}{l|lllllllllllllll}
(ij).a_{kl}
     & a_1 & a_{12} & b_{12} & c_{12} & d_{12} & a_2 & a_{13} & b_{13}
  & c_{13} & d_{13} & a_{23} & b_{23} & c_{23} & d_{23} & a_3 \\ \hline
(12) & a_2 & d_{12} & c_{12} & b_{12} & a_{12} & a_1 & a_{23} & b_{23} & c_{23} & d_{23} & a_{13} & b_{13} & c_{13} & d_{13} & a_3 \\
(23) & a_1 & a_{13} & b_{13} & c_{13} & d_{13} & a_3 & a_{12} & b_{12} & c_{12} & d_{12} & d_{23} & c_{23} & b_{23} & a_{23} & a_2 \\
%     &     &        &        &        &        &     &        &        &        &        &        &        &        &        &    
\end{array}
\]
What about say $(13)a_{23} = (12)(23)(12) a_{23} = d_{12}$
(we can work it out as $a_{21}=d_{12}$)
or $(14)a_{34}$?
%We should get a good check of all these relations by applying symmetry!
%For example
\\
Applying $(12)$ to
\eqref{eq:31xx}(i,ii) we get: \eqref{eq:31ixx}(i,ii) respectively.
\\
Applying $(12)$ to
\eqref{eq:31xxx}(i) we get: the second.
\\
...Applying $(12)$ to
the first of the four equations given in
\eqref{eq:34xx} we get: the second.
Applying $(23)$ we get the first from \eqref{eq:36xx}.
...
\\
Next consider the 4-term equations.
Applying $(12)$ to \eqref{eq:35x}(i) we get \eqref{eq:310x}(i).
Applying $(23)$ to \eqref{eq:35x}(i) we get %\eqref{eq:310x}(i).
...
 (Probably all the unfinished above works. So...)
\\
Next consider the action of $P$ from \eqref{eq:Paction}.
\\
Applying $P$ to $a_{ii} = R_{ii,ii}$ there is no change.
Applying to $a_{12}= R_{12,12}$ we get $P a_{12} = d_{12}$, $P b_{12}
= P R_{12,21} = R_{21,12} = c_{12}$, ...
\\
Applying $P$ to \eqref{eq:35x}(i) we get \eqref{eq:310x}(i),
with an irrelevant sign change. 
%... FINISH!!

Altogether the actions are encoded on the Cayley graph below.
%
%}}}
%{{{ graphs
%
%\medskip
%
Here is a Cayley graph pic of  %one of
the $S_N \times P$ orbit of 4-term expressions:
\[
%\ignore{{
\xymatrix{
        &  24i \ar[dd]_{(12)}^{P_-} \ar[dl]_{(23)}  &  24ii \ar[dll]^(.4){(12)} \ar[dr]^{(23)}_{P_-}
  \\
  25i \ar[drr]^(.7){P_-}  &        &       &  25ii \ar[dl]_{(12)} \\
        &  26i \ar[r]_{(23)}  &  26ii
}
%}}
\]
--- the label $P_-$ means that $P$ acts by a sign change (irrelevant
since expressions are zero, but a formally non-identical action).
NB I have not yet taken care of such signs in general, just where
contradistinguishing two actions.
\\
NB so far the interaction $S_N / P$ looks a bit less symmetric than I was
expecting. something to check!
On some of them the generators all act differently, but on some there
are degenerations (up to sign).
\\
Comments: surely involutive so I don't know why I put arrows on.
It might not look like it but I think this gives the complete picture
for this orbit in this rank...  \\
Next the 3-term orbit under $S_N$ and $P$:
\[
\xymatrix{ 21i \ar[r]^{(12)} \ar[dd]^{(23)} \ar[drrr]^{P}
              & 21i' \ar[dd]^{(23)} \ar[dr]_{P}
  \\ && 21ii \ar[r]_{(12)} \ar[dd]^{(23)} & 21ii' \ar[dd]^{(23)} \\
  22i \ar[dd]^{(12)} \ar[drrr]^{P_-} & 22i' \ar[dd]^{(12)}
  \\ && 22ii \ar[dd]^{(12)} & 22ii' \ar[dd]^{(12)} \\
  23i \ar[r]^{(23)} \ar[drrr]^{P_-} & 23i' \ar[dr]_{P_-}
  \\ && 23ii \ar[r]_{(23)} & 23ii' \\
}
\]
\fi


\end{lemma}


%}}}



%\vspace{1cm}



==> tex/figSymGpAct.tex <==

\module{figSymGpAct}

%{{{ Symm gp actions figure
\begin{figure}
\caption{
Symmetry group actions for an $\pai\pfii\pai$ case.
\ignore{{
Note that some edge matrices are `twisted equal' as shown.
Note that while the  $\pai\pfii$ labelling has  `equilateral'
symmetry (we can start with the $\pfii$ anywhere),
the twists do not: it is not possible to have both `twisted equalities'
to the long edge.
Note that in this $\pai\pfii\pai$
case the $P(13)$ action fixes the original configuration.
However if we start with $\pai\pai\pfii$ it  passes to  $\pfii\pai\pai$.
}}
\label{fig:sga1}}
\[
\xy \xygraph{
!M{\mbermpp{1}{2}{1}{{\pai}}{{\pai}}{{\pfii}}{}{}{} }
[dd]
:@{-->} [dl]^{(12)}
[urrr] :@{-->} [dr]^{(23)}
 [dlllll]
 !M{\mbermpp{1}{2}{2}{{\mai}}{{\pfii}}{{\pai}}{\sim}{\sim}{} }
[rrrr]
!M{\mbermpp{1}{1}{2}{{\pfii}}{{\mai}}{{\pai}}{\sim}{}{\sim} }
 }
 \xygraph{
 [ddlllll]
 :@{-->} [d]^{(23)} [urrrrrrr] :@{-->} [d]^{(12)}
[dllllllll]
!M{\mbermpp{1}{2}{2}{{\pai}}{{\mfii}}{{\mai}}{\sim}{\sim}{} }
[rrrr]
!M{\mbermpp{1}{1}{2}{{\mfii}}{{\pai}}{{\mai}}{\sim}{}{\sim} }
 }
 \xygraph{
 [ddllll]
 :@{-->} [dr]^{(12)} [urrrr] :@{-->} [dl]^{(23)}
[dlll]
!M{\mbermpp{1}{2}{1}{{\mai}}{{\mai}}{{\mfii}}{}{}{} }
}
 \endxy
\]
\end{figure}
%}}}


==> tex/figSymGpAct2orig.tex <==

\module{figSymGpAct2}


%{{{ sym gp actions figure
\begin{figure}
\[
%the layout of this figure embeds xypics (\mbermpp macros) in xy
%here the chunks are moved around with [dl] etc so everything is a bit
%quantised. (Dont know how to adjust separations.)
\xy        %can't adjust R= here.
\xygraph{  %or anywhere here!
!M{\mbermpp{1}{2}{1}{{\pai}}{{\pai}}{{\pfii}}{}{}{} }
[dl]  %moves the first (12)-arrow relative to top triangle
:@{-->} [dl]^{(12)}
[urrrrr] :@{-->} [dr]^{(23)}
 [dlllllll]
 !M{\mbermpp{1}{2}{2}{{\mai}}{{\pfii}}{{\pai}}{\sim}{\sim}{} }
[rrrrrr]
!M{\mbermpp{1}{1}{2}{{\pfii}}{{\mai}}{{\pai}}{\sim}{}{\sim} }
 }
 \xygraph{
 [ddlllllll]
 :@{-->} [d]^{(23)} [urrrrrrrrr] :@{-->} [d]^{(12)}
[dllllllllll]
!M{\mbermpp{1}{2}{2}{{\pai}}{{\mfii}}{{\mai}}{\sim}{\sim}{} }
[rrrrrr]  %moves the 5th triangle
!M{\mbermpp{1}{1}{2}{{\mfii}}{{\pai}}{{\mai}}{\sim}{}{\sim} }
 }
 \xygraph{
 [ddlllll]
 :@{-->} [dr]^{(12)} [urrrr] :@{-->} [dl]^{(23)}
[lll]  %this moves the `cursor', hence last triangle, left a bit
%\POS+(42,0)  %this throws an error!
!M{\mbermpp{1}{2}{1}{{\mai}}{{\mai}}{{\mfii}}{}{}{} }
}
 \endxy
\]
\caption{%(Using xygraph) \hspace{.1in}
Action of 
%Symmetry group actions for an $\pai\pfii\pai$ case.
symmetry group $\Sym_3$ on an $\pai\pfii\pai$ solution.
%\ignore{{
Note that some edge matrices are `twisted equal' (equal up to bar) as shown.
\ppm{[-are the subtle (re)label conventions appropriate here
- see e.g. top left -, or would simple
$\alpha,\beta$ be better?]}
\ignore{{
Note that while the  $\pai\pfii$ labelling has full `equilateral'
symmetry (we can start with the $\pfii$ anywhere),
the twists do not: it is not possible to have both `twisted equalities'
to the long edge.
}}
\label{fig:sga1}}
\end{figure}
%}}}


==> tex/notation-braid.tex <==
\module{notation-braid}
%\newcommand{\integ}{\ppm{natural}}


%\section{Functors from braid categories} \label{ss:ffbc}
%\subsection{Braid categories} \label{ss:braidcats}

%{{{ braid

%{{{ ignore

%\newcommand{\vs}{\varsigma}  % presentation gens
%\newcommand{\vsigma}{\vs}  % presentation gens
%\newcommand{\botimes}{\boxtimes} 

\ignore{{
Here $B_n$ denotes the $n$-string braid group. There are various
alternative definitions defining $B_n$ up to isomorphism.
Informally elements of $B_n$ are braidings of an ordered set of $n$
strings. 

Note that given an ordered pair $(b,b') \in B_n \times B_m$ there is an element 
$b\botimes b' \in B_{n+m}$ obtained by `side-by-side concatenation'.
(Strictly speaking some choices are needed in this construction 
- with details depending on the definition of $B_n$ - 
upon which we shall not dwell here.)
}}
%}}}


%\mdef
Our monoidal category $\Bcat$
has its geometrical definition
%is defined geometrically
in \S\ref{ss:braid}. %above.
But in order to verify functors it is  %very
useful to recall a finite presentation.

Recall, a {\em{\integ}} monoidal category is one whose object monoid is $(\N,+)$
  (confer \cite{MacLane2}).

%% \vs defined in macros2
\newcommand{\vsm}{\vs_-}

\begin{definition} \label{de:Bcat0}
%{{{ ignore
\ignore{{
  {$\;$} \\ $\bullet$ 
  %In what follows, $\Bcat_{-}$
  The {\em ordinary braid category} $\Bcat_{-}$ is the 
%an \integ\  strict monoidal
category
with
object set $\Nn$  and
$\Bcat_{-}(n,n) = B_n$, and 
$\Bcat_{-}(n,m)=\emptyset$ otherwise
(see e.g. \cite[XI.4]{MacLane}).
\\
\item $\bullet$
$\Bcat$ denotes  the {\em braid category}:
%a
an \integ\ 
strict monoidal category
with
%object monoid $(\Nn,+)$ generated by 1, and
$\Bcat(n,n) = B_n$,
$\Bcat(n,m)=\emptyset$ otherwise, and monoidal composition $\otimes$
%is
via side-by-side concatenation of suitable braid representatives
(see e.g. \cite[XI.4]{MacLane}).
\\
\item $\bullet$ 
}}
%}}}
%
  The \integ\ strict monoidal category
$\Bcat'$ is that presented by  generators $\vs$
and $\vsm \in \Bcat'(2,2)$; and relations as follows.
We write
$1_n$ for the identity morphism in $\Bcat'(n,n)$;
$\vsigma_1 = \vsigma\otimes 1_1$;
$\vsigma_2 = 1_1\otimes \vsigma$
in $\Bcat'(3,3)$.
Relations are:
\beq \label{eq:inverse}
\vsigma \; \vsm %\vsigma^{-1}
\;=\; 1_2 \; =\;  %\vsigma^{-1}
\ppm{\vsm}  \; \vsigma
\eq
\beq \label{eq:braidx}
\;\;\;
\vsigma_1 \vsigma_2 \vsigma_1 = \vsigma_2 \vsigma_1 \vsigma_2
\hspace{.3in}\mbox{ that is }\hspace{.34in}
\braidrel{\vsigma}{1_1}
\eq
\end{definition}

%}}}
%{{{ Artin

{
Recall that category
  $\Bcat$ is monoidally generated by the positive braid
    $\sigma\in\Bcat(2,2)$ and its inverse (denoted $\sigma^{-1}$).
}
Via Artin's local presentation \cite{Artin:1925} we have the following.

\begin{proposition} \label{pr:Bcat1}
%  (1)  $\Bcat$ is monoidally generated by the positive braid
%    $\sigma\in\Bcat(2,2)$ and its inverse (denoted $\sigma^{-1}$).
%\\
%(2)
%{\rm \cite{Artin:1925}}
A presentation for $\Bcat$ is given by $\Bcat \cong \Bcat'$
where $\sigma \mapsto \vs$.
\qed
\iffalse

\\
  \ppm{
Note (CLAIM) that all other relations we want for isomorphism
follow from the construction of $\Bcat'$ as a monoidal category.
  }
  
  \fi
  
\end{proposition}

%}}}
%{{{ iffalse

\iffalse
\proof (1)
%(Routine --- depending on how the meta-definition of $B_n$ above unpacks.)
Fix $n$ for a moment and 
let $\sigma_i \in B_n = \Bcat(n,n)$
denote the positive braid generator braiding in the
$i$-and-$i\!+\!1$ position.
We know from the definition that $\Bcat(n,n)$ is multiplicatively
generated by the $\sigma_i$s and inverses.
Now observe that each $\sigma_i$ for each $n$ is expressible using
$\sigma$, $1_1$ and $\otimes$.
\\
(2) It is straightforward to verify that the defining relations of
$\Bcat'$ are obeyed by the images, so the issue is if there is a
kernel.
We compare with Artin's group presentations for the various $B_n$'s
%(Artin's presentation)
and observe  %establish
that the relations in these group presentations arise from the
given monoidal category presentation.  \qed

\medskip

\fi


%}}}



==> tex/notation-composition.tex <==
% $Id: intro.tex,v 1.1 $
\module{notation-composition}

%\hspace{.1in}

\ppm{probably just swap in ericpaulx version here!---}

%{{{ composition notation
\beff{More composition notation}{{

\mdef
  If $\lambda=\lambda_1 \lambda_2 \cdots \lambda_L$ is a composition then we write
  $\Gamma_\lambda$ for the set
  \[
\Gamma_\lambda = \times_{i=1}^{L} \Gamma_{\lambda_i}
\]
Example: $\Gamma_{22} = \{ (11,11), (11,2), (2,11), (2,2) \}$.
We may write $\mu \models \lambda$ for $\mu \in \Gamma_{\lambda}$. 
\\
If $\lambda$ is a partition
we write $\Gamma'_\lambda$ for the subset of $\Gamma_\lambda$ 
of multicompositions $\mu$
such that if there are parts of $\lambda$ of tied order then
their compositions appear in $\mu$ in (weak) lex order.
\\
Example $\Gamma'_{22} = \{  (11,11), (11,2), (2,2) \}$.
We may write $\mu \modelss \lambda$ for $\mu \in \Gamma'_{\lambda}$. 


\medskip

%\newcommand{\gaml}{\gamma^l} 
%\newcommand{\gamr}{\gamma^r} 

\mdef \label{de:laml1}
Let $\lambda=\lambda_1 \lambda_2 \cdots \lambda_L \in \Gamma_N$
be a non-empty composition.
We define
$$
\gaml(\lambda) =\lambda_1 \lambda_2 \cdots (\lambda_L+1)
$$
and
 $\gamr(\lambda) =\lambda_1 \lambda_2 \cdots \lambda_L 1$.
Observe that both
$\gaml$ and $\gamr$
define injective functions from $\Gamma_N$ to  $\Gamma_{N+1}$,
and that $\gaml(\Gamma_N) \cap \gamr(\Gamma_N) = \emptyset$.
Thus in particular
\[
| \Gamma_N | = 2^{N-1}
\]
and the orders of all $\Gamma_\lambda$s follow.

}}

%}}}
%{{{ set to int notation


\beff{Notation}{{

\mdef
Given an integer partition, or indeed a composition,
$\lambda = (\lambda_1, \lambda_2, ..., \lambda_m )$ of $N$
we have a partition of
$\ul{N} = \{1,2,...,N \}$ into
`nations':
$$
\ppp(\lambda) = \{
\{ 1,2,...,\lambda_1 \},
\{ \lambda_1 +1, \lambda_1 +2, ..., \lambda_1 + \lambda_2 \},
\hspace{1.65in}$$ $$\hspace{.65in}
\{ \lambda_1  + \lambda_2+1, \lambda_1  + \lambda_2+2, ..., \lambda_1  + \lambda_2+ \lambda_3 \},
...,
\{ %\lambda_1 +\lambda_2 +...+\lambda_{m-1}+1
\left(\sum_{i=1}^{m-1} \lambda_i \right)+1
, ..., N \}\}
$$


\mdef
Given a set partition $p$ of a set $S$ of order $N$ we write $|p|$ for the integer partition
of $N$ given by the orders of the parts of $p$.
\\
(NB This does not require $S$ to be ordered.
If $S$ is ordered, then we may also extract
a {\em composition} $||p||$.) 

}}


%}}}

%{{{ Local Variables

% Local Variables:
% End:

%}}}


==> tex/reps-N4signature-old.tex <==

\module{reps-N4signature}

\newcommand{\maps}{\rightarrow}  %% notation for signatures


\section{Signatures: Eigenvalues and isomorphism from a linear perspective} \label{ss:signature} \label{ss:spectrum}

%{{{ signatures

%Then signatures for all.

%\newcommand{\varalpha}{{\bf \alpha}} 
%\newcommand{\varalpha}{{\large \alpha}} 
\newcommand{\varalpha}{\alphaa}
\newcommand{\sep}{:}  %% nations:... separator

A {\em signature}  is, roughly, the eigenvalue spectrum of the solution matrix
for each solution type.
Since the actual eigenvalues of a solution come from
the specific point on the variety,
%setting indeterminates from the solutions,
what we focus on here is the generic
degeneracies
%(or generic degeneracies)
rather than the values.
Since the largest block matrix in $F(\sigma)$ is $2\times 2$, we can
compute the generic degeneracies for each variety
(indeed in principle we can compute a  Jordan form including all points).
We will give the degeneracies as an unordered list, and hence as a partition of $N^2$.
Thus we
may
write
$\varalpha \maps \omega(\varalpha)$ if
$\omega(\varalpha)$ is the list of degeneracies for
configuration $\varalpha$.

%}}}
%{{{ more, N=2


It is straightforward to work out eigenvalues and multiplicities
for a specific class of solutions --- i.e. for $F(\sigma)$.
Of course if two eigenvalue spectrums do not agree, then the solutions
cannot be isomorphic. But even when they do agree, they may not be
isomorphic.
%Here we show some examples.



Rank-1 is trivial: we write $\square\maps (1)$ to denote that the trivial
variety $\square$ has solutions with a single eigenvalue with degeneracy 1.
Rank-2 is straightforward.
Our types $0,\pfii,\pai,\off$ are:
\\
$\square\!\square\maps (4)$, \quad
$\includegraphics[width=.251cm]{xfig/tree123Pa2.eps} %thing???
\maps (3,1)$, \quad
$\includegraphics[width=.251cm]{xfig/tree123Pa3.eps} %thing???
\maps (2,2)$, \quad
$ \square\;\square\maps (1^4)$.
%
\\
Let us note in passing: % that 
(1) Type $\pfii$ has two eigenvalues with degeneracies (3,1),
corresponding to the classical $U_qsl_2$ symmetry:
$2\otimes 2 = 3 \oplus 1$ (sometimes written
$\square\otimes\square=\square\!\square\oplus\emptyset$
\cite{drinfeld,Jimbo86}).
%We write this signature as $\pfii \rightarrow 31$.
\\ (2) Type $\off$ can be specialised to $\alpha_1 = \alpha_2$ whereupon
(up to the trivial overall factor)
we
recover the representations given in \cite[\S12.1.1]{Martin91}
(cf. the Birman--Murakami--Wenzl algebra). 

%}}}
%{{{ In general

In general $\omega(\varalpha)$ `factorises' into a contribution
$\phi(\alphaa)$
from $\off$ edges
and a contribution  $ \nu_i(\alphaa)$ from each nation:
$\omega(\varalpha) = \phi(\alphaa) \prod_{i} \nu_i(\alphaa)$.

\mdef \label{de:phinu}
%Also note that t
The contribution of eigenvalues of the form $\pm \mu_{ij}$ from
$\off$ edges is given in general by the following.
Let nations
of a solution $\alphaa$ 
be indexed by some ordered set $I = I(\alphaa)$; and for $i \in I$ let
$N_i = |p_i|$ denote the size of nation $i$.
Then the part of the signature
of solution $\alphaa$
coming from edges between nations is
\[
%formula
\phi(\alphaa) \; =  \prod_{i<j \in I} (N_i N_j, N_i N_j)
%  2 {{\pi}\choose{2}}
\]
--- that is, there are $N_i N_j$ eigenalues $\pm\mu_{ij}$.
For example, If $\lambda = \square\!\square\;\;\square$ then we have just $(2,2)$
from these edges.
The number of free parameters $\mu_{ij}$
in the variety coming from this part of the matrix
is $ {{|I|}\choose{2}}  $.

\newcommand{\hash}{\#} 

%And that
Meanwhile
each nation $i$ contributes (one or) two eigenvalues, with multiplicities given
as follows. Let $\hash_i0$ denote the number of 0 edges.
Let set $J_i$ index the counties, i.e. the elements of $q|p_i$.
Then
$  \hash_i 0 \; = \; \prod_{j\in J_i} {{|q_j|}\choose{2}}  $.
Let $s_2(i)$ denote the set of blue (colour 2) vertices.
We have
\beq \label{eq:nationsignature}
\nu_i(\alphaa) =
({{N_i}\choose{2}} + \hash_i 0 +|s_1(i)|,
 {{N_i}\choose{2}} - \hash_i 0 +|s_2(i)|) . 
\eq
Note: (i) That this does not depend on the order on counties.
(ii) That each one-nation representation is
(up to an elementary rescaling) a representation of some Hecke algebra.
\ignore{{
...by the number of vertices of each colour in that nation
plus \ppm{bla bla bla - write it out!
...Notation...}.
Thus (ignoring the single-county exceptions)
\[
\omega(\alphaa) \;  = 2...|...
\]
}}%

In practice we may notate $\omega(\alphaa)$ as
$(\nu_1 ; \nu_2 ; ... ;\nu_{|I|} \sep \phi)$.
%Note in particular that all one-nation representations are Hecke algebra
%representations (up to an elementary rescaling).
\quad %\\
Now consider rank-3.

%}}}
%{{{ /// etc

\mdef We start with
$\square\;\square\;\square =\off\off\off$ in $N=3$ as in Lemma~\ref{le:///}.
Here there are (up to) 9 distinct eigenvalues
($a_1, a_2, a_3, \pm\mu, \pm\nu,\pm\lambda$),
each of multiplicity 1;
given by 6 free parameters ($a_1, a_2, a_3, \mu, \nu,\lambda$), as shown.
We record this as the `signature'
$(1^9) = (1;1;1\sep 1,1,1,1,1,1)$.
\[
\ber{2}{3}{\;\;\;\;/_{\pm\mu} }{\;\;\;\; /_{\pm\nu} }{\;/_{\pm\lambda} \;}
\hspace{.1in}
\hspace{-.02471in} signature: \; (1^9),6
\]

%}}}
%{{{ here on the left (notes for //f)
\ppmx{[PAUL: Maybe demote this to an eigenvalue section later?]}
%- % here  %on the left

\mdef
For
$\includegraphics[width=.251cm]{xfig/tree123Pa2.eps}\;\square$,
so for example
$\off\off\uppfii$ as in Lem.\ref{le://+},
there is
1 eigenvalue of multiplicity 3;
2 eigenvalues of multiplicity 2;
and there 
are 2 eigenvalues of multiplicity 1, all given by 4 parameters.
Note that there is a variable $\beta$ associated to the $\pfii$ edge which does
not manifest elsewhere.
Note also that the object cannot be diagonalised over the ground ring,
or more specifically it would have a non-trivial Jordan block in the
specialisation $a_1 = \beta$.
\ignore{{
\hspace{.1in}
%On the right
For $\off\off\uppai$
the $\uppai$ does not need such a decoration, since the
eigenvalues are given by the vertex eigenvalues.
}}
%\ppm{- whats going on with eigenvalues in second one? check.
%I think this was not what we wrote in Lemma above! --- but maybe fixed now.}
%}}}

%\includegraphics[width=16cm]{xfig/tree123PajN4.eps}

%{{{ N=3

%%% some macros for organising tables of signatures: %%%
\newcommand{\zzz}{, \qquad}
\newcommand{\zzzz}{&}
%\newcommand{\chomp}[3]{\begin{array}{c} #1 = #2 \\ \maps #3 \end{array}}
\newcommand{\chomp}[3]{\!\!\!\begin{array}{c} #1 \\  #2 \\  #3 \end{array}\!\!\!}
%\newcommand{\chmp}[3]{\begin{array}{c} #1  \\ \maps #3 \end{array}}
\newcommand{\chmp}[3]{\!\!\!\begin{array}{c} #1  \\  #3 \end{array}\!\!\!}

\mdef
Altogether for $N=3$ (here giving just the degeneracies,
for a $\GG_N$-transversal cf. Prop.\ref{pr:N3}): %Fig.\ref{fig:tree123}):
\smallskip
%{{{ TABLE

\noindent
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
$\chomp{\square\!\square\!\square}{=000 }{\maps (9)}$
\zzzz
$\chomp{\includegraphics[width=.51cm]{xfig/tree123Pa13.eps}}{0\pai\pai}{(6,3)}$
\zzzz
$\chomp{\includegraphics[width=.51cm]{xfig/tree123Pa12.eps}}{0ff}{(7,2)}$
\zzzz
$\chomp{\includegraphics[width=.251cm]{xfig/tree123Pa32.eps}}{afa}{(5,4)}$
\zzzz
$\chomp{\includegraphics[width=.251cm]{xfig/tree123Pa23.eps}}{faa}{(5,4)}$
% \ppm{(`external' isomorphism with $afa$?)}
\zzzz
$\chomp{\includegraphics[width=.251cm]{xfig/tree123Pa22.eps}}{fff}{(6,3)}$
%(NB the accidental degeneracy with 0aa.)
%\\ \hline \end{tabular}
%
%\noindent
%\begin{tabular}{|c|c|c|c|c|c|}
%\hline
\zzzz
$\chomp{\square\!\square\;\square}{0\off\off}{(4;1:2,2)}$ %= (4,2,2,1)} $
\zzzz
$\chomp{\includegraphics[width=.251cm]{xfig/tree123Pa2.eps}\;\square}{f\off\off}{(3,1;1:2,2)}$ %=(3,2,2,1,1)}$
\zzzz
$\chomp{\includegraphics[width=.251cm]{xfig/tree123Pa3.eps}\;\square}{a\off\off}{(2,2;1:2,2)}$ %=(2,2,2,2,1)}$
\zzzz
$\chomp{\square\;\square\;\square}{\off\off\off}{  (1;1;1:1^6)}$  %=(1^9)}$
\\ \hline
\end{tabular}

%}}}
\smallskip \noindent
Notes:
(i) In general  %the size
$|\TTT_N | = 1,4,13,46,154,...$
is the Euler `forest' transform of the one-nation sequence $3^{N-1}$
(cf. Fig.\ref{fig:N1234}).
This is A104460 in \cite{Sloane}. 
From the $\PPP$-orbits in 
Fig.\ref{fig:tree123}, %for $N=3$
the $\GG_N$-transversal for $N=3$  %given
here is 3 elements smaller than
the $\Sym_N$-transversal, thus ten entries.
\\
(ii) The two (5,4) cases are
related as per (\ref{de:phinu})(i), but are
not related by our symmetries,
but they are similar as matrices by a non-local conjugation.
\\
(iii) The two (6,3) cases have different Jordan structure over the polynomial ring
of indeterminates.

\medskip

%}}}

\begin{figure}
\includegraphics[width=15.6cm]{xfig/tree123PajN34.eps}
\caption{One-nation configurations up to rank-4. \label{fig:N1234}}
\end{figure}

%{{{ N=4

%\noindent
\mdef
For $N=4$  %Finally here are
the one-nation cases (cf. Fig.\ref{fig:N1234},
and taking account of (\ref{de:phinu})(i))
and some indicative multination cases are: % for $N=4$:

\noindent
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
$\chmp{\square\!\square\!\square\!\square}{000000}{\maps (16)}$
\zzzz
$\chmp{\includegraphics[width=.75cm]{xfig/y000aaa.eps}}{000aaa}{ (12,  4)}$
\zzzz
$\chmp{\includegraphics[width=.75cm]{xfig/y000fff.eps}}{000fff}{ (13,  3)}$
\zzzz
$\chmp{\includegraphics[width=.5cm]{xfig/y0aaaa0.eps}}{0aaaa0}{{(8,8)}}$ % (NB ...)
\zzzz
$\chmp{\includegraphics[width=.5cm]{xfig/y0ffff0.eps}}{0ffff0}{ (12,  4)}$ % (NB ...)
\zzzz
$\chmp{\includegraphics[width=.5cm]{xfig/yaa0faa.eps}}{aa0faa}{(9,  7)}$ % (NB ...)
\zzzz
$\chmp{\includegraphics[width=.5cm]{xfig/yaa0aff.eps}}{aa0aff}{(10,  6)}$ % (NB ...)
\zzzz
$\chmp{\includegraphics[width=.5cm]{xfig/yff0aaa.eps}}{ff0aaa}{(10,  6)}$ % (NB ...)
\zzzz
$\chmp{\includegraphics[width=.5cm]{xfig/yff0fff.eps}}{ff0fff}{{(11,5)}}$ % (NB ...)
\zzzz
$\chmp{\includegraphics[width=.27cm]{xfig/yfaaaaf.eps}}{faaaaf}{(8, \; 8)}$
\zzzz
$\chmp{\includegraphics[width=.27cm]{xfig/yfffaaa.eps}}{fffaaa}{(9, \; 7)}$
\zzzz
$\chmp{\includegraphics[width=.27cm]{xfig/yffffff.eps}}{ffffff}{(10, \; 6)}$
\\ \hline \end{tabular}

\noindent
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
%\\ \hline \end{tabular}
%
%\noindent
%\begin{tabular}{|c|c|c|c|c|c|c|c|}
%\hline
%\zzzz
$\chmp{\square\!\square\!\square\;\square}{000\off\off\off}{ (9;1:3,3)} $
\zzzz
$\chmp{\includegraphics[width=.51cm]{xfig/tree123Pa12.eps}\;\square}{}{(7,2;1\sep 3,3)}$
\zzzz
$\chmp{\square\!\square\;\square\!\square}{0\off\off\off\off 0}{ (4;4:4,4)} $
\zzzz
$\chmp{\includegraphics[width=.2751cm]{xfig/tree123Pa2.eps}\;\square\!\square}{}{(3,1;4\sep 4,4)}$
\zzzz
$\chmp{\includegraphics[width=.2751cm]{xfig/tree123Pa3.eps}\;\square\!\square}{}{(2,2;4\sep 4,4)}$
\zzzz
...
\zzzz
$\chmp{\square\;\square\;\square\;\square}{\off\off\off\off\off\off}{%(1^{16})}$
(1;1;1;1:1^{12})}$
\\ \hline \end{tabular}

%}}}

%\vspace{1cm} %\newpage



%\vspace{1cm}


